Learning RUMs: Reducing Mixture to Single Component via PCA

We consider the problem of learning a mixture of Random Utility Models (RUMs). Despite the success of RUMs in various domains and the versatility of mixture RUMs to capture the heterogeneity in preferences, there has been only limited progress in learning a mixture of RUMs from partial data such as pairwise comparisons. In contrast, there have been significant advances in terms of learning a single component RUM using pairwise comparisons. In this paper, we aim to bridge this gap between mixture learning and single component learning of RUM by developing a `reduction' procedure. We propose to utilize PCA-based spectral clustering that simultaneously `de-noises' pairwise comparison data. We prove that our algorithm manages to cluster the partial data correctly (i.e., comparisons from the same RUM component are grouped in the same cluster) with high probability even when data is generated from a possibly {\em heterogeneous} mixture of well-separated {\em generic} RUMs. Both the time and the sample complexities scale polynomially in model parameters including the number of items. Two key features in the analysis are in establishing (1) a meaningful upper bound on the sub-Gaussian norm for RUM components embedded into the vector space of pairwise marginals and (2) the robustness of PCA with missing values in the $L_{2, \infty}$ sense, which might be of interest in their own right.

==> contents/04_theorem_matrix.tex <==
%%% ======================================================================
%%%	Answer to Problem 1: Matrix Estimation
%%% ======================================================================

\section{Matrix Estimation: Bounding Max Row $\ell_2$ Norm}\label{sec:answer_matrix_estimation}
%\section{On $l_2$ Row Norm in Matrix Estimation}\label{sec:answer_matrix_estimation}

%%% ======================================================================
%%%	Model and Problem Statement
%%% ======================================================================


In this section, we argue that the singular value thresholding (soft and hard) algorithm known
in the literature has the desired property --- that is, it bounds the max $\ell_2$ row norm. This,
in effect, resolves Problem \ref{prob:matrix_estimation} stated in Introduction. 

\subsection{Theorem Statement}
Recall that we let $N, d, p$ denote the number of samples, the dimension of samples, and the probability of 
observing each entries, respectively. We define
\begin{align}
	\Delta(N,d,p) &\triangleq \sqrt{ (1-p) \Lambda^2 + p \tau^2} \sqrt{Np}	\nonumber\\
			&\quad + c_1 (\Lambda + \tau K(p))
			\Big\{\sqrt{C_3 } \big[ (Nd)^{1/4} + (2N \log N)^{1/4} \big] \vee C_3 \big( \sqrt{d} + \sqrt{2 \log N} \big).	\label{eqn:Delta_upper}
\end{align}
We will see that $\Delta(N,d,p)$ plays the role of a high-probability upper bound on $\| Y - pM \|_2$ later in Appendix 
\ref{sec:conditioning_events}\footnote{As a result, $\Delta(N,d,p)$ will be referred many times in the rest of this paper.}. 

\begin{theorem}[Main Theorem]\label{thm:main_MRLE}
	Suppose that Conditions \ref{cond:bounded}, \ref{cond:subgaussian} and \ref{cond:Bernoulli} are satisfied.
	Given $Y \in \Reals^{N \times d}$ and $t^* \geq 0$, let $\widehat {M}= \frac{1}{\hat{p}}\text{HSVT}_{t^*}(Y)$ . 
	Let $r = \text{rank}(M)$. Suppose that 
\begin{enumerate}
	\item $p > \frac{\Delta(N,d,p)}{\sigma_r(M)}$, and
	\item $t^* $ satisfies $\Delta(N,d,p) < t^* < p \sigma_r(M) - \Delta(N,d,p)$.
\end{enumerate}
Then
\begin{align}
	&\max_{i \in [N]} \Big\| \widehat{M}^i - M^i \Big\|_2^2	\nonumber\\
		&\leq 8 c_1^2 c_2^2 \Bigg( \frac{\sqrt{Ndp}}{\sqrt{Ndp} - 2 \sqrt{\log (Nd)}} \Bigg)^2 
			\frac{\big(\tau + \Lambda K(p) \big)^2 }{p^2}
			\left[ r + \left(  \frac{\Delta(N,d,p)}{p \sigma_r(M) - \Delta(N,d,p)} \right)^2 d \right]  \log ( 2d N^5)	\nonumber\\
		&\quad	+ \left[ 2 \left( \frac{2\sqrt{\log(Nd)}}{\sqrt{Ndp} - 2\sqrt{\log(Nd)}} \right)^2
			+ \left( \frac{\Delta(N,d,p)}{ p \sigma_r(M) - \Delta(N,d,p)} \right)^2 \right] \Lambda^2 d	\label{eqn:maxell2_upper}
\end{align}
with probability at least $1 - \frac{4}{N^4} - \frac{2}{N^2d^2}$.
\end{theorem}
In the rest of this paper, we let $\Phi(N,d;p,\tau,\Lambda)$ denote the upper bound in \eqref{eqn:maxell2_upper} to save the space.
We defer the proof of Theorem \ref{thm:main_MRLE} until Appendix \ref{sec:proof_main}.

\subsection{Interpretation of Result}\label{sec:interpretation_main}
If $p \gg \sqrt{\frac{\log (Nd)}{Nd}} $, then $ \frac{\sqrt{Ndp}}{\sqrt{Ndp} - 2 \sqrt{\log (Nd)}} \approx 1$. Moreover, 
if $p \gg \frac{\Delta(N, d, p)}{ \sigma_r(M)}$, then $\frac{\Delta(N,d,p)}{ p \sigma_r(M) - \Delta(N,d,p)} \approx 0$ and 
the upper bound stated in Theorem \ref{thm:main_MRLE} reduces to 
\[	\max_{i \in [N]} \Big\| \widehat{M}^i - M^i \Big\|_2^2
	\leq C \frac{(\tau + \Lambda K(p) )^2 }{p^2} r \log(Nd) = \tilde{O}\Big( \frac{r}{p^2} \Big).	\]
In the following corollary, we present a sufficient condition on $p$ to achieve an asymptotically vanishing error in terms of the squared max row $\ell_2$ norm (normalized).
	
\begin{corollary}\label{cor:matrix_estimation}
	Suppose that the parameter matrix $M$ is `well behaved,' i.e., $\sigma_r(M) = \Omega\Big(\sqrt{ \frac{Nd}{r} } \Big)$ 
	where $r = \rank(M)$. Then we have the following upper bound on the squared max row $\ell_2$ norm error in the asymptotic 
	regime where $N, d \to \infty$:
	\begin{enumerate}
		\item
		When $p = const.$, $\exists C > 0$ such that 
		$\max_{i \in [N]} \big\| \widehat{M}^i - M^i \big\|_2^2  \leq C (\tau + \Lambda)^2 \left( 1 + \sqrt{\frac{d}{N}} + \frac{d}{N} \right) r$.
		\item
		Suppose that $\tau, \Lambda = O(1)$. If $p = \omega \bigg( \Big( \frac{ r \log(Nd) }{d}\Big)^{1/3}  \vee 
		\Big( \frac{r \log(Nd) }{\sqrt{Nd}}\Big)^{1/4} \vee \Big(\frac{r \log(Nd) }{N} \Big)^{1/4}\bigg)$, then 
		$\max_{i \in [N]} \big\| \widehat{M}^i - M^i \big\|_2^2 = o(d)$.
	\end{enumerate}
\end{corollary}

\begin{remark}\label{rem:matrix_estimation}
We may assume $\| M^i \|_2^2 = \Theta(d)$ for all $i \in [N]$ (or equivalently, $|M_{ij}| = \Theta(1)$ for all $i, j$). 
Then Corollary \ref{cor:matrix_estimation} implies we can achieve a vanishing upper bound on the normalized max row $\ell_2$ norm:
\[	p = \omega \bigg( \Big( \frac{ r \log(Nd) }{d}\Big)^{1/3}  \vee \Big( \frac{r \log(Nd) }{\sqrt{Nd}}\Big)^{1/4} 
	\vee \Big(\frac{r \log(Nd) }{N} \Big)^{1/4}\bigg)	\quad\text{implies}\quad
	\frac{1}{d}\max_{i \in [N]} \big\| \widehat{M}^i - M^i \big\|_2^2 = o(1).
	\]
\end{remark}

 
 



==> contents/05_theorem_mixture.tex <==
%%% ======================================================================
%%%	Answer to Problem 1: Mixture Learning
%%% ======================================================================

\section{Learning Mixture with Missing Values }\label{sec:mixture_clustering}
In this section, we describe the algorithm for clustering observations (=data vectors) generated from mixture
distribution. We argue that algorithm clusters the observations\footnote{This is a stronger objective than just 
learning parameters of component distributions. Also, this is essentially the reason why we need a sufficient 
separation between cluster means.} correctly, i.e. all observations in any learned cluster are from the same mixture 
component even when the observations have missing values as long as sufficiently many data points are observed. 
This answers the Problem \ref{prob:mixture_clustering} stated in Introduction. 

\subsection{Preliminaries}
\subsubsection{Some definitions} We recap some definitions and introduce additional notations here. 
Let $k$ denote the number of clusters in the mixture model. For each $a \in [k]$, we define the following quantites.
\begin{enumerate}
%	\item
%		Weight: $w_a \triangleq \Prob{M^i = \mu^a}$.
	\item
		Cluster mean: $\mu^a \triangleq \Exp{X^i \big| M^i = \mu^a}$. We write $\mu_a = (\mu^a)^T$.
%	\item
%		Cluster covariance: \DG{Do we use this quantity?}
%		\[	\Sigma_a \triangleq \Exp{ \big( X^i - M^i \big)^T\big( X^i - M^i \big) \big| M^i = \mu^a}.	\]
	\item
		Cluster $\phi_2$/$\psi_2$-norm: 
		\begin{align*}
			\tau_a \triangleq \inf_{\tau > 0} \bigg\{\sup_{u \in \mathbb{S}^{d-1}} \Exp{ \exp \big( \lambda  (X^i - M^i)u \big) ~\Big|~ M^i = \mu^a} \leq \exp\bigg( \frac{\lambda^2 \tau^2}{2}\bigg) 
		\hfill\text{ for all }\lambda \in \Reals \bigg\}.
		\end{align*}
\end{enumerate}
 Let $\alpha: [N] \to \{ 1, \ldots, k\}$ denote an oracle map such that $\alpha(i)$ denotes the index of the component which 
$X^i$ is drawn from. For each $a, b \in [k]$, let $\Gamma_{a,b} \triangleq \big\| \mu^a - \mu^b \big\|_2$  and
$\Gamma \triangleq \min_{a, b \in [k]} \Gamma_{a,b}$. 


\subsubsection{Induced thresholding operator.} Given a matrix $A = \sum_{j=1}^{\min\{N, d\}} \sigma_j(A) u_j v_j^T$ 
and a threshold $t \geq 0$, the HSVT as per \eqref{eqn:hsvt} suggests the following operator $\varphi_{A;t}^{\text{hard}}: 
\Reals^d \to \Reals^d$ defined as 
\begin{equation*}
	\varphi^{\text{hard}}_{A; t} : w \mapsto \sum_{j=1}^d \Ind{\sigma_j(A) \geq t}  \cP_{v_j} (w),
\end{equation*}
where $\cP_{v_j}$ denotes the projection onto $\text{span}(v_j)$. This operator satisfies the following properties: for 
any matrix $A \in \Reals^{N \times d}$ and $t \geq 0$,
\begin{align*}
	HSVT_t(A)^i = \varphi^{\text{hard}}_{A; t} \big( A^i \big), 	\quad\forall i \in [N],
	\qquad\text{and}\qquad
	\big\| \varphi^{\text{hard}}_{A;t} (w) \big\|_2 \leq \| w \|_2,	\quad\forall w \in \Reals^d.
\end{align*}
See Appendix \ref{sec:more_hsvt} for more details.


\subsection{Theorem Statement}
\subsubsection{Generic Result}
As defined in Section \ref{sec:gen_model}, we observe $N$ random vectors with missing values denoted as the rows 
of matrix $Y \in \Reals^{N\times d}$. The goal of the algorithm is to cluster these $N$ row indices into disjoint clusters, 
i.e. sets $S_1, \dots, S_\ell$ so that $S_a \cap S_b = \emptyset$, $S_a \subset [N]$ for all $a, b \leq \ell$. The algorithm 
{\em does not} know the number of mixture components, $k$. The ideal output would be where $\ell = k$ and $S_a$ 
contains precisely the row that correspond to mixture component $a$ (of course, up to relabeling of the mixture components). 
We propose a generic recipe for clustering as described in Algorithm \ref{alg:main_algorithm}.

The following theorem ensures that known methods for learning a mixture of sub-gaussian distributions apply after 
pre-processing data with a matrix estimation (HSVT, to be precise) subroutine. Note that 
$\frac{1}{\hat{p}}\varphi^{\text{hard}}_{Y;t^*}\big( Y^i \big)$.

\begin{theorem}\label{thm:main_mixture}
Suppose that Conditions \ref{cond:bounded}, \ref{cond:subgaussian} and \ref{cond:Bernoulli} are satisfied.
Given $Y \in \Reals^{N \times d}$ and $t^* \geq 0$, let $\widehat {M}= \frac{1}{\hat{p}}\text{HSVT}_{t^*}(Y)$. 
Let $r = \text{rank}(M)$. Suppose that two assumptions for Theorem \ref{thm:main_MRLE}\footnote{Assumption 1 is: 
$p > \frac{\| Y - pM \|_2}{\sigma_r(M)}$} hold. 
Then the following two conclusions hold with probability at least $1 - \frac{2}{N^2d^2}$:
\begin{enumerate}
	\item	For every $i \in [N]$,
	\begin{align*}
	\bigg\|  \widehat{M}^i - \frac{p}{\hat{p}}\varphi^{\text{hard}}_{Y; t^*} \big(\mu^{\alpha(i)} \big) \bigg\|_{\psi_2}
		&\leq  c_1 \bigg(1 - 2 \sqrt{\frac{\log (Nd)}{ Nd p}}\bigg)^{-1} \bigg(\frac{\tau_{\alpha(i)} + \Lambda K(p) }{p}\bigg).
	\end{align*}

	Here, $C$ is an absolute constant\footnote{More precisely, this constant appears while transferring between the second 
	and the fourth characterizations of subgaussian random variable; see \eqref{prop:subG_characterization}.}.
	
	\item For every $a, b \in [k]$,
	\begin{align*}
		\left\|  \frac{p}{\hat{p}} \varphi_{Y;t^*}^{\text{hard}} \big(  \mu^a - \mu^b \big) \right\|_2^2
		&\geq \left( 1 - \bigg( \frac{ \| Y - pM \|_2 }{p \sigma_r(M) - \| Y - pM \|_2 }\bigg)^2\right)
			\big\|  \mu^a - \mu^b \big\|_2^2.
	\end{align*}
\end{enumerate}
\end{theorem}
The proof of Theorem \ref{thm:main_mixture} can be found in Appendix \ref{sec:proof_thm_mixture.1}.


Theorem \ref{thm:main_mixture} implies that pre-processing with HSVT subroutine (step 2 in Algorithm \ref{alg:main_algorithm}) 
reduces the given mixture learning problem with values to another subgaussian mixture problem. In the new problem, we can consider 
$ \frac{p}{\hat{p}} \varphi_{Y;t^*}^{\text{hard}} \big(  \mu^a \big)  $ as new centers of the clusters, and each component distribution 
of $ \widehat{M}^i - \frac{p}{\hat{p}}\varphi^{\text{hard}}_{Y; t^*} \big(\mu^{\alpha(i)} \big) = \frac{1}{\hat{p}}
\varphi^{\text{hard}}_{Y; t^*} \big(Y^i - p \mu^{\alpha(i)} \big) $ is again subgaussian. The separation between the cluster means 
and the $\psi_2$-norm of the clusters remain the same up to constant as long as there exists a constant $C' > 0$ such that 
$p \geq C'\frac{\| Y - pM \|_2}{\sigma_r(M)}$.

Together with Proposition \ref{prop:subG_Z}, Theorem \ref{thm:main_mixture} translates as: ``mixture learning with missing values 
is equivalent to mixture learning with the cluster $\psi_2$-norms multiplied by $\frac{1}{p}$.''



\subsubsection{A More Concrete Result: Distance-based Clustering}
Now we specifically consider distance-based clustering algorithms to achieve a concrete sufficient condition for identifiability. 
We argue having a sufficiently large separation between cluster means implies that the mixture components are identifiable by 
a simple distance-based clustering. Before stating the theorem, we formally state this separate condition. Recall that 
$\Phi(N,d;p,\tau,\Lambda)$ denotes the expression on the right hand side of \eqref{eqn:maxell2_upper}.

\begin{condition}[Sufficient mean separation]\label{cond:minimum_gap}
Let $N$ denote the number of samples, $d$ denote the dimension of data vectors, and $p$ denote the probability of observing 
each entry of data vectors. The minimum separation between two cluster means satisfy
\begin{align*}
	\Gamma^2
		&\geq 4 \Phi(N,d;p,\tau,\Lambda).
\end{align*}
\end{condition}

We emphasize that Condition \ref{cond:minimum_gap} is a sufficient condition for learnability of a mixture 
with missing values, which allows a simple distance-based clustering algorithm to correctly group the data vectors. 
This is not a necessary condition for the learnability (and the identifiability) of a mixture model. Also, we note that 
unlike the aforementioned three conditions--\ref{cond:bounded}, \ref{cond:subgaussian}, \ref{cond:Bernoulli}--imposed 
on the generative model, condition \ref{cond:minimum_gap} (weakly, though) depends on the instance of parameter matrix 
$M \in \Reals^{N \times d}$ through its smallest nonzero singular value, $\sigma_r(M)$ and $N$ (=the number of samples).


\begin{theorem}\label{thm:clustering}
Given $Y \in \Reals^{N \times d}$ and $t^* \geq 0$, let $\widehat {M}= \frac{1}{\hat{p}}\text{HSVT}_{t^*}(Y)$. 
Let $r = \text{rank}(M)$. Suppose that  conditions \ref{cond:bounded}, \ref{cond:subgaussian}, 
\ref{cond:Bernoulli} and \ref{cond:minimum_gap} are satisfied. Moreover, suppose that two conditions for Theorem 
\ref{thm:main_MRLE} hold. Then
\begin{align*}
	\sup_{i_1, i_2 \in [N] \atop \alpha(i_1) = \alpha(i_2)} \big\| \hat{M}^{i_1} - \hat{M}^{i_2} \big\|_2 
		<
	\inf_{i_1, i_2 \in [N] \atop \alpha(i_1) \neq \alpha(i_2)} \big\| \hat{M}^{i_1} - \hat{M}^{i_2} \big\|_2
\end{align*}
	with probability at least  $1 - \frac{4}{N^4} - \frac{2}{N^2d^2}$.
\end{theorem}
The proof of Theorem \ref{thm:clustering} can be found in Appendix \ref{sec:proof_thm_mixture.2}.


\begin{corollary}\label{cor:distance_clustering}
Suppose that the generative model satisfies conditions \ref{cond:bounded}, \ref{cond:subgaussian} 
and \ref{cond:minimum_gap}. Then with probability at least $1 - \frac{4}{N^4} - \frac{2}{N^2d^2}$
\footnote{If we consider a random problem instance, it is solvable with this probability.}, the mixture components 
in a problem instance $Y_1, \ldots, Y_N \in \Reals^d$ are learnable (hence, identifiable) when $p> \frac{\Delta(N,d,p)}{\sigma_r(M) }$.
\end{corollary}

\begin{corollary}\label{cor:mixture_clustering}
	Suppose that the parameter matrix $M$ is `well behaved,' i.e., $\sigma_r(M) = \Omega\Big(\sqrt{ \frac{Nd}{r} } \Big)$ 
	where $r = \rank(M)$. Then we have the following lower bound on the minimum separation $\Gamma^2$ and sample complexity $p$ 
	in the asymptotic regime where $N, d \to \infty$:
	\begin{enumerate}
		\item
		Given $N, d, p$, if $\Gamma^2 \geq C \frac{(\tau + \Lambda)^2 r}{p^3} \left(1 + \frac{1}{p}\sqrt{\frac{d}{N}} 
		+ \frac{1}{p}\frac{d}{N} \right) \log(Nd)$ for sufficiently large $C > 0$, then distance-based clustering succeeds with high probability.
		\item
		Given $N, d, \Gamma$, if $p \geq C \bigg[ \Big( \frac{(\tau + \Lambda)^2r \log(Nd)}{\Gamma^2}\Big)^{1/3} \vee 
		\Big( \frac{(\tau + \Lambda)^2r \log(Nd)}{\Gamma^2}\Big)^{1/4}\Big( \frac{d^{1/4}}{N^{1/4}} \vee \frac{d^{1/8}}{N^{1/8}} \Big) \bigg] $ 
		for sufficiently large $C > 0$, then distance-based clustering succeeds with high probability.
	\end{enumerate}
\end{corollary}

\begin{remark}\label{rem:clustering.1}
Assuming $N \gg d$ and $\tau, \Lambda = O(1)$, requiring $\Gamma = \tilde{\Omega}\Big( \frac{r}{p^{3/2}} \Big)$ is sufficient 
for distance-based clustering to succeed with high probability. That means we need $\frac{1}{p^{3/2}}$ times larger separation 
to compensate having only $p$ fraction of entries observed.
\end{remark}

\begin{remark}\label{rem:clustering.2}
Assuming $N \gg d$ and $\tau, \Lambda = O(1)$, observing $p = \tilde{\Omega}\Big(\frac{r}{\Gamma^2}\Big)^{1/3}$ fraction 
of entries is sufficient for distance-based clustering to succeed with high probability. Since $\Gamma^2 = O(d)$, we need at least 
$p = \tilde{\Omega}\Big( \big(\frac{r}{d}\big)^{1/3} \Big)$ in the best scenario.
\end{remark}


==> contents/06_mixture_ranking.tex <==
\section{Application to Learning a Mixture of Ranking Models}\label{sec:ranking_identifiability}
In this section, we discuss how we reduce the problem of learning a mixture of ranking models to 
a more extensively studied problem of learning a mixture in vector space. We obtain a 
identifiability/learnability theorem as a consequence of the discussion in this section. This provides 
an answer to Problem \ref{prob:ranking_identifiability} stated in Introduction.


\subsection{Embedding Permutations to Its Pairwise Marginals}
%Given a permutation $\sigma \in S_n$, its pairwise marginal is a ${n \choose 2}$-dimensional binary vector, 
%whose $ij$-th coordinate ($1 \leq i < j \leq n$) takes value $\pm 1$. We formally define the embedding map first.
%\begin{definition}[Embedding to pairwise marginals]
%Let the embedding of permutation to its pairwise marginals, denoted $\iota: S_n \to \{ \pm 1 \}^{n \choose 2}$, 
%be defined as follows: for $\sigma \in S_n$ and $1 \leq i < j \leq n$,
%\[	
%	\iota(\sigma)_{ij} =\begin{cases}
%					1	&\text{if }\sigma^{-1}(i) \geq \sigma^{-1}(j),\\
%					-1	&\text{otherwise}.
%		\end{cases}
%\]
%\end{definition}
%\begin{remark}\label{rem:norm_embedding}
%	Note that for any $\sigma \in S_n$, $\iota(\sigma) \in \{ \pm 1 \}^{n \choose 2}$, and hence, 
%	$\big\| \iota(\sigma) \big\|_2 = \sqrt{\frac{n(n-1)}{2}}$.
%\end{remark}

Now we argue that the Kendall's tau metric in $S_n$ is equivalent (up to constant) to the squared $\ell_2$ metric 
in the embedded space, $\iota(S_n)$.
\begin{definition}\label{def:kendall_tau}
	Given $\sigma_1, \sigma_2 \in S_n$, the Kendall's tau distance between $\sigma_1$ and $\sigma_2$ is defined as
	\[	d_{KT}(\sigma_1, \sigma_2) \triangleq \sum_{1 \leq i < j \leq n} \Ind{ \iota(\sigma_1)_{ij} \neq \iota(\sigma_2)_{ij} }.	\]
\end{definition}

\begin{proposition}\label{prop:KT_ell2}
	For any positive integer $n$ and for any $\sigma_1, \sigma_2 \in S_n$,
	\[	d_{KT}(\sigma_1, \sigma_2) = \frac{1}{4} \big\| \iota(\sigma_1) - \iota(\sigma_2) \big\|_2^2.	\]
\end{proposition}
The proof of Proposition \ref{prop:KT_ell2} can be found in Appendix \ref{sec:proof_kt_ell2}.


\begin{remark}
	The cluster mean, $\Exp{ \iota(\sigma)} \in [-1, 1]^{n \choose 2}$, is introduced as a tool for analysis. 
	In general, it may not correspond to the image of any realizable permutation in $S_n$.
\end{remark}

\subsection{Two Popular Examples of Ranking Models}
\subsubsection{Random Utility Model}\label{sec:gen_permutations}
There are $n$ options available. Each option $i \in [n]$ has a deterministic utility $u_i$ associated with it. 
The random utility $Y_i$ associated with option $i \in [n]$ obeys the form
\begin{equation}\label{eqn:random_utility}
	Y_i = u_i + \eps_i,
\end{equation}
where $\eps_i$ are independent random variables. Once random variables $Y_i$ are generated for all $i \in [n]$ 
as per \eqref{eqn:random_utility}, $Y_1, \ldots, Y_n$ are sorted in descending order. The order of indices is output 
as a permutation.

\begin{example}[Multinomial Logit Model (MNL)]
Let $\eps_i$ drawn as per Gumbel distribution with mode $\mu_i$ and scaling parameter $\beta_i > 0$, 
i.e., the PDF of $\eps_i$ is given by 
\[	f(x) = \frac{1}{\beta_i} \exp \left( - \left( \frac{x - \mu_i}{\beta_i} + 
	\exp \Big( - \frac{x - \mu_i}{\beta_i} \Big) \right) \right).	\]
In the homogeneous setting, $\mu_i = \mu$, $\beta_i = \beta$ for all $i$.
for all $i \in [n]$.
\end{example}

\begin{proposition}\label{prop:subg_rum}
	Let $\sigma$ generated as per a random utility model; see \eqref{eqn:random_utility}. Then the derived distribution 
	of $\iota(\sigma)$ is subgaussian. Moreover,
	\[	\big\| \iota(\sigma) - \bbE \iota(\sigma) \big\|_{\psi_2}\leq C \sqrt{n-1}.	\]
\end{proposition}
The proof of Proposition \ref{prop:subg_rum} can be found in Appendix \ref{sec:proof_subg_rum}.


\subsubsection{Mallows Model}
The Mallows model  and its generalizations are another example of ranking model of choice used in various fields 
including statistics, political science, etc. The distribution (probability mass function) of the Mallows model is 
characterized by the center permutation $\sigma_0 \in S_n$ and scaling factor $\phi \in (0, 1)$. Specifically, 
given $\sigma_0$ and $\phi$, 
\begin{equation}\label{eqn:mallows}
	\Prob{\sigma} = \frac{\phi^{d_{KT}(\sigma, \sigma_0)}}{Z},
\end{equation}
where $Z = \sum_{\sigma \in S_n} \phi^{d_{KT}(\sigma, \sigma_0)}$ is the partition function.

\begin{proposition}\label{prop:subg_mallows}
	Let $\sigma$ generated as per a Mallows model; see \eqref{eqn:mallows}. Then the derived distribution of 
	$\iota(\sigma)$ is subgaussian. Moreover,
	\[	\big\| \iota(\sigma) - \iota(\sigma_0) \big\|_{\psi_2}\leq C \sqrt{n \log n}.	\]
\end{proposition}
The proof of Proposition \ref{prop:subg_mallows} can be found in Appendix \ref{sec:proof_subg_mallows}.


\subsection{Theorem Statement and Discussion}
Now our samples $Y_1, \ldots, Y_N$ are partial (and possibly noisy) observations of pairwise marginals in 
$\{ \pm 1\}^{n \choose 2}$. The parameter matrix $M \in [-1, 1]^{N \times {n \choose 2}}$ in this setup is 
the stack of cluster means in the embedded space, i.e., $\Exp{ \iota(\sigma) ~ \big| ~ a = \alpha(i) } \in [-1, 1]^{n \choose 2}$.


\begin{theorem}[Sufficient condition for identifiability of ranking mixture]\label{thm:identifiable}
Suppose that $\| \iota(\sigma) - \bbE \iota(\sigma) \|_{\phi_2} \leq \tau$ for all clusters in the mixture and that 
condition \ref{cond:Bernoulli} is satisfied. If 
\begin{enumerate}
	\item $\Gamma^2	\geq  8 ~\text{rank}(M) \left(1 + 32 c_1^2 c_2^2  \frac{\big(\tau + K(p) \big)^2 }{p^2} \log ( 2n^2 N^5) \right)$ and
	\item $p> \frac{\Delta\big(N,{n \choose 2},p\big)}{\sigma_r(M) }$,
\end{enumerate}
then with probability at least $1 - \frac{4}{N^4} - \frac{2}{N^2n^4}$ 
\footnote{If we consider a random problem instance, it is solvable with this probability.}, the mixture components 
in a mixture ranking problem instance are identifiable/learnable.
\end{theorem}
The proof of Theorem \ref{thm:identifiable} can be found in Appendix \ref{sec:proof_learnable}.

Equipped with the upper bounds stated in Proposition \ref{prop:subg_rum} and Proposition \ref{prop:subg_mallows}, 
Theorem \ref{thm:identifiable} suggests a sufficient condition for when the components in a mixture ranking model is 
learnable (hence, identifiable). We recall that $\Lambda = 1$, and $d = {n \choose 2}$ for any ranking models; and that 
$\tau \asymp \big\| \iota(\sigma) - \bbE \iota(\sigma) \big\|_{\psi_2} \leq C\sqrt{n}$ for random utility model. From 
Theorem \ref{thm:identifiable} and the discussions in Section \ref{sec:interpretation_main} (paragraph on sample complexity), 
we can deduce the following conclusions.
\begin{enumerate}
	\item Having the cluster means separated by at least $\tilde{\Omega} \Big( \frac{ \sqrt{r n}}{p} \Big)$ 
		is sufficient for learnability. 
	\item	Observing at least $N \gtrsim \frac{n r}{p^2}$ number of samples is sufficient to recover $M$.
	\item When $N \gg d$, we can recover $M$ if we have $p \gtrsim \frac{r}{n}$ fraction of observations.
\end{enumerate}

Now suppose that $p = 1$. The separation condition becomes $\Gamma = \tilde{O}(\sqrt{nr})$. Also, the sample complexity 
becomes $N \gtrsim nr$, which means having $n^3 r$ number of pairwise comparisons is sufficient for learning the model 
(because there are ${n \choose 2}$ number of entries in each sample when $p = 1$).


\subsubsection{Further Discussion}
Note that Kendall's tau distance can range from $0$ to ${n \choose 2}$. Therefore, the separation condition of 
$\tilde{\Omega} \Big( \frac{ \sqrt{r n}}{p} \Big)$ already provides a nontrivial learnability condition. Due to 
the equivalence of Kendall's tau with the squared $\ell_2$ distance in the embedding (see Proposition \ref{prop:KT_ell2}), 
$\| \iota(\sigma_1) - \iota(\sigma_2) \|_2^2$ ranges from $0$ to $\sqrt{2n(n-1)}$. Therefore, if two cluster means 
$\mu_1, \mu_2 \in S_n$ are sampled uniformly at random, then they would highly likely satisfy 
$\|\iota(\mu_1) - \iota(\mu_2) \|_2 \gg \sqrt{n}$.

Nevertheless, we believe our results could be improved further in several directions. First, we believe that the upper bounds 
on the cluster subgaussian norms stated in Proposition \ref{prop:subg_rum} and Proposition \ref{prop:subg_mallows} 
are suboptmal. We believe $O(\sqrt{n})$ for random utility model (and $O(\sqrt{n \log n})$ for Mallows model) is a loose 
upper bound because (i) its proof barely utilizes structural properties of Random utility model; and (ii) the upper bound 
does not depend on the deterministic utilities $u_i$'s at all. We believe this upper bound can be improved significantly, 
which will lead to an equivalent improvement in the separation requirement stated in Theorem \ref{thm:identifiable}.

Second, Theorem \ref{thm:identifiable} is a corollary of Theorem \ref{thm:clustering} and Corollary \ref{cor:distance_clustering}. 
It only considers learnability of ranking mixture for distance-based clustering algorithms. We believe this result can be extended to 
a more general class of mixture learning methods as Theorem \ref{thm:main_mixture} suggests that the user is left with a usual 
sub-gaussian mixture learning problem after the pre-processing step--(i) reducing the ranking problem to a mixture learning with 
missing values and then (ii) running a matrix estimation subroutine. It would be interesting to see if one can get results for mixture 
ranking problems that are similar to those in \cite{regev2017learning, diakonikolas2016robust, kothari2017better, hopkins2018mixture}.

Lastly, the model for partial, noisy observations can be extended further. Currently, we consider the following data generation process: 
(i) a noisy version of permutation is drawn from a mixture component, and then (ii) a fraction of entries in its embedded image is masked 
(deleted). Since we replace $\star$ with $0$ while running HSVT operation, we may consider the data vector $Y_i$ as a projection of 
a point in $\iota(S_n) \subset \{\pm 1\}^{n \choose 2}$ onto some subspace $\Reals^n_1 \times \{0\}^{{n \choose 2} - n_1}$.

In practical applications, data vectors are usually gathered as a collection of pairwise comparisons. That means aggregating a batch 
of those pairwise marginals might not lead to a consistent total ordering, even when they are gathered from a single person/subject. 
In other words, the pre-masked data vector could be any point in the entire hypercube $\{\pm 1\}^{n \choose 2}$, which has a much 
larger cardinality than $\iota(S_n) $; $2^{n \choose 2}$ vs $n! \approx 2^{n \log n}$. Also, one could come up with a different masking 
scheme: nonuniform mask, partial observation with a confidence level, etc.



Recall Corollary \ref{cor:mixture_clustering} first. Note that $d = {n \choose 2}$, $\Lambda = 1$, and we have $\tau = O(\sqrt{n})$ for 
random utility model ($\tau = \tilde{O}(\sqrt{n})$ for Mallows model).
\begin{corollary}\label{cor:ranking}
	Suppose that the parameter matrix $M$ is `well behaved,' i.e., $\sigma_r(M) = \Omega\Big( n\sqrt{\frac{N}{r} } \Big)$ 
	where $r = \rank(M)$. Then we have the following lower bound on the minimum separation $\Gamma^2$ and sample complexity $p$ 
	in the asymptotic regime where $N, n \to \infty$:
	\begin{enumerate}
		\item
		Given $N, n, p$, if $\Gamma^2 \geq C \frac{n r}{p^3} \left(1 + \frac{1}{p}\frac{n}{\sqrt{N}} 
		+ \frac{1}{p}\frac{n^2}{N} \right) \log(Nn)$ for sufficiently large $C > 0$, then distance-based clustering succeeds with high probability.
		\item
		Given $N, n, \Gamma$, if $p \geq C \bigg[ \Big( \frac{nr \log(Nn)}{\Gamma^2}\Big)^{1/3} \vee 
		\Big( \frac{n r \log(Nn)}{\Gamma^2}\Big)^{1/4}\Big( \frac{n^{1/2}}{N^{1/4}} \vee \frac{n^{1/4}}{N^{1/8}} \Big) \bigg] $ 
		for sufficiently large $C > 0$, then distance-based clustering succeeds with high probability.
	\end{enumerate}
\end{corollary}



\begin{remark}\label{rem:ranking.1}
Assuming $N \gg n$, requiring $\Gamma = \tilde{\Omega}\Big( \frac{\sqrt{nr}}{p^{3/2}} \Big)$ is sufficient for distance-based 
clustering to succeed with high probability. Note that $\sqrt{n}$ factor stems from our upper bound on the subgaussian norm of 
component distributions and possibly further improved.
%That means we need $\frac{1}{p^{3/2}}$ times larger separation to compensate having only $p$ fraction of entries observed.
\end{remark}

\begin{remark}\label{rem:ranking.2}
Assuming $N \gg n$, observing $p = \tilde{\Omega}\Big(\frac{n r}{\Gamma^2}\Big)^{1/3}$ fraction of entries is sufficient for 
distance-based clustering to succeed with high probability. Since $\Gamma^2 = O(n^2)$, we need at least $p = \tilde{\Omega}\Big( \big(\frac{r}{n}\big)^{1/3} \Big)$ in the best scenario.
\end{remark}



==> contents/11_conclusion.tex <==
\section{Conclusion}


==> contents/Appx02_key_lemma_and_proof.tex <==
%%% ======================================================================
%%%	Proof of Theorems
%%% ======================================================================

\section{ Key Lemma for Theorem \ref{thm:main_MRLE}}\label{sec:proof_preliminary}

\subsection{More on HSVT}\label{sec:more_hsvt}
\subsubsection{Induced Thresholding Operator.} Given a matrix $A = \sum_{j=1}^{\min\{N, d\}} \sigma_j(A) u_j v_j^T$ 
and a threshold $t \geq 0$, the HSVT as per \eqref{eqn:hsvt} suggests the following operator $\varphi_{A;t}^{\text{hard}}: 
\Reals^d \to \Reals^d$ defined as 
\begin{equation} \label{eq:hardsvt.1} 
	\varphi^{\text{hard}}_{A; t} : w \mapsto \sum_{j=1}^d \Ind{\sigma_j(A) \geq t}  \cP_{v_j} (w),
\end{equation}
where $\cP_{v_j}$ denotes the projection onto $\text{span}(v_j)$; specifically, when $w \in \Reals^d$ 
as a row vector representation, $\cP_{v_j}(w) = w v_j v_j^T$. If we take the column vector 
representation, it would be natural to consider $\cP^{v_j}(w) = v_j v_j^T w$
\footnote{These are just two different representations of the same projection operation, 
and we shall switch between the row vector representation (left multiplication) and the column vector representation  
(right multiplication) for convenience of explanation; however it will be clear from the context whether we are using row or
column representation.}.

\begin{lemma}\label{lem:contraction}
	For any matrix $A \in \Reals^{N \times d}$ and $t \geq 0$, $\varphi^{\text{hard}}_{A;t}$ is a contraction, i.e.,
	\[	\big\| \varphi^{\text{hard}}_{A;t} (w) \big\|_2 \leq \| w \|_2,	\qquad \forall w \in \Reals^d.	\]
\end{lemma}

\begin{proof}
	Write $A = \sum_{j=1}^{\min\{N, d\}} \sigma_j (A) u_j v_j^T$. Recall that the right singular vectors of $A$ 
	forms an orthonormal basis of $\Reals^{\min\{N, d\}}$. For any $w \in \Reals^d$,
	\begin{align*}
		\big\| \varphi^{\text{hard}}_{A;t} (w) \big\|_2^2
			&= \left(\sum_{j=1}^{\min\{N, d\}} \Ind{\sigma_j(A) \geq t}  \cP_{v_j} (w) \right)^2\\
			&= \sum_{j=1}^{\min\{N, d\}} \Ind{\sigma_j(A) \geq t}  \cP_{v_j} (w)^2\\
			&\leq  \sum_{j=1}^{\min\{N, d\}} \cP_{v_j} (w)^2\\
			&= \| w \|_2^2.
	\end{align*}
\end{proof}


\begin{lemma}\label{lem:hsvt_induced}
	Given $A \in \Reals^{N \times d}$ and $t \geq 0$,  
	\[	\HSVT_t(A)^i = \varphi^{\text{hard}}_{A; t} \big( A^i \big), \qquad \forall i \in [N].	\]
\end{lemma}

\begin{proof}  
Let $A = \sum_{j = 1}^{\min\{N, d\}} \sigma_j(A) u_j v_j^T$ be the SVD of $A$. By the orthonormality of the left singular vectors, 
\begin{align*}
	 \varphi^{\text{hard}}_{A; t} \big( A^i \big)
	 	&= \sum_{a=1}^{\min\{N, d \}} \Ind{\sigma_i (A) \geq t} \cP_{v_i} \big(A^a \big)
		= \sum_{a=1}^{\min\{N, d \}} \Ind{\sigma_a (A) \geq t}A^i v_a v_a^T\\
		&= \sum_{a, b=1}^{\min\{N, d \}} \Ind{\sigma_a (A) \geq t} e_i^T \sigma_{b}(A) u_{b} v_{b}^T  v_a v_a^T\\
		&= e_i^T \sum_{a, b=1}^{\min\{N, d \}} \Ind{\sigma_a (A) \geq t} \sigma_{b}(A) u_{b} \delta_{a b} v_a^T\\
		&= e_i^T \HSVT_t(A)
		= \HSVT_t(A)^i.
\end{align*}
This completes the proof. 
\end{proof}



\subsubsection{A Small Lemma for the Choice of $t^*$ so that $\widehat{M}= \frac{1}{\hat{p}}\HSVT_{t^*}(Y)$}
\begin{lemma}\label{lemma:thresholding_rank}
Given $Y \in \Reals^{N \times d}$ and $t^* \geq 0$, let $\widehat{M} = \frac{1}{\hat{p}}\HSVT_{t^*}(Y)$. Let $r = \emph{rank}(M)$.
If $\| Y - pM \|_2 < t^* < \sigma_r(M) - \| Y - pM \|_2$, then $\emph{rank}(\widehat{M}) = r$. 
\end{lemma}

\begin{proof}
Recall from \eqref{eqn:hsvt} that 
$$	\HSVT_{t^*}(Y)	= \sum_{j=1}^{\min\{N, d\}} \sigma_j(Y) \Ind{\sigma_j(Y) \geq t} u_j v_j^T	$$
and hence, only the components of $Y$ with singular value at greater than or equal to $t^*$ survive after 
$\HSVT_{t^*}$ operation. Therefore, it suffices to show $\sigma_{r+1}(Y) < t^* \leq  \sigma_r(Y)$.

We may write $Y$ as
\[	Y = pM + \big( Y - pM \big).	\]
Note that $\sigma_r(M) > \sigma_{r+1}(M) = 0$ by the assumption. By Weyl's theorem,
\begin{align*}
	\sigma_{r}(Y) &\ge \sigma_r(pM) - \| Y - pM \|_2= p\sigma_r(M) - \| Y - pM \|_2, \quad \text{and} \\
	\sigma_{r+1}(Y) &\le \sigma_{r+1}(pM) + \| Y - pM \|_2 = \| Y - pM \|_2.
\end{align*}
This completes the proof. 
\end{proof}


\subsection{Key Lemma for Theorem \ref{thm:main_MRLE}}\label{sec:proof_key_lemma}
Here we present a preliminary version of Theorem \ref{thm:main_MRLE}. This is a deterministic statement assuming 
a certain set of conditions. We prove Theorem \ref{thm:main_MRLE} in Appendix \ref{sec:proof_main} based on this key lemma.
\begin{theorem}\label{thm:preliminary_MRLE}
Given $Y \in \Reals^{N \times d}$ and $t^* \geq 0$, let $\widehat {M}= \frac{1}{\hat{p}}\text{HSVT}_{t^*}(Y)$ and 
let $r = \text{rank}(M)$. Suppose %that 
\begin{enumerate}
	\item $\big\| Y - p M \big\|_2 \leq \Delta $ for some $\Delta \geq 0$,
	\item $p > \frac{\Delta}{\sigma_r(M)}$,
	\item $ \frac{1}{\varepsilon} p \leq \hat{p} \leq \varepsilon p$ for some $\varepsilon \geq 1$, and
	\item $t^* $ satisfies $\Delta < t^* < p \sigma_r(M) - \Delta$.
\end{enumerate}
Then for every $i \in [N]$,
\begin{align*}
	\Big\| \widehat{M}^i - M^i \Big\|_2^2 
		&\leq \frac{2 \varepsilon^2}{p^2} \left\| \varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) \right\|_2^2
		+ 2 ( \varepsilon - 1 )^2\left\| \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) \right\|_2^2
			+ \left( \frac{\Delta}{ p \sigma_r(M) - \Delta} \right)^2 \big\| M^i \big\|_2^2.
\end{align*}
\end{theorem}

\begin{proof}
We present the proof in three steps.
\paragraph{Step 1: Decomposition of $\widehat{M}^i - M^i$.}
Fix a row index $i \in [N]$. Observe that
\begin{equation*}
	\widehat{M}^i - M^i
		= \Big( \widehat{M}^i - \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) \Big) 
			+ \Big( \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) - M^i \Big).
\end{equation*}
Note that assumption 4 implies $\text{rank}(\widehat{M}) = \text{rank}(M)$ by Lemma \ref{lemma:thresholding_rank}. 
By definition (cf. \eqref{eq:hardsvt.1}), we have that $\varphi_{Y;t^*}^{\text{hard}}: \Reals^d \to \Reals^d$ is 
the projection onto the span of the top $r$ right singular vectors of $Y$.

Let $v^M_1, \ldots, v^M_r$ and $v^Y_1, \ldots, v^Y_r$ denote the top $r$ right singular vectors of $M$ and $Y$, respectively. 
Given a subspace $V \subset \Reals^d$, we let $\mathcal{P}_V: \Reals^d \to V$ denote the projection operation onto $V$. Then 
\[
	\widehat{M}^i - \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big)
		=  \varphi_{Y;t^*}^{\text{hard}} \bigg( \frac{1}{\hat{p}} Y^i -  M^i \bigg) 
		= \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y \} } \bigg( \frac{1}{\hat{p}} Y^i -  M^i \bigg) 
		\in \text{span}\{v_1^Y, \ldots, v_r^Y \}
\]
and
\[
	\varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) - M^i 
		= \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y \}} (M^i)  - M^i  \in \text{span}\{v_1^Y, \ldots, v_r^Y \}^{\perp}.
\]
Therefore, $\widehat{M}^i - \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big)$ is orthogonal to 
$\varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) - M^i $ and by Pythagorean theorem,
\begin{equation}\label{eqn:pythagorean}
	\big\| \widehat{M}^i - M^i \big\|_2^2
		=	\big\| \widehat{M}^i - \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) \big\|_2^2
			+ \big\| \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) - M^i \big\|_2^2.
\end{equation}
Now it remains to bound the two terms on the right hand side of \eqref{eqn:pythagorean}.
%
\paragraph{Step 2: Upper Bound on $\big\| \widehat{M}^i - \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) \big\|_2^2$.}
Next, we find an upper bound for the first term on the right hand side of \eqref{eqn:pythagorean}. Note that
\begin{align*}
	\widehat{M}^i - \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big)
		&= \varphi_{Y;t^*}^{\text{hard}} \bigg( \frac{1}{\hat{p}} Y^i -  M^i \bigg) \\
		&= \frac{1}{\hat{p}}\varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) 
			+ \frac{p - \hat{p}}{\hat{p}}\varphi_{Y;t^*}^{\text{hard}} \big( M^i \big).
\end{align*}
Applying Young's inequality for products (equivalently, by Cauchy-Schwarz inequality),
\begin{align}
	\big\| \widehat{M}^i - \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) \big\|_2^2
		&\leq 2 \left\| \frac{1}{\hat{p}}\varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) \right\|_2^2
			+ 2 \left\| \frac{p - \hat{p}}{\hat{p}}\varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) \right\|_2^2		\nonumber\\
		&\leq \frac{2}{\hat{p}^2} \left\| \varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) \right\|_2^2
			+ 2 \left(\frac{ p - \hat{p}}{\hat{p}} \right)^2 \left\| \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) \right\|_2^2	\nonumber\\
		&\leq \frac{2 \varepsilon^2}{p^2} \left\| \varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) \right\|_2^2
			+ 2 ( \varepsilon - 1 )^2\left\| \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) \right\|_2^2		\label{eqn:pythagorean.term.1}
\end{align}
because assumption 3 implies $\frac{1}{\hat{p}} \leq \frac{\varepsilon}{p}$ and 
$\left( \frac{p - \hat{p}}{\hat{p}} \right)^2 \leq (\varepsilon-1)^2$.
%
\paragraph{Step 3: Upper Bound on $\big\| \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) - M^i \big\|_2^2$.}
We now bound the second term on the right hand side of \eqref{eqn:pythagorean}. We apply the Davis-Kahan Sin $\Theta$ Theorem 
(see Theorem \ref{thm:DK_sin} in Appendix \ref{sec:DK_sin_theta}) to arrive at the following inequality:
\begin{align}
	\big\| \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y\}} - \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M\}} \big\|_2
		&\leq  \frac{\| Y - p M \|}{p \sigma_r(M) - \sigma_{r+1}(Y)}		\nonumber\\
		&\leq  \frac{\| Y - p M \|}{p \sigma_r(M) - \| Y - p M \|_2}		\qquad\because \sigma_{r+1}(Y) \leq \| Y - pM \|_2 \nonumber\\
		&\leq  \frac{\Delta}{ p \sigma_r(M) - \Delta}.		\label{eq:davis_kahan}
\end{align}
We utilized assumption 1 to bound $\| Y - pM \|_2 \leq \Delta$. Also, assumption 2 implies $p \sigma_r(M) - \sigma_{r+1}(M) > 0$ and 
ensures the validity of Davis-Kahan upper bound.

Now we observe that $ \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) = \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y\}} (M^i)$ 
and $M^i = \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \}} (M^i)$. Therefore, 
\begin{align}
	\big\| \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) - M^i \big\|_2^2
		&= \left\| \big(  \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y\}} 
			- \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M\}} \big) M^i  \right\|_2^2	\nonumber\\
		&\leq \left\| \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y\}} - \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M\}} \right\|_2^2
			\big\| M^i \big\|_2^2		\nonumber\\
		&\leq \left( \frac{\Delta}{ p \sigma_r(M) - \Delta} \right)^2 \big\| M^i \big\|_2^2.	\label{eqn:pythagorean.term.2}
\end{align}
The last inequality follows from \eqref{eq:davis_kahan}.
Inserting \eqref{eqn:pythagorean.term.1} and \eqref{eqn:pythagorean.term.2} back to \eqref{eqn:pythagorean} completes the proof.
\end{proof}


==> contents/Appx03_lemma_E1E2E3.tex <==
\section{Helper Lemmas for the Proof of Theorem \ref{thm:main_MRLE}: Conditioning Events}\label{sec:conditioning_lemmas_proof}

\subsection{Defining Three High-probability Events for Conditioning: $\cE_1, \cE_2, \cE_3$}\label{sec:conditioning_events}
We define the following three events for conditioning. The constant $c_3$ in the definition of $\cE_1$ is an absoulte constant\footnote{This constant will be described later in Lemma \ref{lem:noise_singular}}.
\begin{align}
	\mathcal{E}_1 &:= \bigg\{ \big\| Y - p M \big\|_2 \leq  
					\sqrt{ (1-p) \Lambda^2 + p \tau^2} \sqrt{Np}	\label{eqn:cE_1}\\
					&\qquad\qquad\qquad + c_1 (\Lambda + \tau K(p))
					\Big\{\sqrt{c_3 } \big[ (Nd)^{1/4} + (2N \log N)^{1/4} \big] \vee c_3 \big( \sqrt{d} + \sqrt{2 \log N} \big) \Big\},	
					\nonumber
	\\ \mathcal{E}_2&:= \Bigg\{ \Bigg(1 - 2 \sqrt{\frac{\log (Nd)}{ Nd p}}\Bigg) p \le \hat{p} 
					\le \Bigg(1 - 2 \sqrt{\frac{ \log (Nd)}{ Ndp}}\Bigg)^{-1} p \Bigg\},		
					\label{eqn:cE_2}
	\\ \mathcal{E}_3 &:= \Bigg\{ \max_{i \in [N]} \left\| \varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) \right\|_2^2 
					\leq  4 \max_{i \in [N]} \left\|  Y^i - p M^i  \right\|_{\phi_2}^2 \log ( 2d N^5)	\nonumber\\
				&\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad
					\times\left[ r + \left(  \frac{\| Y - p M \|_2}{p \sigma_r(M) - \| Y - p M \|_2} \right)^2 d \right]  \Bigg\}.
					\label{eqn:cE_3}
\end{align}
Note that $\Prob{\cE_1}, \Prob{\cE_2}, \Prob{\cE_3} = 1- 1/\mathsf{poly}(N,d)$, cf. Remarks \ref{rem:E1}, \ref{rem:E2}, \ref{rem:E3}.


%%% ======================================================================
%%%	E1 is a high-probability event
%%% ======================================================================

\subsection{Proof of $\Prob{\cE_1} = 1- 1/\mathsf{poly}(N,d)$ }\label{sec:lemma_E1}

Consider the data matrix $Y$ as the sum of scaled parameter matrix $pM$ and perturbation $Y - pM$. 
We show a high-probability upper bound on the spectral norm of the perturbation matrix. 
This upper bound implies that $\sqrt{Np}$ is the correct order of singular value thresholding.

\begin{lemma} \label{lem:noise_singular}
For every $t \geq 0$,
\begin{align*}
	\sigma_{1}(Y - pM) &\leq \Big\{ Np \Big[ (1-p) \big( \max_{i,j} M_{ij}^2 \big) + p \| X^1 \|_{\phi_2}^2 \Big]\\
		&\qquad+\big\| Y^1 - pM^1 \big\|_{\psi_2}^2
			\Big[ c_3 \sqrt{N} \big( \sqrt{d} + \sqrt{2 \log N} \big) \vee c_3^2 \big( \sqrt{d} + \sqrt{2 \log N} \big)^2 \Big] \Big\}^{1/2}
\end{align*}
with probability at least $1 - \frac{2}{N^4}$. Here, $c_3 = c_3(c_0) > 0$ is an absolute constant, which depends 
only on another absolute constant $c$\footnote{Though we do not specify what the value of $c$ is, it is an absolute 
constant that does not depend on other parameters. It is the same constant $c$ that appears in Bernstein's inequality; 
see Lemma \ref{lem:Bernstein}.}.
\end{lemma}

The proof is based on Matrix Chernoff bound for random matrices with independent sub-gaussian rows; see Lemma \ref{lem:corr_op} 
and Corollary \ref{cor:op_upper}.
\begin{proof}
Let $Z = Y - pM$. Observe that $Z$ is an $N \times d$ matrix whose rows $Z^i$ are independent, mean zero, 
sub-gaussian random vectors in $\Reals^d$ (see Appendix \ref{sec:missing_values}). 
Matrix Chernoff bound (cf. Corollary \ref{cor:op_upper}) yields for every $t \geq 0$,
\begin{align*}
	\sigma_{1}(Y - pM) &\leq \Big\{ \sigma_{1}\big( \Exp{(Y - pM)^T (Y - pM)} \big) \\
		&\qquad+ \max_{i \in [N]}\big\| Y^i - pM^i \big\|_{\psi_2}^2
		\Big[ c_3 \sqrt{N}(\sqrt{d} + t ) \vee c_3^2 (\sqrt{d} + t )^2 \Big] \Big\}^{1/2}
\end{align*}
with probability at least $1 - 2 \cdot 9^{-t^2}$.

By Lemma \ref{lem:cov_Y},
\begin{align*}
	 \Exp{(Y - pM)^T (Y - pM)}	
	 	&= p(1-p) diag\big(M^T M \big)	+ p^2 \Exp{ \big(X - M \big)^T \big(X - M \big) }.
\end{align*}
Therefore,
\begin{align*}
	&\sigma_{1}\big( \Exp{(Y - pM)^T (Y - pM) } \big)\\
	&\qquad\leq p(1-p) \sigma_1 \Big( diag\big(M^T M \big)\Big)	+p^2 \sigma_1 \Big( \Exp{ \big(X - M \big)^T \big(X - M \big) } \Big)\\
	&\qquad\leq p(1-p) \max_{j \in [d]} \bigg( \sum_{i=1}^N M_{ij }^2 \bigg) 	+ p^2 \sum_{i=1}^N \sigma_1 \Big( \Exp{ \big(X^i - M^i \big)^T \big(X^i - M^i \big) } \Big)  \\
	&\qquad\leq Np \Big[ (1-p) \Big( \max_{i,j} M_{ij}^2 \Big) + p \| X^i \|_{\phi_2}^2 \Big]. 
\end{align*}
The last inequality follows from Lemma \ref{lem:tail_to_variance};
$\Big\| \Exp{ \big(X^i - M^i \big)^T \big(X^i - M^i \Big) } \Big\|_2 \leq \| X^i \|_{\phi_2}^2$. 
Choosing $t = \sqrt{2 \log N}$ completes the proof as $9^{-t^2} = \big( e^{2 \ln 3}\big)^{-2 \log N} 
= \big(\frac{1}{N^4}\big)^{\ln 3} \leq \frac{1}{N^4}$ for all $N \geq 1$.

\end{proof}



%with probability at least $1 - 2 \exp(-Np^2)$:
%\begin{align}
%	&\sigma_{1}\left( Y - pM \right)	\nonumber\\
%		&\leq 	\bigg\{ N \big\| \Sigma_Y(p) \big\|_2
%			+ 2 c_1 C_2 Np \left(  \tau + \Lambda K(p) \right)^2  \bigg\}^{1/2}.
%		\label{eqn:smax_upper}
%\end{align}

\begin{corollary}\label{cor:Z_spectral}
	Suppose that Conditions \ref{cond:bounded} and \ref{cond:subgaussian} hold. 
	Then for given $p \in [0,1]$,
	\begin{align*}
		\sigma_{1}(Y - pM) 
			&\leq \sqrt{ (1-p) \Lambda^2 + p \tau^2} \sqrt{Np}\\
				&\qquad + c_1 (\Lambda + \tau K(p))
					\Big\{\sqrt{c_3} \big[ (Nd)^{1/4} + (2N \log N)^{1/4} \big] \vee c_3 \big( \sqrt{d} + \sqrt{2 \log N} \big) \Big\}
	\end{align*}
	with probability at least $1 - \frac{2}{N^4}$. Here, $c_3 = c_3(c_0) > 0$ is the same constant as in 
	Lemma \ref{lem:noise_singular}.
\end{corollary}

\begin{proof}
First of all, we utilize a simple inequality: for $a, b > 0$, $\sqrt{a + b} \leq \sqrt{a} + \sqrt{b}$. 
When Conditions \ref{cond:bounded} holds, $\max_{i,j} \big| M_{ij} \big| \leq \Lambda$ and 
$\big\| Y^1 - pM^1 \big\|_{\psi_2} \leq c_1 (\Lambda + \tau K(p))$ by Proposition \ref{prop:subG_Z}.
\end{proof}

\begin{remark}\label{rem:E1}
Suppose that Conditions \ref{cond:bounded} and \ref{cond:subgaussian} hold. Then
\[	\Prob{\cE_1^c} \leq \frac{2}{N^4}	\]
follows as an immediate consequence of Corollary \ref{cor:Z_spectral}.
\end{remark}
%%% ======================================================================
%%%	E2 is a high-probability event
%%% ======================================================================

\subsection{Proof of $\Prob{\cE_2} = 1- 1/\mathsf{poly}(N,d)$}\label{sec:lemma_E2}

When $N, d \gg 1$, we may identify $\hat{p}$ with $p$. The exact statement of this claim is as follows.
%\begin{lemma}\label{lem:conc_p}
%	The fraction of observed entries, $\hat{p}$, concentrates to the sampling probability $p$. 
%	Specifically, for any $\eta > 0$,
%	\begin{equation}\label{eqn:binomial}
%		\Prob{\cE_1(\eta)^c} \leq 2  \exp \left( - \frac{ 3\eta^2}{2(\eta+3)}Nd p \right).
%	\end{equation}
%\end{lemma}
%\begin{proof}
%	By Bernstein's inequality, for any $t \geq 0$,
%	\[	\Prob{|\hat{p} - p | > t}	\leq 2 \exp \left( - \frac{ 3Ndt^2}{6p(1-p) + 2t} \right).	\]
%	Therefore,
%	\begin{align*}
%		\Prob{|\hat{p} - p | > \eta p}	&\leq 2 \exp \left( - \frac{ 3Nd \eta^2p^2}{6p(1-p) + 2 \eta p} \right)\\
%			&=		2 \exp \left( - \frac{ 3Nd \eta^2p^2}{(2\eta+6)p - 6p^2} \right)\\
%			&\leq 	2 \exp \left( - \frac{ 3\eta^2}{2(\eta+3)}Nd p \right).
%	\end{align*} 
%\end{proof}
%
%We may assume $0 < \eta \leq 1$. Then the right hand side of \eqref{eqn:binomial} is bounded above by 
%$2 \exp \left( - \frac{3\eta^2}{8} Ndp \right)$. We need $\eta = \Omega \left( \frac{\log N + \log d}{\sqrt{Ndp}} \right)$ 
%to make this probability decay no slower than a polynomial rate of $N, d$ as $N, d \to \infty$.

\begin{lemma}\label{lemma:replace_p_hat_with_p}
	For any $\varepsilon > 1$,
	\begin{align*}
		\Prob{  \frac{1}{\varepsilon} p \le \hat{p} \le \varepsilon p } 
			\geq 1 - 2 \exp \left( - \frac{(\varepsilon - 1)^2}{2 \varepsilon^2} Ndp \right).
	\end{align*}
\end{lemma}
\begin{proof}
	Recall that we assumed observations made through i.i.d. Bernoulli mask with parameter $p \in (0,1]$ 
	and that we define $\hat{p}$ as
	\[	\hat{p} = \frac{1}{Nd} \sum_{i=1}^{N} \sum_{j=1}^d \Ind{ Y_{ij} \text{ observed}} \vee \frac{1}{Nd}.	\]
	By the binomial Chernoff bound, for $\varepsilon > 1$,
	\begin{align*}
		\Prob{ \hat{p} > \varepsilon p }
			&\leq \exp\left( - \frac{(\varepsilon - 1 )^2}{\varepsilon + 1} Ndp \right),	\quad\text{and}\\
		\Prob{ \hat{p} < \frac{1}{\varepsilon} p  }
			&\leq \exp \left( - \frac{(\varepsilon - 1)^2}{2 \varepsilon^2} Ndp \right).
	\end{align*}
	By the union bound,
	\[
		\Prob{  \frac{1}{\varepsilon} p \le \hat{p} \le \varepsilon p }
			\geq 1 - \Prob{ \hat{p} > \varepsilon p } -  \Prob{ \hat{p} < \frac{1}{\varepsilon} p  }.
	\]
	Noticing $\varepsilon + 1 < 2 \varepsilon < 2 \varepsilon^2$ for all $\varepsilon > 1$ completes the proof.
\end{proof}

\begin{remark}\label{rem:E2}
By choosing $\varepsilon = \bigg(1 - 2 \sqrt{\frac{\log (Nd)}{ Ndp}}\bigg)^{-1} $ in Lemma \ref{lemma:replace_p_hat_with_p},
it follows that
\[	\Prob{\cE_2^c} \leq \frac{2}{N^2d^2}.	\]
\end{remark}


%%% ======================================================================
%%%	E3 is a high-probability event
%%% ======================================================================

\subsection{Proof of $\Prob{\cE_3} = 1- 1/\mathsf{poly}(N,d)$}\label{sec:lemma_E3}

\subsubsection{Helper Lemma: Typical $\ell_2$ Norm of a Sub-gaussian Random Vector}
\begin{lemma}\label{lem:subg_projection}
	Let $X \in \Reals^d$ be a sub-gaussian random vector with $\| X \|_{\phi_2} < \infty$. 
	Let $V \in \Reals^{d \times r}$ be a matrix with orthogonal columns. $V$ is allowed to be random as long as it is independent of $X$. 
	Then for any $s > 0$,
	\[	\Prob{ \| VV^T X \|_2^2 > s }	\leq 2r \exp \left( - \frac{s}{2r \|  X \|_{\phi_2}^2 } \right).	\]
\end{lemma}
\begin{proof}
	Observe that $ \| VV^T X \|_2^2 = X^T VV^T X = \sum_{j=1}^r X^T V_j V_j^T X$ where $V_j$ denotes the $j$-th column of $V$.
	Now observe that for any $s > 0$, 
	\begin{align*}
		X^T VV^T X > s		\quad\text{implies that}\quad
				&\exists j \in [r]	\quad\text{s.t.}\quad		X^T V_j V_j^T X > \frac{s}{r}.
	\end{align*}
	This observation leads to the following inequality by applying the union bound:
	\begin{align*}
		\Prob{ X^T VV^T X > s	}	&\leq \sum_{j=1}^r \Prob{X^T V_j V_j^T X > \frac{s}{r}}.
	\end{align*}

	It remains to find an upper bound for
	\begin{align*}
		\Prob{X^T V_j V_j^T X > \frac{s}{r}}
			&= 	\Prob{ V_j^T X > \sqrt{\frac{s}{r}} } + \Prob{ V_j^T X < - \sqrt{\frac{s}{r}} }.
	\end{align*}
	By Markov's inequality (Chernoff bound) and the definition of $\| \cdot \|_{\phi_2}$ (see Definition \ref{defn:phi2}), 
	for any $\lambda > 0$,
	\begin{align*}
		\Prob{ V_j^T X > \sqrt{\frac{s}{r}} }
			&\leq		\Exp{ \exp\left( \lambda   V_j^T X   \right) } \exp\left(- \lambda \sqrt{\frac{s}{r}} \right)\\
			&\leq		\Exp{\Exp{ \exp\left( \lambda   V_j^T X   \right) ~ \big| ~ V }} \exp\left(- \lambda \sqrt{\frac{s}{r}} \right)\\
			&\leq 	\Exp{ \exp\left( \frac{\lambda^2 \|  V_j^T X  \|_{\phi_2}^2}{2} \right) } \exp\left(- \lambda \sqrt{\frac{s}{r}} \right)\\
			&\leq 	\exp\left( \frac{\lambda^2 \|  X  \|_{\phi_2}^2}{2} \right) \exp\left(- \lambda \sqrt{\frac{s}{r}} \right).
	\end{align*}
	Optimizing over $\lambda > 0$ (observe that $-\lambda a + \frac{\lambda^2}{2b}$ is minimized to $- \frac{a^2 b}{2}$ with $\lambda = ab$),
	\begin{align*}
		\Prob{  V_j^T X   > \sqrt{\frac{s}{r}}  }
			&\leq \exp \left( - \frac{s}{2r \|  X \|_{\phi_2}^2 } \right).
	\end{align*}
	We obtain the same upper bound on $\Prob{  V_j^T X  < - \sqrt{\frac{s}{r}}  }$.
	
	All in all,
	\[	\Prob{ X^T VV^T X > s	}	\leq 2r \exp \left( - \frac{s}{2r \| X \|_{\phi_2}^2 } \right).	\]
\end{proof}


\subsubsection{High-probability Upper Bound on $\big\| \varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) \big\|_2^2$}

We want a high probability upper bound on $ \big|\varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) \big\|_2^2 $, 
which is essentially the squared $\ell_2$ norm of a projection of sub-gaussian random vector projected onto the subspace 
spanned by top-$r$ right singular vectors of $Y$. We know that the $\ell_2$-norm of a sub-gaussian random vector 
projected onto a fixed $r$-dimensional subspace is of order $\tilde{O}(\sqrt{r})$ with high probability. However, there is 
an additional complication in analyzing $ \big\|\varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) \big\|_2^2 $ 
because the subspace (=span of top $r$ right singular vectors of $Y$) is dependent on the vector (=the $i$-th row of 
$Y - pM$) to take projection. 


\begin{lemma}\label{lem:ell2_upper}
Suppose that $p > \frac{\| Y - pM \|_2}{\sigma_r(M)}$ and $\| Y - pM \|_2 < t^* < \sigma_r(M) - \| Y - pM \|_2$. Then for each $i \in [N]$,
\begin{align*}
	\left\| \varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2^2 
		&\leq 4\left\|  Y^i - p M^i  \right\|_{\phi_2}^2 \left[ r + \left(  \frac{\| Y - p M \|_2}{p \sigma_r(M) - \| Y - p M \|_2} \right)^2 d \right]\log ( 2d N^5)
\end{align*}
with probability at least $1 - \frac{2}{N^5}$.
\end{lemma}

\begin{proof}
Let $v_1^M, \ldots, v_r^M$ and $v_1^Y, \ldots, v_r^Y$ denote the top $r$ right singular vectors of $M$ and $Y$, respectively. Also, note that
\begin{align*}
	\varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) = \varphi_{M;0}^{\text{hard}} \big(  Y^i - p M^i \big) 
		+ \Big[ \varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) - \varphi_{M;0}^{\text{hard}} \big(  Y^i - p M^i \big) \Big].
\end{align*}

Then Young's inequality for products yields
\begin{align*}
	\left\| \varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) \right\|_2^2 
		&\leq 2\left\| \varphi_{M;0}^{\text{hard}} \big(  Y^i - p M^i \big) \right\|_2^2
		+ 2 \left\| \varphi_{Y;t^*}^{\text{hard}} \big(  Y^i - p M^i \big) - \varphi_{M;0}^{\text{hard}} \big(  Y^i - p M^i \big) \right\|_2^2	\nonumber\\
		&= 2\left\| \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} } \big(  Y^i - p M^i \big) \right\|_2^2	\nonumber\\
			&\qquad+  2\left\|  \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y \} } \big(  Y^i - p M^i \big) - \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} } \big(  Y^i - p M^i \big) \right\|_2^2	\nonumber\\
		&\leq 2\left\| \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} } \big(  Y^i - p M^i \big) \right\|_2^2	\nonumber\\
			&\qquad+ 2\left\|  \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y \} } - \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} }\right\|_2^2 
			\big\|  Y^i - p M^i \big\|_2^2.	%\label{eqn:young}
\end{align*}
Next, it follows from Davis-Kahan Sin $\Theta$ theorem (see \eqref{eq:davis_kahan}) that
\begin{align*}
	\big\| \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y\}} - \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M\}} \big\|_2
		&\leq  \frac{\| Y - p M \|_2}{p \sigma_r(M) - \| Y - p M \|_2}.
\end{align*}
Lastly, by applying Lemma \ref{lem:subg_projection}, we observe that for any $s_1, s_2 > 0$,
\begin{align*}
	&\Prob{\left\| \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} } \big(  Y^i - p M^i \big) \right\|_2^2 > s_1}
		\leq 2 r \exp \bigg( - \frac{s_1}{2r \left\|  Y^i - p M^i  \right\|_{\phi_2}^2} \bigg),\\
	&\Prob{\left\|  Y^i - p M^i \right\|_2^2 > s_2}
		\leq 2 d \exp \bigg( - \frac{s_2}{2d \left\|  Y^i - p M^i  \right\|_{\phi_2}^2} \bigg).
\end{align*}
Choose $s_1 = 2r \left\|  Y^i - p M^i  \right\|_{\phi_2}^2 \log ( 2r N^5)$ and 
$s_2 = 2d \left\|  Y^i - p M^i  \right\|_{\phi_2}^2 \log ( 2d N^5)$ to complete the proof.
\end{proof}


\begin{remark}\label{rem:E3}
Suppose that $p > \frac{\| Y - pM \|_2}{\sigma_r(M)}$ and $\| Y - pM \|_2 < t^* < \sigma_r(M) - \| Y - pM \|_2$. Then 
	\[	\Prob{\cE_3^c} \leq \frac{2}{N^4}	\]
follows as a corollary of Lemma \ref{lem:ell2_upper} by taking union bounds over $i \in [N]$.
\end{remark}






==> contents/Appx04_proof_main_theorem.tex <==
%%% ======================================================================
%%%	Proof of Theorems
%%% ======================================================================

\section{Proof of Theorem \ref{thm:main_MRLE}}\label{sec:proof_main}
In this section we conclude the proof of Theorem \ref{thm:main_MRLE} that is the first main theorem of this paper. 
The proof is built based on the Key Lemma for the theorem --Theorem \ref{thm:preliminary_MRLE}. Combining 
the Key Lemma with the three conditioning events defined in Appendix \ref{sec:conditioning_events} yields 
the desired conclusion of Theorem \ref{thm:main_MRLE}. Equipped with two simple probabilistic tricks to be 
described in \ref{sec:frequent_technique},we complete the proof of Theorem \ref{thm:main_MRLE} in \ref{sec:proof_main}.

\subsection{Helpful Probabilistic Techniques for the Proof of Theorem \ref{thm:main_MRLE}}\label{sec:frequent_technique}
Many of our theorems and lemmas are about establishing deviation inequalities of the following form: 
given a function $f$ of the data matrix $Y$ and the (hidden) parameter matrix $M$, there exists $g: \Reals_+ \to \Reals_+$ 
such that 
\[	\Prob{f(Y, M) > t} \leq g(t) .	\]
The following two techniques are frequently used in the proof of our theorems and lemmas.

\begin{itemize}
	\item
	{\bf Union Bound. }Suppose that there exist $f_1, f_2$ such that $f(Y,M) \leq f_1(Y,M) + f_2(Y,M)$. 
	For any $t_1, t_2 > 0$, ``$f_1(Y,M) \leq t_1$ and $f_2(Y,M) \leq t_2$'' implies ``$f(Y,M) \leq t_1 + t_2$.'' 
	The contraposition of this statement yields
	\begin{align*}
		\Prob{ f(Y,M) > t_1 + t_2 } &\leq \Prob{ f_1(Y,M) > t_1 \text{ or }f_2(Y,M) > t_2 }\\
			&\leq \Prob{ f_1(Y,M) > t_1 } + \Prob{ f_2(Y,M) > t_2 }.
	\end{align*} 
	\item
	{\bf The Law of Total Probability. }
	For any two events $E_0, E_1$, we have $\Prob{E_0} = \Prob{E_0|E_1}\Prob{E_1} +  \Prob{E_0|E_1^c}\Prob{E_1^c}$. 
	.Let $E_0$ denote the event of our interest, and $E_1$ be an auxiliary event for conditioning. Since probability takes value in $[0,1]$, 
	\[	\Prob{E_0} \leq \Prob{E_0 | E_1} + \Prob{E_1^c}.	\]
\end{itemize}


\subsection{Proof of Theorem \ref{thm:main_MRLE}}\label{sec:proof_main}
We prove Theorem \ref{thm:main_MRLE} by combining Theorem \ref{thm:preliminary_MRLE} with Remarks \ref{rem:E1}, 
\ref{rem:E2}, \ref{rem:E3}.
\begin{proof}
%Recall that we define
%\begin{align*}
%	&\Phi(N,d; p, \tau, \Lambda)\\
%		&\triangleq 8 c_1^2 c_2^2 \Bigg( \frac{\sqrt{Ndp}}{\sqrt{Ndp} - 2 \sqrt{\log (Nd)}} \Bigg)^2 
%			\frac{\big(\tau + \Lambda K(p) \big)^2 }{p^2}
%			\left[ r + \left(  \frac{\Delta(N,d,p)}{p \sigma_r(M) - \Delta(N,d,p)} \right)^2 d \right]  \log ( 2d N^5)	\nonumber\\
%		&\quad	+ \left[ 2 \left( \frac{2\sqrt{\log(Nd)}}{\sqrt{Ndp} - 2\sqrt{\log(Nd)}} \right)^2
%			+ \left( \frac{\Delta(N,d,p)}{ p \sigma_r(M) - \Delta(N,d,p)} \right)^2 \right] \Lambda^2 d.
%\end{align*}
For any value $s > 0$, we have the following upper bound on $\Prob{ \max_{i \in [N]}\big\| \widehat{M}^i - M^i \big\|_2^2  > s  }$ 
by the law of total probability and the union bound:
\begin{align*}
	&\Prob{ \max_{i \in [N]}\big\| \widehat{M}^i - M^i \big\|_2^2  > s  } \\
	&\qquad\leq \Prob{ \max_{i \in [N]} \big\| \widehat{M}^i - M^i \big\|_2^2 > s  ~\big| ~ \cE_1 \cap \cE_2 \cap \cE_3 } 
			+ \Prob{\cE_1^c \cup \cE_2^c \cup \cE_3^c}\\
	&\qquad\leq \sum_{i = 1}^N  \Prob{ \big\| \widehat{M}^i - M^i \big\|_2^2> s  ~\big| ~ \cE_1 \cap \cE_2 \cap \cE_3 } 
			+ \Prob{\cE_1^c} + \Prob{\cE_2^c} + \Prob{\cE_3^c}.
\end{align*}
 
Conditioned on $\cE_1 \cap \cE_2 \cap \cE_3$, we can choose $\Delta = \Delta(N,d,p)$ (see definition of $\cE_1$ in \eqref{eqn:cE_1}) and 
$\varepsilon = \left( 1 - 2\sqrt{\frac{\log(Nd)}{Ndp}} \right)^{-1}$ (see definition of $\cE_2$ in \eqref{eqn:cE_2}). Also, we have an upper bound 
on $\big\| \varphi_{Y;t^*}^{\text{hard}} \big(Y^i - pM^i \big) \big\|_2^2$ (see definition of $\cE_3$ in \eqref{eqn:cE_3}). Note that 
$\max_{i \in [N]} \left\|  Y^i - p M^i  \right\|_{\phi_2} \leq c_1 c_2 \big( \tau + \Lambda K(p) )$ by Proposition \ref{prop:subG_Z}.

Moreover, we observe that
\[	\left\| \varphi_{Y;t^*}^{\text{hard}} \big( M^i \big) \right\|_2^2	\leq \big\| M^i \big\|_2^2 \leq d \Lambda^2.	\]
by the contraction property of $\varphi^{\text{hard}}_{Y;t^*}$ (see Lemma \ref{lem:contraction}) and Condition \ref{cond:bounded} 
(boundedness of $M$).

Based on these observations, we choose\footnote{Assuming $p \geq \frac{16 \log(Nd)}{Nd}$, $1 - 2\sqrt{\frac{\log(Nd)}{Ndp}} \geq \frac{1}{2}$ and 
$\left( 1 - 2\sqrt{\frac{\log(Nd)}{Ndp}} \right)^{-1} \leq 2$.}
\begin{align*}
	s
		&=
		\frac{2 }{p^2}  \left( 1 - 2\sqrt{\frac{\log(Nd)}{Ndp}} \right)^{-2} \\
			&\qquad\qquad\qquad\times
			4 \big[ c_1 c_2 \big( \tau + \Lambda K(p) ) \big]^2 \log ( 2d N^5)
			\left[ r + \left(  \frac{ \Delta(N,d,p) }{p \sigma_r(M) - \Delta(N,d,p) } \right)^2 d \right] \\
		&
		\quad+ 2 \Bigg( \left( 1 - 2\sqrt{\frac{\log(Nd)}{Ndp}} \right)^{-1} - 1 \Bigg)^2 d \Lambda^2
			+ \left( \frac{\Delta(N,d,p)}{ p \sigma_r(M) - \Delta(N,d,p)} \right)^2 d \Lambda^2\\
		&=\frac{32 c_1^2 c_2^2 \big(\tau + \Lambda K(p) \big)^2 }{p^2} 
			\left[ r + \left(  \frac{ \Delta(N,d,p) }{p \sigma_r(M) - \Delta(N,d,p) } \right)^2 d \right] \log ( 2d N^5) \\
		&
		\quad+ \left[ 2 \left( \frac{2\sqrt{\log(Nd)}}{\sqrt{Ndp} - 2\sqrt{\log(Nd)}} \right)^2  + \left( \frac{\Delta(N,d,p)}{ p \sigma_r(M) - \Delta(N,d,p)} \right)^2 \right] d \Lambda^2.
\end{align*}

By Theorem \ref{thm:preliminary_MRLE}, $ \Prob{ \big\| \widehat{M}^i - M^i \big\|_2^2> s  ~\big| ~ \cE_1 \cap \cE_2 \cap \cE_3 } = 0$. 
The proof is complete.
\end{proof}


==> contents/Appx05_proof_matrix_corollary.tex <==
%%% ======================================================================
%%%	Proof in Mixture Section
%%% ======================================================================
\section{Proof of Corollary \ref{cor:matrix_estimation}}\label{sec:proof_matrix}

\begin{proof}
	We let $C > 0$ denote a sufficiently large constant. The exact value $C$ represents will change from line to line in the proof, 
	but it is an absolute constant, independent of parameters $N, d, p$, etc. 
	
	To begin with, we make the following observations.
	\paragraph{Step 1. Trimming using $p \geq \frac{16 \log(Nd)}{Nr}$ assumption.}
	Recall we assume that $p \geq \frac{16 \log(Nd)}{Nr}$ in Theorem \ref{thm:main_MRLE}.
	Therefore $\sqrt{Ndp} \geq 4 \sqrt{ \frac{d \log(Nd)}{r}}$ and it follows that
	\begin{align}
		\frac{\sqrt{Ndp}}{\sqrt{Ndp} - 2 \sqrt{\log (Nd)}} &= \frac{1}{1 - \frac{2 \sqrt{\log(Nd)}}{\sqrt{Ndp}}}
			\leq \frac{1}{1 - \frac{\sqrt{r}}{2\sqrt{d}}} \leq 2,	\label{eqn:coro_ME_obs.1}\\
		\frac{ 2 \sqrt{\log (Nd)}}{\sqrt{Ndp} - 2 \sqrt{\log (Nd)}} &\leq \frac{ 2 \sqrt{\log (Nd)}}{ 4 \sqrt{ \frac{d \log(Nd)}{r}} - 2 \sqrt{\log (Nd)}}
			= \frac{\sqrt{r}}{2 \sqrt{d} - \sqrt{r}} \leq \sqrt{\frac{r}{d}}.	\label{eqn:coro_ME_obs.2}
	\end{align} 
	
	\paragraph{Step 2: Ensuring \eqref{eqn:p_lower_cor.1} is sufficient for $p \sigma_r(M) \geq 2 \Delta(N,d,p)$.} 
	Next, we show that if $p$ satisfies the lower bound stated in \eqref{eqn:p_lower_cor.1}, i.e., if 
	\begin{equation}\label{eqn:p_necessary}
		p \geq C\left\{  (\tau + \Lambda)^2 \frac{r}{d} +  (\tau + \Lambda)  \bigg[ \frac{\sqrt{r}}{(Nd)^{1/4}} + \sqrt{\frac{r}{N}} \bigg]\right\}
	\end{equation}
	for sufficiently large $C > 0$, then $p \sigma_r(M) \geq 2 \Delta(N,d,p)$. This leads to 
	\begin{equation}\label{eqn:coro_ME_obs.3}
		\frac{\Delta(N,d,p)}{p \sigma_r(M) - \Delta(N,d,p)} \leq \frac{2 \Delta(N,d,p)}{p \sigma_r(M)}
	\end{equation}
	
	First, recall from \eqref{eqn:Delta_upper} that $\Delta(N,d,p) \leq C (\tau + \Lambda) \big[ \sqrt{Np} + (Nd)^{1/4} + \sqrt{d} \big]$ 
	for some large constant $C > 0$. 
%	\begin{align*}
%	\Delta(N,d,p) 
%%			&\triangleq \sqrt{ (1-p) \Lambda^2 + p \tau^2} \sqrt{Np}	\nonumber\\
%%			&\quad + c_1 (\Lambda + \tau K(p))
%%			\Big\{\sqrt{c_3 } \big[ (Nd)^{1/4} + (2N \log N)^{1/4} \big] \vee c_3 \big( \sqrt{d} + \sqrt{2 \log N} \big)\\
%			&\leq C (\tau + \Lambda) \big[ \sqrt{Np} + (Nd)^{1/4} + \sqrt{d} \big]
%	\end{align*}
%	for some large constant $C > 0$. 
	Then we observe that $p \sigma_r(M) \geq 2 \Delta(N,d,p)$ if and only if $p \geq \frac{2 \Delta(N,d,p)}{ \sigma_r(M) }$. 	
	Since we assumed $\sigma_r(M) \geq c \sqrt{\frac{Nd}{r}}$ for some $c > 0$ (i.e., $M$ is `well-behaved'), it follows that 
	\begin{align}
		\frac{2 \Delta(N,d,p)}{ \sigma_r(M) }
			&\leq C(\tau + \Lambda) \sqrt{\frac{r}{Nd}} \big(\sqrt{Np} + (Nd)^{1/4} + \sqrt{d} \big)		\nonumber\\
			&\leq C(\tau + \Lambda) \Big( \sqrt{\frac{rp}{d}} + \frac{r^{1/2}}{(Nd)^{1/4}} + \sqrt{\frac{r}{N}} \Big)	\label{eqn:upper_ratio}
	\end{align}
	because $N = \mathsf{poly}(d)$ ensures $(2N \log N)^{1/4} \leq C (Nd)^{1/4}$ and $\sqrt{2 \log N} \leq \sqrt{d}$.
	
	If $p \geq C' (\tau + \Lambda) \sqrt{\frac{Np}{d}}$ and $p \geq C' (\tau + \Lambda) \Big(\frac{r^{1/2}}{(Nd)^{1/4}} 
	+ \sqrt{\frac{r}{N}} \Big)$, then $p \geq C' (\tau + \Lambda)\Big( \sqrt{\frac{rp}{d}} + \frac{r^{1/2}}{(Nd)^{1/4}} 
	+ \sqrt{\frac{r}{N}} \Big)$. By taking a sufficiently large $C'$, this lower bound on $p$ can be made bigger than 
	the upper bound on $\frac{2 \Delta(N,d,p)}{\sigma_r(M)}$ stated in \eqref{eqn:upper_ratio}.
	
	Observe that 
	\begin{align*}
		p \geq C(\tau + \Lambda) \sqrt{\frac{Np}{d}} \qquad&\text{if and only if}\qquad
		\sqrt{p} \geq C' (\tau + \Lambda) \sqrt{\frac{N}{d}}\\
		&\text{if and only if}\qquad p \geq C' (\tau + \Lambda)^2\frac{r}{d}.
	\end{align*}
	Therefore, if $p$ satisfies the lower bound in \eqref{eqn:p_lower_cor.1}, then $p \geq C' (\tau + \Lambda) \sqrt{\frac{Np}{d}}$. 
	Also, if $p$ satisfies the lower bound in \eqref{eqn:p_lower_cor.1}, it trivially satisfies $p \geq C' (\tau + \Lambda) 
	\Big(\frac{r^{1/2}}{(Nd)^{1/4}} + \sqrt{\frac{r}{N}} \Big)$.
	
	In conclusion, we can choose $C'$ in an adaptive manner to $C$ we need in \eqref{eqn:upper_ratio}. If $p$ satisfies 
	the lower bound in \eqref{eqn:p_lower_cor.1} for a large $C' > 0$ chosen in such a fashion, then 
	\[	p \geq C(\tau + \Lambda) \Big( \sqrt{\frac{rp}{d}} + \frac{r^{1/2}}{(Nd)^{1/4}} + \sqrt{\frac{r}{N}} \Big) \geq \frac{2 \Delta(N,d,p)}{\sigma_r(M)}. \]
	
	\paragraph{Step 3: Simplifying \eqref{eqn:maxell2_upper} based on Steps 1 and 2.}
	When $p$ satisfies the conditions for steps 1 and 2 (for sufficiently large $N$ and $d$), we obtain the following high-probability 
	bound\footnote{With probability at least $1 - \frac{4}{N^4} - \frac{2}{N^2d^2}$; see Theorem \ref{thm:main_MRLE}.} by combining 
	\eqref{eqn:coro_ME_obs.1}, \eqref{eqn:coro_ME_obs.2}, \eqref{eqn:coro_ME_obs.3} with \eqref{eqn:maxell2_upper} in 
	Theorem \ref{thm:main_MRLE}:	
	\begin{align}
	&\max_{i \in [N]} \Big\| \widehat{M}^i - M^i \Big\|_2^2		\nonumber\\
		&\leq C	\frac{\big(\tau + \Lambda K(p) \big)^2 }{p^2}	\left[ r +\frac{\Delta(N,d,p)^2}{4 p^2 \sigma_r(M)^2} d \right]  \log ( 2d N^5)
		+ \left[ \frac{2r}{d}	+  \frac{\Delta(N,d,p)^2}{4 p^2 \sigma_r(M)^2}  \right] \Lambda^2 d	\nonumber\\
		&\leq C	\frac{\big(\tau + \Lambda K(p) \big)^2 }{p^2}	\left[ r + C \frac{Np + \sqrt{Nd} + d }{4 p^2 \frac{Nd}{r}} d \right]  \log ( 2d N^5)
		+ \Lambda^2 \left[ 2r	+  C\frac{Np + \sqrt{Nd} + d}{4 p^2 \frac{Nd}{r}} d  \right]				\nonumber\\
%		&\leq C	\frac{\big(\tau + \Lambda K(p) \big)^2 r }{p^2}
%			\left[ 1 + C \frac{Np + \sqrt{Nd} + d }{4 p^2 N}  \right]  \log ( 2d N^5)					\nonumber\\
		&\leq C	\frac{\big(\tau + \Lambda K(p) \big)^2 r }{p^2}
			\left[ 1 + \frac{1}{p} + \frac{1}{p^2} \sqrt{\frac{d}{N}} + \frac{1}{p^2}\frac{d}{N} \right]  \log ( 2d N^5).	\label{eqn:coro_ME_simplified}
	\end{align}
\end{proof}



==> contents/Appx07_proof_mixture_corollary.tex <==
%%% ======================================================================
%%%	Proof of Mixture Corollary
%%% ======================================================================

\section{Proof of Corollary \ref{cor:mixture_clustering} and Corollary\ref{cor:mixture_clustering_p}}\label{sec:proof_coro_clustering}

\subsection{Proof of Corollary \ref{cor:mixture_clustering}}
\begin{proof}
We can obtain a label $\hat{\alpha}:[N] \to [k]$ that correctly groups (up to permutation) $\widehat{M}^i$'s 
based on the pairwise distance if
\begin{equation}\label{eqn:separation_condition}
	\sup_{i_1, i_2 \in [N] \atop \alpha(i_1) = \alpha(i_2)} \big\| \widehat{M}^{i_1} - \widehat{M}^{i_2} \big\|_2
		< \inf_{i_1, i_2 \in [N] \atop \alpha(i_1) = \alpha(i_2)} \big\| \widehat{M}^{i_1} - \widehat{M}^{i_2} \big\|_2. 
\end{equation}
Theorem \ref{thm:main_clustering} provides a sufficient condition\footnote{Recall that we simplified the bounds 
from \eqref{eqn:oversimple_1} to \eqref{eqn:oversimple_1}by multiplying $\sqrt{2 \log(2dN^5)}$ to the nominal term i
n the square bracket to obtain a readable form. Here, we undo that simplification for the purpose of proof.} 
to achieve such a separation as described in \eqref{eqn:separation_condition}.


Observe that \eqref{eqn:separation_condition} follows if
\begin{align}
	 \left( 1 - \frac{ \Delta(N,d,p) }{p \sigma_r(M) - \Delta(N,d,p) } \right) \Gamma 
	&> C \frac{ \big( \tau + \Lambda K(p) \big) \sqrt{ r \log(Nd) }}{p}	\nonumber\\
	&\qquad\times
	\left[ 1 + \frac{ C' d}{\sqrt{r}} \frac{  \tau + \Lambda K(p)  }{p \sigma_r(M) - 3 \Delta(N,d,p)}  \sqrt{\log(Nd)} \right] 	\label{eqn:sufficient_condition}
\end{align}
for absolute constants $C, C' > 0$ (more precisely, $C = 80 c_1 c_2$ and $C' = c_1 c_2$).

We assumed $p > \frac{3\Delta(N,d,p)}{\sigma_r(M)}$ and $M$ `well-behaved', hence, $\sigma_r(M) = \Theta\Big( \sqrt{\frac{Nd}{r}} \Big)$. 
Then we can rewrite \eqref{eqn:sufficient_condition} as
\begin{align*}
	\Gamma
		> C \frac{ \big( \tau + \Lambda K(p) \big) \sqrt{ r \log(Nd)}}{p}
			\left[ 1 + \frac{ C' d}{\sqrt{r}} \frac{  \tau + \Lambda K(p)  }{p \sigma_r(M) } \sqrt{\log(Nd)}  \right] ,
\end{align*}
for a sufficiently large $C > 0$ ($C'$ is still the same absolute constant).
From $\sigma_r(M) \geq c \sqrt{\frac{Nd}{r}}$, it follows that
\begin{equation}\label{eqn:minimum_gap}
	\Gamma
		> C \frac{ \big( \tau + \Lambda  \big) \sqrt{ r \log(Nd) }}{p}	\left( 1 +C'\frac{  \tau + \Lambda }{p }\sqrt{\frac{d}{N}} \sqrt{\log(Nd)}  \right).
\end{equation}
for sufficiently large $C, C' > 0$. 

Now suppose that $C_1 \frac{(\tau + \Lambda)^2}{p^2} d \log(d) \leq N \leq \mathsf{poly}(d)$ for some absolute constant $C_1$. Then
\[	C'\frac{\tau + \Lambda}{p}\sqrt{\frac{d}{N}} \leq C''	\qquad \text{and} \qquad \log(Nd) \leq C''' \log(d)		\]
for some $C'', C''' > 0$.

Then it suffices to have 
\begin{equation}\label{eqn:final.1}
	\Gamma > C  \frac{\tau + \Lambda}  {p} \sqrt{ r \log(d)}
\end{equation}\label{eqn:final.1}
for a sufficiently large $C > 0$ for $\Gamma$ to satisfy the condition stated in \eqref{eqn:minimum_gap}.
Note that $C$ in \eqref{eqn:final.1} depends on the absolute constant $C_1$.

\paragraph{Concluding the proof.}
Given that 
\begin{equation}\label{eqn:coro_assumptions}
\text{(i) }C_1 \frac{(\tau + \Lambda)^2}{p^2} d \log(d) \leq N \leq \mathsf{poly}(d) 
\qquad\text{and}\qquad 
\text{(ii) }\Gamma p > C_2(\tau + \Lambda) \sqrt{r \log(d)}
\end{equation}
where $C_2$ is chosen to satisfy $C_2 > C$ for the constant $C$ in \eqref{eqn:final.1}, the recovery condition \eqref{eqn:sufficient_condition} 
is satisfied. From the assumptions stated in \eqref{eqn:coro_assumptions}, it follows that 
\begin{align*}
	\sup_{i_1, i_2 \in [N] \atop \alpha(i_1) = \alpha(i_2)} \big\| \widehat{M}^{i_1} - \widehat{M}^{i_2} \big\|_2
		&\leq C \frac{ \big( \tau + \Lambda  \big) \sqrt{ r \log(Nd) }}{p}	\left( 1 +C'\frac{  \tau + \Lambda }{p }\sqrt{\frac{d}{N}}  \log(Nd)  \right) \\
		&= \Theta\Big( \frac{  \tau + \Lambda }{p}\sqrt{ r  \log(Nd)} \Big).
\end{align*}
\end{proof}


\subsection{Proof of Corollary \ref{cor:mixture_clustering_p}}
\begin{proof}
Now, we rewrite \eqref{eqn:minimum_gap} in the proof of Corollary \ref{cor:mixture_clustering} as an inequality for $p$:
\begin{equation}\label{eqn:minimum_gap_p}
	p
		> C (\tau + \Lambda)  \left( \frac{\sqrt{r}}{\Gamma} + \frac{r^{1/4} d^{1/4}}{\Gamma^{1/2} N^{1/4}} \right) \sqrt{\log(Nd)}.
\end{equation}
Given $\Gamma$, it is sufficient to have p satisfy \eqref{eqn:minimum_gap_p} for a sufficiently large $C > 0$ as long as 
$N \leq \mathsf{poly}(d)$.

%Recall from \eqref{eqn:p_necessary_analysis} that we need
%$p > C \left\{ (\tau + \Lambda)^2 \frac{r}{d} + (\tau + \Lambda) \left[ \frac{\sqrt{r}}{(Nd)^{1/4}} + \sqrt{\frac{r}{N}} \right] \right\}$ 
%for some large $C > 0$ to satisfy $p > \frac{\Delta(N,d,p)}{\sigma_r(M)}$. However, all the terms are dominated by terms in 
%\eqref{eqn:minimum_gap} because $\Gamma \leq O(\sqrt{d})$ due to Condition \ref{cond:bounded} (boundedness of $M$). 
%Therefore, \eqref{eqn:minimum_gap} sets the effective lower bound on $p$ that provides a sufficient condition in our analysis 
%for the success of distance-based clustering.

As a result, we can conclude that under the assumptions stated in Corollary \ref{cor:mixture_clustering}, there exists $d^*$ such that 
\[	\sup_{i_1, i_2 \in [N] \atop \alpha(i_1) = \alpha(i_2)} \big\| \widehat{M}^{i_1} - \widehat{M}^{i_2} \big\|_2
		< \inf_{i_1, i_2 \in [N] \atop \alpha(i_1) = \alpha(i_2)} \big\| \widehat{M}^{i_1} - \widehat{M}^{i_2} \big\|_2 	\]
%with $d^* = \Theta\Big( \frac{\tau + \Lambda}{p} \sqrt{r \log(d)}\Big)$, 
when conditioned on $\cE_1 \cap \cE_2 \cap \cE_3'$. 
Since $\Prob{\cE_1 \cap \cE_2 \cap \cE_3'} \geq 1 - \frac{4}{N^4} - \frac{2}{N^2d^2}$, the proof is complete.
\end{proof}

==> contents/Appx08_proof_mixture_theorem.tex <==
%%% ======================================================================
%%%	Proof for Mixture Main Theorem
%%% ======================================================================

\section{Effect of Preprocessing with HSVT on Sub-gaussian Mixture Problem}\label{sec:effect_ME_mixture}
In this section, we discuss the efficacy of matrix estimation (HSVT) as a model-agnostic data preprocessor. We argue in 
Theorem \ref{thm:ME_clustering} that $\widehat{M}$ output by the HSVT subroutine has sub-gaussian rows with new means, 
which is the projection of $Y^i$ onto the left singular space of $Y$ with singular values at least $t^*$ (scaled by $\frac{p}{\hat{p}}$) 
and the variance (actually $\psi_2$ norm) being amplified by $\frac{1}{p}$.

\begin{theorem}\label{thm:ME_clustering}
Suppose that Conditions \ref{cond:bounded} and \ref{cond:subgaussian} are satisfied. Given $Y \in \Reals^{N \times d}$ and 
$t^* \geq 0$, let $\widehat {M}= \frac{1}{\hat{p}}\text{HSVT}_{t^*}(Y)$. Suppose that (i) $p > \frac{\Delta(N,d,p)}{\sigma_r(M)}
\vee \frac{16 \log(Nd)}{Nd}$, and (ii) $t^* $ satisfies $\Delta(N,d,p) < t^* < p \sigma_r(M) - \Delta(N,d,p)$ where $r = \text{rank}(M)$.
Then with probability at least $1 - \frac{2}{N^2d^2}$, the following inequalities hold:
\begin{align*}
	&\forall i \in [N],
	&&\bigg\|  \widehat{M}^i - \frac{p}{\hat{p}}\varphi^{\text{hard}}_{Y; t^*} \big(\mu^{\alpha(i)} \big) \bigg\|_{\psi_2}
	\leq  c_1 \Bigg(1 - 2 \sqrt{\frac{\log (Nd)}{ Nd p}}\Bigg)^{-1} \Bigg(\frac{\tau_{\alpha(i)} + \Lambda K(p) }{p}\Bigg),\\
	&\forall a \neq b \in [k],
	&&\left\|  \frac{p}{\hat{p}} \varphi_{Y;t^*}^{\text{hard}} \big(  \mu^a - \mu^b \big) \right\|_2^2
	\geq \Bigg(1 - 2 \sqrt{\frac{\log (Nd)}{ Nd p}}\Bigg)^{2}\\
	&&&\qquad\qquad\qquad\qquad\qquad \times \left( 1 - \bigg( \frac{ \| Y - pM \|_2 }{p \sigma_r(M) - \| Y - pM \|_2 }\bigg)^2\right)
		\big\|  \mu^a - \mu^b \big\|_2^2.
\end{align*}
\end{theorem}

We make the following observation on Theorem \ref{thm:ME_clustering} that matrix estimation (HSVT in this case) imputes the 
missing values in observations at the cost of increasing the cluster variance by the factor of $\frac{1}{p}$. Remark \ref{rem:ME_preprocessing}
justifies the use of matrix estimation as a preprocessor.
\begin{remark}\label{rem:ME_preprocessing}
Note that when $p \gg \frac{\sqrt{\log(Nd)}}{Nd}$ and $p \gg \frac{\|Y - pM\|_2}{\sigma_r(M)}$, the conclusions of Theorem \ref{thm:ME_clustering} 
can be simplified as: for every $i \in [N]$ and for every $a, b \in [k]$,
\[	\bigg\|  \widehat{M}^i - \frac{p}{\hat{p}}\varphi^{\text{hard}}_{Y; t^*} \big(\mu^{\alpha(i)} \big) \bigg\|_{\psi_2} \leq  \frac{C(\tau_{\alpha(i)} + \Lambda K(p)}{p}
	\quad\text{and}\quad
	\left\|  \frac{p}{\hat{p}} \varphi_{Y;t^*}^{\text{hard}} \big(  \mu^a - \mu^b \big) \right\|_2^2 \geq C\big\|  \mu^a - \mu^b \big\|_2^2.
\]
That is, we may consider $\frac{p}{\hat{p}}\varphi^{\text{hard}}_{Y; t^*} \big(\mu^{\alpha(i)} \big)$ as the cluster means of the data 
processed by matrix estimation (HSVT, in this case). The transformed problem is a sub-gaussian mixture clustering problem with 
cluster means separated by constant times the original separation and cluster $\psi_2$ norm amplified by $\frac{1}{p} \times \text{constant}$.
\end{remark}




\begin{proof}
We prove the two conclusions one by one. The proof strategy is similar to that of Theorem \ref{thm:main_MRLE}. 
However, we only use $\cE_2$ for conditioning (instead of $\cE_1 \cap \cE_2 \cap \cE_3$) unlike in the proof of 
Theorem \ref{thm:main_MRLE}. Then it suffices to note $\Prob{\cE_2^c} \leq \frac{2}{N^2 d^2}$ so that we conclude 
the proof by the law of total probability.

\paragraph{Part 1: Sub-gaussianity.}
First, we recall that $\widehat{M}^i = HSVT_{t^*}(Y^i) = \frac{1}{\hat{p}}\varphi^{\text{hard}}_{Y;t^*}(Y^i)$. Then 
\begin{align*}
	\widehat{M}^i - \frac{p}{\hat{p}}\varphi^{\text{hard}}_{Y; t^*} \big(\mu^{\alpha(i)} \big)
		&= \frac{1}{\hat{p}} \varphi^{\text{hard}}_{Y; t^*} \big( Y^i - p \mu^{\alpha(i)} \big).
\end{align*}
Recall that when $ t^* $ is in the range, $\rank(\widehat{M}) = r$ by Lemma \ref{lemma:thresholding_rank}. 
Let $v_1^Y, \ldots, v_r^Y$ denote the top-$r$ right singular vectors of $Y$. Then we can rewrite the operator 
$\varphi_{Y;t^*}^{\text{hard}}$ as the sum of $r$ orthogonal projections:
\[	\varphi_{Y;t^*}^{\text{hard}} = \sum_{j=1}^r \cP_{v_j^Y}.	\]

By definition of $\psi_2$-norm,
\begin{align}
	\left\| \varphi^{\text{hard}}_{Y; t^*} \big( Y^i - p \mu^{\alpha(i)} \big) \right\|_{\psi_2}
		&= \left\| \varphi^{\text{hard}}_{Y; t^*} \big( Y^i - p \mu^{\alpha(i)} \big) \right\|_{\psi_2}	\nonumber\\
		&= \sup_{u \in \bbS^{d-1}} \left\| \varphi^{\text{hard}}_{Y; t^*} \big( Y^i - p \mu^{\alpha(i)} \big) u \right\|_{\psi_2}	\nonumber\\
		&= \sup_{u \in \cP_{\text{span}\{v_1^Y, \ldots, v_r^Y\}} \bbS^{d-1}} \left\| \big( Y^i - p \mu^{\alpha(i)} \big) u \right\|_{\psi_2}	\nonumber\\
		&\leq \sup_{u \in \bbS^{d-1}} \left\| \big( Y^i - p \mu^{\alpha(i)} \big) u \right\|_{\psi_2}	\nonumber\\
		&= \left\| Y^i - p \mu^{\alpha(i)} \right\|_{\psi_2}.	\label{eqn:mixture_subg.term.1}
\end{align}

Since we assumed Conditions \ref{cond:bounded} and \ref{cond:subgaussian} hold, it follows from 
Proposition \ref{prop:subG_Z} that
\begin{equation}\label{eqn:mixture_subg.term.2}
	\left\| Y^i - p \mu^{\alpha(i)} \right\|_{\psi_2} \leq c_1 \big( \tau_{\alpha(i)} + \Lambda K(p) \big).
\end{equation}
We apply the same conditioning argument as in the proof of Theorem \ref{thm:main_MRLE}. Conditioned on $\cE_2$,
\begin{equation}\label{eqn:mixture_subg.term.3}
	\frac{1}{\hat{p}} \leq  \Bigg(1 - 2 \sqrt{\frac{\log (Nd)}{ Nd p}}\Bigg)^{-1}\frac{1}{ p }.
\end{equation}
Putting \eqref{eqn:mixture_subg.term.1}, \eqref{eqn:mixture_subg.term.2}, \eqref{eqn:mixture_subg.term.3} together, we conclude
\begin{align*}
	\left\| \widehat{M}^i - \frac{p}{\hat{p}}\varphi^{\text{hard}}_{Y; t^*} \big(\mu^{\alpha(i)} \big) \right\|_{\psi_2}
		&= \frac{1}{\hat{p}}\left\| \varphi^{\text{hard}}_{Y; t^*} \big( Y^i - p \mu^{\alpha(i)} \big) \right\|_{\psi_2}\\
		&\leq \frac{1}{\hat{p}} \left\| Y^i - p \mu^{\alpha(i)} \right\|_{\psi_2}\\
		&\leq \frac{c_1}{ p }\Bigg(1 - 2 \sqrt{\frac{\log (Nd)}{ Nd p}}\Bigg)^{-1} \big( \tau_{\alpha(i)} + \Lambda K(p) \big).
\end{align*}


\paragraph{Part 2: Mean separation after HSVT.}
Let $v_1^M, \ldots, v_r^M$ denote the top-$r$ right singular vectors of $M$. Then we observe that 
$\mu^a - \mu^b \in \text{span}\{ v_1^M, \ldots, v_r^M\}$. Therefore, 
\[	\cP_{\text{span}\{v_1^M, \ldots, v_r^M\}} \big(  \mu^a - \mu^b \big) =  \mu^a - \mu^b.	\]
Recall that when $ t^* $ is in the range, $\rank(\widehat{M}) = r$ by Lemma \ref{lemma:thresholding_rank}.
Therefore, $\varphi_{Y;t^*}^{\text{hard}} \big(  \mu^a - \mu^b \big) = \cP_{\text{span}\{v_1^Y, \ldots, v_r^Y\}}\big(  \mu^a - \mu^b \big)$, 
and by Pythagorean theorem,
\begin{align}
	\left\| \varphi_{Y;t^*}^{\text{hard}} \big(  \mu^a - \mu^b \big) \right\|_2^2
		&= \big\|  \mu^a - \mu^b \big\|_2^2 - \left\| \cP_{\text{span}\{v_1^Y, \ldots, v_r^Y\}}\big(  \mu^a - \mu^b \big) 
			- \big(  \mu^a - \mu^b \big) \right\|_2^2		\nonumber\\
		&= \big\|  \mu^a - \mu^b \big\|_2^2 - \left\| \Big( \cP_{\text{span}\{v_1^Y, \ldots, v_r^Y\}}\big(  \mu^a - \mu^b \big) 
			- \cP_{\text{span}\{v_1^M, \ldots, v_r^M\}} \Big) \big(  \mu^a - \mu^b \big) \right\|_2^2		\nonumber\\
		&\geq \left( 1 - \bigg( \frac{ \| Y - pM \|_2 }{p \sigma_r(M) - \| Y - pM \|_2 }\bigg)^2\right)
			\big\|  \mu^a - \mu^b \big\|_2^2.	\label{eqn:mixture_subg.term.4}
\end{align}
Recall that when conditioned on $\cE_2$,
\begin{equation}\label{eqn:mixture_subg.term.5}
	\frac{1}{\hat{p}} \geq  \Bigg(1 - 2 \sqrt{\frac{\log (Nd)}{ Nd p}}\Bigg)\frac{1}{ p }.
\end{equation}
Combining with \eqref{eqn:mixture_subg.term.4} with \eqref{eqn:mixture_subg.term.5} leads to the conclusion.
\end{proof}


==> contents/Appx99_lemma_E2.tex <==
%%% ======================================================================
%%%	E2 is a high-probability event
%%% ======================================================================

\subsection{Proof of Lemma \ref{lem:E2}: $\hat{p} \approx p$}\label{sec:lemma_E2}

When $N, d \gg 1$, we may identify $\hat{p}$ with $p$. The exact statement of this claim is as follows.
\begin{lemma}\label{lem:conc_p}
	The fraction of observed entries, $\hat{p}$, concentrates to the sampling probability $p$. 
	Specifically, for any $\eta > 0$,
	\begin{equation}\label{eqn:binomial}
		\Prob{\cE_1(\eta)^c} \leq 2  \exp \left( - \frac{ 3\eta^2}{2(\eta+3)}Nd p \right).
	\end{equation}
\end{lemma}
\begin{proof}
	By Bernstein's inequality, for any $t \geq 0$,
	\[	\Prob{|\hat{p} - p | > t}	\leq 2 \exp \left( - \frac{ 3Ndt^2}{6p(1-p) + 2t} \right).	\]
	Therefore,
	\begin{align*}
		\Prob{|\hat{p} - p | > \eta p}	&\leq 2 \exp \left( - \frac{ 3Nd \eta^2p^2}{6p(1-p) + 2 \eta p} \right)\\
			&=		2 \exp \left( - \frac{ 3Nd \eta^2p^2}{(2\eta+6)p - 6p^2} \right)\\
			&\leq 	2 \exp \left( - \frac{ 3\eta^2}{2(\eta+3)}Nd p \right).
	\end{align*} 
\end{proof}

We may assume $0 < \eta \leq 1$. Then the right hand side of \eqref{eqn:binomial} is bounded above by 
$2 \exp \left( - \frac{3\eta^2}{8} Ndp \right)$. We need $\eta = \Omega \left( \frac{\log N + \log d}{\sqrt{Ndp}} \right)$ 
to make this probability decay no slower than a polynomial rate of $N, d$ as $N, d \to \infty$.




\begin{lemma}\label{lemma:replace_p_hat_with_p}
	Suppose that Condition \ref{cond:Bernoulli} holds. Then for any $\varepsilon > 1$,
	\begin{align*}
		\Prob{  \frac{1}{\varepsilon} p \le \hat{p} \le \varepsilon p } 
			\geq 1 - 2 \exp \left( - \frac{(\varepsilon - 1)^2}{2 \varepsilon^2} Ndp \right).
	\end{align*}
\end{lemma}
\begin{proof}
	Recall that we define $\hat{p}$ as
	\[	\hat{p} = \frac{1}{Nd} \sum_{i=1}^{N} \sum_{j=1}^d \Ind{ Y_{ij} \text{ observed}} \vee \frac{1}{Nd}.	\]
	By the binomial Chernoff bound, for $\varepsilon > 1$,
	\begin{align*}
		\Prob{ \hat{p} > \varepsilon p }
			&\leq \exp\left( - \frac{(\varepsilon - 1 )^2}{\varepsilon + 1} Ndp \right),	\quad\text{and}\\
		\Prob{ \hat{p} < \frac{1}{\varepsilon} p  }
			&\leq \exp \left( - \frac{(\varepsilon - 1)^2}{2 \varepsilon^2} Ndp \right).
	\end{align*}
	By the union bound,
	\[
		\Prob{  \frac{1}{\varepsilon} p \le \hat{p} \le \varepsilon p }
			\geq 1 - \Prob{ \hat{p} > \varepsilon p } -  \Prob{ \hat{p} < \frac{1}{\varepsilon} p  }.
	\]
	Noticing $\varepsilon + 1 < 2 \varepsilon < 2 \varepsilon^2$ for all $\varepsilon > 1$ completes the proof.
\end{proof}




==> contents/Appx99_lemma_E3.tex <==
%%% ======================================================================
%%%	E3 is a high-probability event
%%% ======================================================================

\subsection{Proof of Lemma \ref{lem:E3}}\label{sec:lemma_E3}

We want a high probability upper bound on $ \left\|\varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2^2 $, 
which is the squared $\ell_2$ norm of a projection of sub-gaussian random vector. We know that the $\ell_2$-norm of 
a sub-gaussian random vector projected onto a fixed $r$-dimensional subspace is of order $\tilde{O}(\sqrt{r})$. 
However, there is an additional complication in analyzing $ \left\|\varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2^2 $ because the subspace (=span of top $r$ right singular vectors of $Y$) is dependent on the vector 
(=the $i$-th row of the perturbation matrix) to take projection. 


\begin{lemma}\label{lem:ell2_upper}
Suppose that $\sigma_r(M) > \frac{\| Y - pM \|_2}{p}$ and $\| Y - pM \|_2 < t^* < \sigma_r(M) - \| Y - pM \|_2$. Then 
\begin{align*}
	\left\| \varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2^2 
		&\leq 4\left\|  Y^i - p M^i  \right\|_{\phi_2}^2 \left[ r + \left(  \frac{\| Y - p M \|_2}{p \sigma_r(M) - \| Y - p M \|_2} \right)^2 d \right]\log ( 2d N^5)
\end{align*}
%and
%\begin{align*}
%	\left\| \varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2^2 
%		& \leq 2\left\|  Y^i - p M^i  \right\|_{\phi_2}^2 \left( \sqrt{r} +   \frac{\| Y - p M \|_2}{p \sigma_r(M) - \| Y - p M \|_2}\sqrt{d} \right)^2\log ( 2d N^5) 
%\end{align*}
with probability at least $1 - \frac{2}{N^5}$.
\end{lemma}

\begin{proof}
Let $v_1^M, \ldots, v_r^M$ and $v_1^Y, \ldots, v_r^Y$ denote the top $r$ right singular vectors of $M$ and $Y$, respectively. Also, note that
\begin{align*}
	\varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) = \varphi_{M;0}^{\text{hard}} \Big(  Y^i - p M^i \Big) 
		+ \bigg[ \varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) - \varphi_{M;0}^{\text{hard}} \Big(  Y^i - p M^i \Big) \bigg].
\end{align*}

%\paragraph{Upper bounds on $\left\| \varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2^2 $}
%This observation leads to the following two inequalities. First, triangle inequality yields
%\begin{align}
%	\left\| \varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2 
%		&\leq \left\| \varphi_{M;0}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2
%		+ \left\| \varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) - \varphi_{M;0}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2	\nonumber\\
%		&= \left\| \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} } \Big(  Y^i - p M^i \Big) \right\|_2\nonumber\\
%			&\quad+ \left\|  \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y \} } \Big(  Y^i - p M^i \Big) - \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} } \Big(  Y^i - p M^i \Big) \right\|_2	\nonumber\\
%		&\leq \left\| \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} } \Big(  Y^i - p M^i \Big) \right\|_2	\nonumber\\
%			&\quad+ \left\|  \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y \} } - \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} }\right\|_2 
%			\Big\|  Y^i - p M^i \Big\|_2.		\label{eqn:triangle}
%\end{align}

Then Young's inequality of products yields
\begin{align*}
	\left\| \varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2^2 
		&\leq 2\left\| \varphi_{M;0}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2^2
		+ 2 \left\| \varphi_{Y;t^*}^{\text{hard}} \Big(  Y^i - p M^i \Big) - \varphi_{M;0}^{\text{hard}} \Big(  Y^i - p M^i \Big) \right\|_2^2	\nonumber\\
		&= 2\left\| \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} } \Big(  Y^i - p M^i \Big) \right\|_2^2	\nonumber\\
			&\quad+  2\left\|  \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y \} } \Big(  Y^i - p M^i \Big) - \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} } \Big(  Y^i - p M^i \Big) \right\|_2^2	\nonumber\\
		&\leq 2\left\| \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} } \Big(  Y^i - p M^i \Big) \right\|_2^2	\nonumber\\
			&\quad+ 2\left\|  \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y \} } - \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} }\right\|_2^2 
			\Big\|  Y^i - p M^i \Big\|_2^2.	\label{eqn:young}
\end{align*}
%We can see that \eqref{eqn:triangle} provides a sharper upper bound than \eqref{eqn:young} 
%when $\sigma_r(M) \approx \frac{1}{p}\| Y - pM \|_2$; the opposite is the case when $\sigma_r(M) \gg \frac{1}{p}\| Y - pM \|_2$.

%\paragraph{Stability of subspace}
Next, we have
\begin{align*}
	\big\| \mathcal{P}_{\text{span}\{v_1^Y, \ldots, v_r^Y\}} - \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M\}} \big\|_2
		&\leq  \frac{\| Y - p M \|_2}{p \sigma_r(M) - \| Y - p M \|_2}
\end{align*}
by Davis-Kahan $\sin \Theta$ theorem (see \eqref{eq:davis_kahan}).

Lastly, by applying Lemma \ref{lem:subg_projection}, we observe that for any $s_1, s_2 > 0$,
\begin{align*}
	&\Prob{\left\| \mathcal{P}_{\text{span}\{v_1^M, \ldots, v_r^M \} } \Big(  Y^i - p M^i \Big) \right\|_2^2 > s_1}
		\leq 2 r \exp \left( - \frac{s_1}{2r \left\|  Y^i - p M^i  \right\|_{\phi_2}^2} \right),\\
	&\Prob{\left\|  Y^i - p M^i \right\|_2^2 > s_2}
		\leq 2 d \exp \left( - \frac{s_2}{2d \left\|  Y^i - p M^i  \right\|_{\phi_2}^2} \right).
\end{align*}
Choose $s_1 = 2r \left\|  Y^i - p M^i  \right\|_{\phi_2}^2 \log ( 2r N^5)$ and 
$s_2 = 2d \left\|  Y^i - p M^i  \right\|_{\phi_2}^2 \log ( 2d N^5)$ to complete the proof.
\end{proof}




==> contents/Appx99_lemma_E3p.tex <==
%%% ======================================================================
%%%	E3' is a high-probability event
%%% ======================================================================

\section{Proof of Lemma \ref{lem:E3p}}\label{sec:lemma_E3p}
In this section, we present two intermediate propositions, which will be combined to yield Theorem \ref{thm:main_thm}. 
Throughout this section, we suppose that the parameter matrix $M$ and the data matrix $Y$ satisfy the model assumptions 
in section \ref{sssec: assumptions}. For $\eta, \zeta > 0$, let $\cE_1(\eta), \cE_2(\zeta)$ denote the conditioning events 
defined in Eq. \eqref{eqn:conditioning_event.1}, \eqref{eqn:conditioning_event.2}. Given $\eta, \zeta > 0$, let $t^*$ be chosen so that 
\begin{equation}\label{eqn:t.star}
	\frac{1}{\sqrt{1 - \eta}}\zeta \big( \sqrt{N} + \sqrt{d} \big) \sqrt{\hat{p}}	<	t^*	
	<	\frac{1}{\sqrt{1 + \eta}}\Big( \sqrt{\frac{ \hat{p} }{1 + \eta}} \frac{\sigma_r(M)}{\sqrt{N} + \sqrt{d} } - \zeta \Big) \big( \sqrt{N} + \sqrt{d} \big) \sqrt{\hat{p}}.
\end{equation}
In practice, one may not know $\sigma_r(M)$ a priori and may choose $t^*$ based on a lower bound on $\sigma_r(M)$.

The difference $ \left\|  \frac{1}{\hat{p}}  \varphi_{Y;t^*} \big(Y^i \big) - M^i \right\|_2$ (in the row $\ell_2$ norm sense) between our estimate 
and the parameter matrix is the quantity of our primary interest. By triangle inequality, 
\[	 \left\|  \frac{1}{\hat{p}}  \varphi_{Y;t^*} \big(Y^i \big) - M^i \right\|_2
		\leq \left\|  \frac{1}{\hat{p}}  \varphi_{Y;t^*} \big(Y^i \big) - \varphi_{Y;t^*} \big( M^i \big) \right\|_2	
			+	 \left\|  \varphi_{Y;t^*} \big( M^i \big) - M^i \right\|_2.
\]
We obtain deviation inequalities for $ \left\|  \frac{1}{\hat{p}}  \varphi_{Y;t^*} \big(Y^i \big) - \varphi_{Y;t^*} \big( M^i \big) \right\|_2$ (in 
Proposition \ref{prop:subG_proj}), and $ \left\|  \varphi_{Y;t^*} \big( M^i \big) - M^i \right\|_2$ (in Proposition \ref{prop:stable_subsp}) separately, 
and then integrate them into Theorem \ref{thm:main_thm} by the union bound.

Propositions \ref{prop:subG_proj}, \ref{prop:stable_subsp} and Theorem \ref{thm:main_thm} are stated in a conditional form on $\cE_1(\eta) \cap \cE_2(\zeta)$. 
Note that $\eta, \zeta > 0$ are parameters introduced solely for analysis and they do not appear in our algorithm. Later in section \ref{sec:proof_theorem.1}, 
we choose appropriate value for $\eta, \zeta > 0$ to prove the theorem.


\subsection{Deviation from the Mean after SVT}

We let $\hat{M} = \frac{1}{\hat{p}} SVT (Y; t^*)$. We have seen $\hat{M}^i = \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big)$ 
for each $i \in [N]$. We argue in the following proposition that $\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) 
- \varphi_{Y; t^*} \big( M^i \big) \right\|_{2}$ is small with high probability.

For $p, \eta, \zeta > 0$, define 
\begin{align}
	s^*_1(p, \eta, \zeta) 	
		&\triangleq \frac{1}{(1-\eta)p} \left( \frac{ \big(2\sqrt{2} c_1 \big( \tau + \Lambda K(p) \big) \sqrt{d} \big)^3 }{\sigma_r(M) - 2\zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p}} 
		\left( \log (2d) \log (N \vee d )\right)^{3/2}\right)^{\frac{1}{2}}.	\label{eqn:s_star.1}
\end{align}

\begin{proposition}\label{prop:subG_proj}
	Given $\eta, \zeta > 0$, \DG{ $\zeta < \frac{\sigma_r(M)}{2\sqrt{p} \left(\sqrt{N} + \sqrt{d}\right)}$, which is less strict than $\zeta < \frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}}$ when $p \leq \frac{1}{2}$} let $t^*$ satisfy \eqref{eqn:t.star}. For every $i \in [N]$ and every $s > s^*_1(p, \eta, \zeta)$,
	\begin{align*}
		&\Prob{ \left\|  \frac{1}{\hat{p}}  \varphi_{Y;t^*} \big(Y^i \big) - \varphi_{Y;t^*} \big( M^i \big) \right\|_2 > \frac{\eta}{1-\eta} \| M^i \|_2 + s ~\bigg|~ \cE_1(\eta) \cap \cE_2(\zeta)}\\
		&\qquad\leq \frac{1}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}} \Bigg[ 2r \exp \left( - \frac{ (1-\eta)^2 p^2~ \big\{ s^2 - s^*_1(p, \eta, \zeta)^2 \big\} }
		{4r c_1^2 c_2^2 \big( \tau + \Lambda K(p) \big)^2  } \right)+ \frac{1}{ (N \vee d )^4} \Bigg].
	\end{align*}
\end{proposition}

\begin{proof}
	First of all, we note that if $t^*$ satisfies \eqref{eqn:t.star}, then $\rank(\hat{M}) = \rank(M) = r$, according to Corollary \ref{cor:rank_data}. 
	
	Next, write the SVD of $Y$ as $Y = \hat{U} \hat{\Sigma} \hat{V}^T = \sum_{j=1}^{N \wedge d} \sigma_j(Y) \hat{U}_j \hat{V}_j^T$. We recall 
	from \eqref{eq:softsvt.1}, \eqref{eq:hardsvt.1} that for any $w \in \Reals^d$, $\varphi_{Y; t^*}(w) = \sum_{j=1}^r \rho_j \cP_{\hat{V}}^j(w)$ 
	where the contraction coefficient $\rho_j = 1$ for hard SVT and $\rho_j = \frac{\sigma_j(Y ) - t^*}{\sigma_j (Y )} \leq 1$ for soft SVT. 
	Note that whether soft or hard, $\varphi_{Y; t^*}$ is a linear contraction map, i.e., $\varphi_{Y;t^*} (\lambda w) = \lambda \varphi_{Y;t^*}(w)$ 
	and $\| \varphi_{Y;t^*}(w) \|_2 \leq \|w \|_2$ for any $\lambda \in \Reals, w \in \Reals^d$.

	By triangle inequality,
	\begin{equation}\label{eqn:prop1.term.0}
		\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \varphi_{Y; t^*} \big( M^i \big) \right\|_2
			\leq  \left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \frac{p}{\hat{p}}\varphi_{Y; t^*} \big( M^i \big) \right\|_2
				+  \left|\frac{p - \hat{p}}{\hat{p}}\right| \left\| \varphi_{Y; t^*} \big( M^i \big) \right\|_2.
	\end{equation}
	Therefore, for any $s_1, s_2 > 0$, and for any event $\cE$,
	\begin{align}
		\Prob{\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_1 + s_2 ~\bigg| ~ \cE}
			&\leq \Prob{\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \frac{p}{\hat{p}}\varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_1 ~\bigg| ~ \cE}
					\label{eqn:prop1.term.1}\\
				&\quad+ \Prob{  \left|\frac{p - \hat{p}}{\hat{p}}\right| \left\| \varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_2 ~\bigg| ~ \cE}.
					\label{eqn:prop1.term.2}
	\end{align}
	We choose $\cE = \cE_1(\eta) \cap \cE(\zeta)$.
	
	We establish separate upper bounds on \eqref{eqn:prop1.term.1} and \eqref{eqn:prop1.term.2} in the rest of the proof.
	In summary, provided that $s_1 \geq s^*_1(p, \eta, \zeta)$, 
	\begin{equation}\label{eqn:prop1.intermediate.1}
		\Prob{\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \frac{p}{\hat{p}}\varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_1 ~\bigg| ~ \cE}
			\leq		 \frac{1}{\Prob{\cE}} \Bigg[ 2r \exp \left( - \frac{ (1-\eta)^2 p^2~ (s_1^2 - s^*_1(p, \eta, \zeta)^2) }{2r \|  Y^i - p M^i \|_{\phi_2}^2 } \right)	
			+ \frac{1}{ (N \vee d )^4} \Bigg].
	\end{equation}
	Also, provided that $s_2 \geq  \frac{\eta}{1-\eta} \| M^i \|_2$, 
	\begin{equation}\label{eqn:prop1.intermediate.2}
		\Prob{  \left|\frac{p - \hat{p}}{\hat{p}}\right| \left\| \varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_2 ~\bigg| ~ \cE} = 0.
	\end{equation}
	
	Given $s \geq s^*_1(p, \eta, \zeta)$, choose $s_1 = s$ and $s_2 =  \frac{\eta}{1-\eta} \| M^i \|_2$. 
	Inserting \eqref{eqn:prop1.intermediate.1} to \eqref{eqn:prop1.term.1} and \eqref{eqn:prop1.intermediate.2} to \eqref{eqn:prop1.term.2} completes the proof 
	(recall that $ \|  Y^i - p M^i \|_{\phi_2} \leq c_2 \|  Y^i - p M^i \|_{\psi_2}  \leq c_1 c_2 \big( \tau + \Lambda K(p) \big)$ by Lemma \ref{lem:subG_Y}).
	
	\medskip
	Now, it remains to prove \eqref{eqn:prop1.intermediate.1} and \eqref{eqn:prop1.intermediate.2}.
	\begin{itemize}
	\item
	{\bf Proof of \eqref{eqn:prop1.intermediate.1}.}
	First of all, we obtain the following inequality because $\varphi_{Y;t^*}$ is a linear map and $\rho_j^2 \leq 1$ for all $j$. 
	\begin{align}
		\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \frac{p}{\hat{p}}\varphi_{Y; t^*} \big( M^i \big) \right\|_2^2
			&= \frac{1}{\hat{p}^2} \left\| \varphi_{Y; t^*} \big( Y^i - p M^i \big) \right\|_2^2		\nonumber\\
			&= \frac{1}{\hat{p}^2} \sum_{j=1}^r \rho_j^2 \cP_{\hat{V}}^j \Big( Y^i - p M^i \Big)^2		\nonumber\\
			&\leq  \frac{1}{\hat{p}^2} \sum_{j=1}^r \cP_{\hat{V}}^j \Big( Y^i - p M^i \Big)^2		\nonumber\\
			&= \frac{1}{\hat{p}^2}\left< \hat{V}_{1:r}\hat{V}_{1:r}^T ~, ~\Big( Y^i - p M^i \Big)^T \Big( Y^i - p M^i \Big) \right>,	\label{eqn:prop1.term.3}
	\end{align}
	where $\hat{V}_{1:r} \in \Reals^{d \times r}$ denote the matrix whose $j$-th column is equal to $\hat{V}_j$ and $\left<A, B\right> := \trace (A^TB)$ 
	denotes the inner product of two matrices $A, B \in \Reals^{n_1 \times n_2}$.
	
	To find an upper bound on \eqref{eqn:prop1.term.3}, we decouple the randomness in $Y^i - M^i$ from the randomness in all the other rows. 
	We fix $i \in [N]$ and define $\tilde{Y}(i) \in \Reals^{N \times d}$ such that $\tilde{Y}(i)^i = pM^i$ and $\tilde{Y}(i)^k = Y^k$ for $k \neq i$.
	Observe that $\tilde{Y}(i) = Y + \tilde{Z}(i)$ where 
	\[	 \tilde{Z}(i)^k = 
			\begin{cases}
				pM^i - Y^i	&	\text{if } k = i;\\
				0		&	\text{otherwise.}	
			\end{cases}			\]
	Write the SVD of $\tilde{Y}(i)$ as $\tilde{Y}(i) = \tilde{U}(i) \tilde{\Sigma}(i) \tilde{V}(i)^T = \sum_{j=1}^{N \wedge d} \sigma_j(\tilde{Y}(i)) \tilde{U}(i)_j \tilde{V}(i)_j^T$. 
	Since $\hat{V}_{1:r}\hat{V}_{1:r}^T = \tilde{V}(i)_{1:r}\tilde{V}(i)_{1:r}^T + \hat{V}_{1:r}\hat{V}_{1:r}^T - \tilde{V}(i)_{1:r}\tilde{V}(i)_{1:r}^T$ and $\left<A, B \right>
	\leq \|A \|_F \|B \|_F$ (Cauchy-Schwarz inequality), we can upper bound \eqref{eqn:prop1.term.3} as
	\begin{align}
		& \left< \hat{V}_{1:r}\hat{V}_{1:r}^T ~,~ \Big( Y^i - p M^i \Big)^T \Big( Y^i - p M^i \Big) \right>	\nonumber\\
			&\qquad\leq		 \left< \tilde{V}(i)_{1:r}\tilde{V}(i)_{1:r}^T ~,~ \Big( Y^i - p M^i \Big)^T \Big( Y^i - p M^i \Big) \right>	\label{eqn:prop1.term.4}\\
			&\qquad\quad
				+ \left\| \hat{V}_{1:r}\hat{V}_{1:r}^T - \tilde{V}(i)_{1:r}\tilde{V}(i)_{1:r}^T \right\|_F \left\| \Big( Y^i - p M^i \Big)^T \Big( Y^i - p M^i \Big) \right\|_F.	
					\label{eqn:prop1.term.5}
	\end{align}
	
	
	
	We further upper bound \eqref{eqn:prop1.term.1} using \eqref{eqn:prop1.term.3}, \eqref{eqn:prop1.term.4}, and \eqref{eqn:prop1.term.5}. 
	For $s_{11}, s_{12} > 0$ and $s_1 \geq \sqrt{s_{11} + s_{12}}$, 
	\begin{align}
		&\Prob{\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \frac{p}{\hat{p}}\varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_1 ~\bigg| ~ \cE}	\nonumber\\
			&\qquad=\Prob{\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \frac{p}{\hat{p}}\varphi_{Y; t^*} \big( M^i \big) \right\|_2^2 > s_1^2 ~\bigg| ~ \cE}	\nonumber\\
			&\qquad\leq	\Prob{ \frac{1}{\hat{p}^2} \left< \tilde{V}(i)_{1:r}\tilde{V}(i)_{1:r}^T ~, ~\Big( Y^i - p M^i \Big)^T \Big( Y^i - p M^i \Big) \right> > s_{11} ~\bigg| ~ \cE}
					\label{eqn:prop1.term.6}\\
			&\qquad\quad + \Prob{  \frac{1}{\hat{p}^2} \left\| \hat{V}_{1:r}\hat{V}_{1:r}^T - \tilde{V}(i)_{1:r}\tilde{V}(i)_{1:r}^T \right\|_F \left\| \Big( Y^i - p M^i \Big)^T \Big( Y^i - p M^i \Big) \right\|_F > s_{12} ~\bigg| ~ \cE}.		\label{eqn:prop1.term.7}
	\end{align}
	
	We establish upper bounds on \eqref{eqn:prop1.term.6} and \eqref{eqn:prop1.term.7} separately and then apply the union bound.
	Specifically, provided that $s_1 > s^*_1(p, \eta, \zeta)$ (see \eqref{eqn:s_star.1} for the definition of $s^*_1(p, \eta, \zeta)$), we choose 
	$s_{11} = s_1^2 - s^*_1(p, \eta, \zeta)^2$ and $s_{12} = s^*_1(p, \eta, \zeta)^2$ to achieve
	\begin{equation*}
		\Prob{\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \frac{p}{\hat{p}}\varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_1 ~\bigg| ~ \cE}
			\leq		 \frac{1}{\Prob{\cE}} \Bigg[ 2r \exp \left( - \frac{ (1-\eta) p~ (s_1^2 - s^*_1(p, \eta, \zeta)^2) }{2r \|  Y^i - p M^i \|_{\phi_2}^2 } \right)	
				+ \frac{1}{ (N \vee d )^4} \Bigg].
	\end{equation*}
	 
	
	\begin{enumerate}
	
	\item \emph{ Upper bounding \eqref{eqn:prop1.term.6}:}
	
	Recall that $\hat{p} \geq (1-\eta) p$ conditioned on $\cE = \cE_1(\eta) \cap \cE_2(\zeta)$. 
	By the law of total probability, if $\cE > 0$, then $\Prob{E_0 | \cE} \leq \frac{\Prob{E_0 }}{\Prob{\cE}}$.
	Observe that $ \tilde{V}(i)_{1:r} $ has orthogonal columns and $ \tilde{V}(i)_{1:r}$ is independent from $Y^i - pM^i$ as $ \tilde{V}(i)_{1:r}$ depends on 
	the randomness in the rows except for the $i$-th row. Therefore, for $s_{11} > 0$,
	\begin{align*}
		&\Prob{ \frac{1}{\hat{p}^2} \left< \tilde{V}(i)_{1:r}\tilde{V}(i)_{1:r}^T ~, ~\Big( Y^i - p M^i \Big)^T \Big( Y^i - p M^i \Big) \right> > s_{11} ~\bigg| ~ \cE}\\
		&\qquad\leq	 \Prob{ \left< \tilde{V}(i)_{1:r}\tilde{V}(i)_{1:r}^T ~, ~\Big( Y^i - p M^i \Big)^T \Big( Y^i - p M^i \Big) \right> > (1-\eta)^2 p^2~s_{11} ~\bigg| ~ \cE}\\
		&\qquad\leq	\frac{1}{\Prob{\cE}} \Prob{ \left< \tilde{V}(i)_{1:r}\tilde{V}(i)_{1:r}^T ~, ~\Big( Y^i - p M^i \Big)^T \Big( Y^i - p M^i \Big) \right> > (1-\eta)^2 p^2~s_{11} }\\
		&\qquad\leq	\frac{2r}{\Prob{\cE}} \exp \left( - \frac{ (1-\eta)^2 p^2~s_{11} }{2r \|  Y^i - p M^i \|_{\phi_2}^2 } \right)	
			\qquad\because \text{Lemma }\ref{lem:subg_projection}.
	\end{align*}
	By Lemma \ref{lem:subG_Y}, $ \|  Y^i - p M^i \|_{\phi_2} \leq c_2 \|  Y^i - p M^i \|_{\psi_2}  \leq c_1 c_2 \big( \tau + \Lambda K(p) \big)$.
	
	\item
	\emph {Upper bounding \eqref{eqn:prop1.term.7}:}
	First, we find a simplified upper bound on \eqref{eqn:prop1.term.5} as
	\begin{align*}
		 \left\| \hat{V}_{1:r}\hat{V}_{1:r}^T - \tilde{V}_{1:r}\tilde{V}_{1:r}^T \right\|_F \left\| \Big( Y^i - p M^i \Big)^T \Big( Y^i - p M^i \Big) \right\|_F
		 	&=  \left\| \hat{V}_{1:r}\hat{V}_{1:r}^T - \tilde{V}_{1:r}\tilde{V}_{1:r}^T \right\|_F \left\| Y^i - p M^i \right\|_2^2\\
			&\leq \frac{\| \tilde{Z}(i) \|_F}{\sigma_r(Y) - \sigma_{r+1}(\tilde{Y}(i))}  \left\| Y^i - p M^i \right\|_2^2\\
			&= \frac{\left\| Y^i - p M^i \right\|_2^3}{\sigma_r(Y) - \sigma_{r+1}(\tilde{Y}(i))}.
	\end{align*}
	
	Note that $\sigma_{r+1}(\tilde{Y}(i)) \leq \| Y - pM \|_2$. It is because $Y - pM = \tilde{Y}(i) - pM + \tilde{Z}(i)$
	where the $i$-th row of $\tilde{Y}(i) - pM$ is zero and $\tilde{Z}(i)$ is zero except the $i$-th row. 
	This implies
	\[	\sigma_{r+1}(\tilde{Y}(i)) \leq	\sigma_{r+1}(M) + \| \tilde{Y}(i) - pM \|_2 \leq   \| Y - pM \|_2.	\]
	Conditioned on $\cE = \cE_1(\eta) \cap \cE_2(\zeta)$, 
	\[	\sigma_r(Y) - \sigma_{r+1}(\tilde{Y}(i)) \geq \sigma_r(M) - 2\zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p}. 	\]
	
	Then \eqref{eqn:prop1.term.7} has the following upper bound: for $s_{12} > 0$,
	\begin{align}
		& \Prob{  \frac{1}{\hat{p}^2} \left\| \hat{V}_{1:r}\hat{V}_{1:r}^T - \tilde{V}(i)_{1:r}\tilde{V}(i)_{1:r}^T \right\|_F \left\| \Big( Y^i - p M^i \Big)^T \Big( Y^i - p M^i \Big) \right\|_F > s_{12} ~\bigg| ~ \cE}		\nonumber\\
			&\qquad\leq \Prob{	\frac{\left\| Y^i - p M^i \right\|_2^3}{\sigma_r(Y) - \sigma_{r+1}(\tilde{Y}(i))}	> (1-\eta)^2 p^2 ~ s_{12} ~\bigg| ~ \cE}		\nonumber\\
			&\qquad\leq \Prob{	\frac{\left\| Y^i - p M^i \right\|_2^3}{\sigma_r(M) - 2\zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p}}	> (1-\eta)^2 p^2 ~ s_{12} ~\bigg| ~ \cE}	\nonumber\\
			&\qquad\leq \frac{1}{\Prob{\cE}}\Prob{	\frac{\left\| Y^i - p M^i \right\|_2^3}{\sigma_r(M) - 2\zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p}}	> (1-\eta)^2 p^2 ~ s_{12} }.
				\label{eqn:prop1.term.8}
	\end{align}
	We define a conditioning event indexed by $i \in [N]$ and parameterized by $\xi > 0$ as %$ 2 \big\| Y^i - p M^i \|_{\phi_2} \sqrt{\log d}$
	\[	\cE_3^{(i)}(\xi)	\triangleq \{	\big\| Y^i - p M^i \|_2 \leq \xi	\}.	\]
	
	Let $\{ \be_1, \ldots, \be_d \} \in \Reals^d$ be an orthonormal basis vectors of $\Reals^d$ such that $\sum_{l=1}^d \be_l \be_l^T = I_d$.
	\begin{align*}
		\Prob{ \big\| Y^i - p M^i \|_2 > \xi }	&= 	\Prob{ \big\| Y^i - p M^i \|_2^2 > \xi^2 }\\
			&= \Prob{ \sum_{l=1}^d  \Big(\big( Y^i - p M^i \big) \be_l \Big)^2 > \xi^2 }\\
			&\leq \sum_{l=1}^d \Prob{  \Big(\big( Y^i - p M^i \big) \be_l \Big)^2 > \frac{\xi^2}{d} }\\
			&=\sum_{l=1}^d \Prob{ \big( Y^i - p M^i \big) \be_l  > \sqrt{\frac{\xi^2}{d}} }\\
			&\leq 2d \exp \left( - \frac{\xi^2}{2d \| Y^i - pM^i \|_{\phi_2}^2} \right)
	\end{align*}
	by the same argument as in the proof of Lemma \ref{lem:subg_projection}. Choose $\xi \geq 2  \| Y^i - pM^i \|_{\phi_2} \sqrt{2d}\sqrt{\log 2d } \sqrt{ \log (N \vee d)}$. 
	Then $\Prob{\cE_3^{(i)}(\xi) \geq 1 - \frac{1}{(N \vee d )^4}}$. We let $\xi_* \triangleq 2\sqrt{2} c_1 \big( \tau + \Lambda K(p) \big) \sqrt{d \log (2d) \log (N \vee d ) }$ denote 
	the value.
	
	Again by the law of total probability, we obtain the following upper bound on \eqref{eqn:prop1.term.8}:
	\begin{align*}
		&\frac{1}{\Prob{\cE}}\Prob{	\frac{\left\| Y^i - p M^i \right\|_2^3}{\sigma_r(M) - 2\zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p}}	> (1-\eta)^2 p^2 ~ s_{12} }\\
			&\qquad\leq \frac{1}{\Prob{\cE}} \Bigg[ \Prob{\frac{\left\| Y^i - p M^i \right\|_2^3}{\sigma_r(M) - 2\zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p}}	> (1-\eta)^2 p^2 ~ s_{12} ~\Bigg|~ \cE_3^{(i)}(\xi_*) }\Prob{\cE_3^{(i)}(\xi_*)}\\
				&\qquad\qquad\qquad\quad +  \Prob{\frac{\left\| Y^i - p M^i \right\|_2^3}{\sigma_r(M) - 2\zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p}}	> (1-\eta)^2 p^2 ~ s_{12} ~\Bigg|~ \cE_3^{(i)}(\xi_*)^c }\Prob{\cE_3^{(i)}(\xi_*)^c} \Bigg]\\
			&\qquad\leq
				 \frac{1}{\Prob{\cE}} \Bigg[ \Prob{\frac{\left\| Y^i - p M^i \right\|_2^3}{\sigma_r(M) - 2\zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p}}	> (1-\eta)^2 p^2 ~ s_{12} ~\Bigg|~ \cE_3^{(i)}(\xi_*) } + \Prob{\cE_3^{(i)}(\xi_*)^c} \Bigg]\\
			&\qquad\leq
				 \frac{1}{\Prob{\cE}} \Bigg[ \Prob{\frac{ \xi_*^3}{\sigma_r(M) - 2\zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p}}	> (1-\eta)^2 p^2 ~ s_{12} ~\Bigg|~ \cE_3^{(i)}(\xi_*) } + \Prob{\cE_3^{(i)}(\xi_*)^c} \Bigg]\\
			&\qquad\leq
				 \frac{1}{\Prob{\cE}} \Bigg[ \frac{1}{\Prob{\cE_3^{(i)}(\xi_*)}}\Prob{\frac{ \xi_*^3}{\sigma_r(M) - 2\zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p}}	> (1-\eta)^2 p^2 ~ s_{12} } + \Prob{\cE_3^{(i)}(\xi_*)^c} \Bigg] \\
			&=\frac{\Prob{\cE_3^{(i)}(\xi_*)^c}}{\Prob{\cE}}\\
			&\leq \frac{1}{\Prob{\cE}}\frac{1}{ (N \vee d )^4}
	\end{align*}
	provided that 
	\[	s_{12} \geq \frac{1}{(1-\eta)^2p^2}  ~ \frac{ \xi_*^3}{\sigma_r(M) - 2\zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p}}. 	\]
	\end{enumerate}
	
	
		
	\item
	{\bf Proof of \eqref{eqn:prop1.intermediate.2}.}
	
	Observe that $ \left|\frac{p - \hat{p}}{\hat{p}}\right| \leq \frac{\eta}{1-\eta}$ when conditioned on $\cE_1(\eta)$. 
	Moreover, $\left\| \varphi_{Y; t^*} \big( M^i \big) \right\|_2 \leq \| M^i \|_2 $ because $\varphi_{Y; t^*}$ is a contraction map. Therefore,
	\begin{align*}
		 \Prob{  \left|\frac{p - \hat{p}}{\hat{p}}\right| \left\| \varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_2 ~\bigg| ~ \cE}
		 	&\leq  \Prob{ \frac{\eta}{1-\eta} \left\| \varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_2 ~\bigg| ~ \cE}	\\
			&\leq \frac{1}{\Prob{\cE}}   \Prob{ \frac{\eta}{1-\eta} \left\| \varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_2 }	\\
			& = 0	
	\end{align*}
	provided that $s_2 \geq  \frac{\eta}{1-\eta} \| M^i \|_2$.
	\end{itemize}
\end{proof}


%%% ======================================================================
%%%	A Simpler Version of Proposition 1
%%% ======================================================================

\subsubsection{A Simpler Version Assuming $\sigma_r(M) \gg \frac{\sqrt{N}+\sqrt{d}}{p}$}

In this section, we state and prove a much simpler version of Proposition \ref{prop:subG_proj}. 
Actually, it establishes a sharper upper bound than the one stated in Proposition \ref{prop:subG_proj} 
provided that $\sigma_r(M) \gg \frac{\sqrt{N}+\sqrt{d}}{p}$ is necessary.

\begin{proposition}\label{prop:subG_proj_simple}
	Given $\eta, \zeta > 0$, \DG{$ \zeta < \frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}}$ as this prop relies on C.8} let $t^*$ satisfy \eqref{eqn:t.star}. For every $i \in [N]$ and every $s > 0$,
	\begin{align*}
		&\Prob{\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \varphi_{Y; t^*} \big( M^i \big) \right\|_2 
			> \frac{\eta}{1-\eta} \| M^i \|_2 +  \left(1 + \sqrt{\frac{d}{r}} \frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta} \right)s 
			~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}\\
		&\qquad\leq \frac{4d}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}}
				\exp\left( - \frac{(1-\eta)^2 p^2}{2 c_1^2 c_2^2 \big( \tau + \Lambda K(p) \big)^2} \frac{ s^2}{r} \right).
	\end{align*}	
\end{proposition}

\begin{proof}
	We establish an upper bound on \eqref{eqn:prop1.term.1} assuming $\sigma_r(M) \gg \frac{\sqrt{N}+\sqrt{d}}{p}$.
	\DG{Where did we use this assumption?}
	
	Write the SVD of $Y$ as $Y = \hat{U} \hat{\Sigma} \hat{V}^T = \sum_{j=1}^{N \wedge d} \sigma_j(Y) \hat{U}_j \hat{V}_j^T$. We recall 
	from \eqref{eq:softsvt.1}, \eqref{eq:hardsvt.1} that for any $w \in \Reals^d$\footnote{we take the row vector and right multiplication representation here}, 
	$\varphi_{Y; t^*}(w) = \sum_{j=1}^r \rho_j \cP_{\hat{V}}^j(w) = \sum_{j=1}^r \rho_j w \hat{V}_j \hat{V}_j^T $ where the contraction coefficient $\rho_j = 1$ 
	for hard SVT and $\rho_j = \frac{\sigma_j(Y ) - t^*}{\sigma_j (Y )} \leq 1$ for soft SVT. Note that whether soft or hard, $\varphi_{Y; t^*}$ is a linear contraction map, 
	i.e., $\varphi_{Y;t^*} (\lambda w) = \lambda \varphi_{Y;t^*}(w)$ and $\| \varphi_{Y;t^*}(w) \|_2 \leq \|w \|_2$ for any $\lambda \in \Reals, w \in \Reals^d$.
	
	\begin{align*}
		\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \frac{p}{\hat{p}}\varphi_{Y; t^*} \big( M^i \big) \right\|_2
			&= \frac{1}{\hat{p}} \left\| \varphi_{Y; t^*} \big( Y^i - pM^i \big)  \right\|_2\\
			&= \frac{1}{\hat{p}} \left\| \sum_{j=1}^r \rho_j \big( Y^i - pM^i \big)  \hat{V}_j \hat{V}_j^T  \right\|_2\\
			&\leq \frac{1}{\hat{p}} \left\| \sum_{j=1}^r \big( Y^i - pM^i \big)  \hat{V}_j \hat{V}_j^T  \right\|_2		
					\qquad\because \rho_j \leq 1 ~ \text{and}~ \hat{V}_{j_1}^T \hat{V}_{j_2} = \delta_{j_1 j_2}\\
			&=  \frac{1}{\hat{p}} \left \|  \big( Y^i - pM^i \big) \hat{V}_{1:r} \hat{V}_{1:r}^T \right\|_2.
	\end{align*}
	Here, $\hat{V}_{1:r} \in \Reals^{d \times r}$ denote the matrix whose columns are top $r$ right singular vectors of $Y$. In the same manner, 
	we let $V_{1:r} \in \Reals^{d \times r}$ denote the matrix whose columns are top $r$ right singular vectors of $M$.
	
	By triangle inequality, 
	\begin{align*}
		 \frac{1}{\hat{p}} \left \|  \big( Y^i - pM^i \big) \hat{V}_{1:r} \hat{V}_{1:r}^T \right\|_2	
		 	&\leq		\frac{1}{\hat{p}} \left \|  \big( Y^i - pM^i \big) V_{1:r} V_{1:r}^T \right\|_2 
				+  \frac{1}{\hat{p}} \left \|  \big( Y^i - pM^i \big) \left( \hat{V}_{1:r} \hat{V}_{1:r}^T - V_{1:r} V_{1:r}^T \right) \right\|_2\\
			&\leq		\frac{1}{\hat{p}} \left \|  \big( Y^i - pM^i \big) V_{1:r} V_{1:r}^T \right\|_2 
				+  \frac{1}{\hat{p}} \left\| \hat{V}_{1:r} \hat{V}_{1:r}^T - V_{1:r} V_{1:r}^T \right\|_2 \left \| Y^i - pM^i \right\|_2	
	\end{align*}

	For any $s_1, s_2 > 0$,
	\begin{align}
		&\Prob{\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \frac{p}{\hat{p}}\varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_1 + s_2 
				~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}	\nonumber\\
			&\qquad \leq \Prob{\frac{1}{\hat{p}} \left \|  \big( Y^i - pM^i \big) V_{1:r} V_{1:r}^T \right\|_2 > s_1~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta) }	\nonumber\\
				&\qquad\quad+ \Prob{  \frac{1}{\hat{p}} \left\| \hat{V}_{1:r} \hat{V}_{1:r}^T - V_{1:r} V_{1:r}^T \right\|_2 \left \| Y^i - pM^i \right\|_2	> s_2 
				~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}	\nonumber\\
			&\qquad \leq \Prob{ \left \|  \big( Y^i - pM^i \big) V_{1:r} V_{1:r}^T \right\|_2 > (1-\eta) p s_1~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta) }
					\label{eqn:prop.1.1.term.1}\\
				&\qquad\quad+ \Prob{ \left\| \hat{V}_{1:r} \hat{V}_{1:r}^T - V_{1:r} V_{1:r}^T \right\|_2 \left \| Y^i - pM^i \right\|_2	> (1-\eta) p s_2 
				~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}.	\label{eqn:prop.1.1.term.2}
	\end{align}
	
	First, we find an upper bound on \eqref{eqn:prop.1.1.term.1}:
	\begin{align}
		&\Prob{ \left \|  \big( Y^i - pM^i \big) V_{1:r} V_{1:r}^T \right\|_2 > (1-\eta) p s_1~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta) }	\nonumber\\
			&\qquad\leq \frac{1}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}}
				\Prob{ \left \|  \big( Y^i - pM^i \big) V_{1:r} V_{1:r}^T \right\|_2 > (1-\eta) p s_1 }	\nonumber\\
			&\qquad\leq \frac{2r}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}}
				\exp\left( - \frac{(1-\eta)^2 p^2 s_1^2}{2r \| Y^i - pM^i \|_{\phi_2}^2} \right)		\label{eqn:prop.1.1.term.3}
	\end{align}
	by Lemma \ref{lem:subg_projection}. 	
	
	Next, we observe that when conditioned on $\cE_2(\zeta)$ (for any $\zeta > 0$), 
	\[	\left\| \hat{V}_{1:r} \hat{V}_{1:r}^T - V_{1:r} V_{1:r}^T \right\|_2
			=\| \sin \Theta(\hat{V}_{1:r}, V_{1:r}) \| _2 
			\leq \frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta}.	\]
	by Lemma \ref{lem:subsp_stable}. 
	\DG{Here we need the assumption of $\sigma_r(M) > \zeta \frac{\sqrt{N} + \sqrt{d}}{\sqrt{p}}$.}
	
	With aid of this observation, we establish an upper bound on \eqref{eqn:prop.1.1.term.2}:
	\begin{align}
		&\Prob{ \left\| \hat{V}_{1:r} \hat{V}_{1:r}^T - V_{1:r} V_{1:r}^T \right\|_2 \left \| Y^i - pM^i \right\|_2	> (1-\eta) p s_2 
				~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}	\nonumber\\
			&\qquad\leq	\Prob{  \frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta} \left \| Y^i - pM^i \right\|_2	
				> (1-\eta) p s_2 ~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}	\nonumber\\
			&\qquad\leq	\Prob{   \left \| Y^i - pM^i \right\|_2	
				> \frac{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta}{\zeta} (1-\eta) p s_2 ~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}	\nonumber\\
			&\qquad\leq	\frac{1}{ \Prob{\cE_1(\eta) \cap \cE_2(\zeta)}} \Prob{   \left \| Y^i - pM^i \right\|_2	
				> \frac{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta}{\zeta} (1-\eta) p s_2 }	\nonumber\\
			&\qquad\leq \frac{2d}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}}
				\exp\left( - \frac{(1-\eta)^2 p^2 s_2^2}{2d \| Y^i - pM^i \|_{\phi_2}^2} 
					\bigg( \frac{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta}{\zeta}  \bigg)^2 \right)	\label{eqn:prop.1.1.term.4}
	\end{align}
	again by Lemma \ref{lem:subg_projection}. 	
	
	Inserting \eqref{eqn:prop.1.1.term.3} to \eqref{eqn:prop.1.1.term.1} and \eqref{eqn:prop.1.1.term.4} to \eqref{eqn:prop.1.1.term.2} yields
	\begin{align*}
		&\Prob{\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \frac{p}{\hat{p}}\varphi_{Y; t^*} \big( M^i \big) \right\|_2 > s_1 + s_2 
				~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}	\\
			&\qquad \leq \frac{2}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}}
				\Bigg\{ r\exp\left( - \frac{(1-\eta)^2 p^2}{2 \| Y^i - pM^i \|_{\phi_2}^2} \frac{ s_1^2}{r} \right)
					+ d \exp\left( - \frac{(1-\eta)^2 p^2 }{2 \| Y^i - pM^i \|_{\phi_2}^2} 
					\bigg( \frac{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta}{\zeta}  \bigg)^2 \frac{s_2^2}{d} \right)	\Bigg\}
	\end{align*}
	Choose $s_2 = s_1 \sqrt{\frac{d}{r}} \frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta}$. Then
	\begin{align}
		&\Prob{\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \frac{p}{\hat{p}}\varphi_{Y; t^*} \big( M^i \big) \right\|_2 
			>  \left(1 + \sqrt{\frac{d}{r}} \frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta} \right)s_1 ~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}	
						\nonumber\\
			&\qquad \leq \frac{2}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}}
				\Bigg\{ r\exp\left( - \frac{(1-\eta)^2 p^2}{2 \| Y^i - pM^i \|_{\phi_2}^2} \frac{ s_1^2}{r} \right)
					+ d \exp\left( - \frac{(1-\eta)^2 p^2 }{2 \| Y^i - pM^i \|_{\phi_2}^2} 
					\bigg( \frac{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta}{\zeta}  \bigg)^2 \frac{s_1^2}{r} \right)	\Bigg\}
							\nonumber\\
			&\qquad\leq	\frac{4d}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}}
				\exp\left( - \frac{(1-\eta)^2 p^2}{2 \| Y^i - pM^i \|_{\phi_2}^2} \frac{ s_1^2}{r} \right).		\label{eqn:prop.1.1.term.5}
	\end{align}
	
	Putting \eqref{eqn:prop.1.1.term.5} back to \eqref{eqn:prop1.term.1}, we obtain the following inequality: for any $s > 0$,
	\begin{align*}
		&\Prob{\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \varphi_{Y; t^*} \big( M^i \big) \right\|_2 
			> \frac{\eta}{1-\eta} \| M^i \|_2 +  \left(1 + \sqrt{\frac{d}{r}} \frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta} \right)s 
			~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}\\
		&\qquad\leq \frac{4d}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}}
				\exp\left( - \frac{(1-\eta)^2 p^2}{2 \| Y^i - pM^i \|_{\phi_2}^2} \frac{ s^2}{r} \right).
	\end{align*}
	We can conclude the proof by realizing that $\| Y^i - pM^i \|_{\phi_2} \leq c_1 c_2 \big( \tau + \Lambda K(p) \big)$.
\end{proof}


%%% ======================================================================
%%%	Intermediate Proposition 2
%%% ======================================================================

\subsection{Stability of Top-$r$ Singular Subspace}
\begin{proposition}\label{prop:stable_subsp}
	Given $\eta, \zeta > 0$, \DG{upper bound on $\zeta$; $ \zeta < \frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}}$ as per C.8} let $t^*$ satisfy \eqref{eqn:t.star}. When conditioned on $\cE_1(\eta) \cap \cE_2(\zeta)$, 
	for any vector $w$ in the row space of $M$,
	\begin{align*}
		&\Big\|~ \varphi^{\text{hard}}_{Y; t^*} \big( w \big) - w \Big\|_2 
			\leq		\frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta}  \big\| w \big\|_2,	\quad\text{and}\\
		&\Big\|~ \varphi^{\text{soft}}_{Y; t^*} \big( w \big) - w \Big\|_2
			\leq	\frac{ \Big[  \Big( \frac{ t^*}{ (\sqrt{N} + \sqrt{d} ) \sqrt{p} }  \Big)^2 + \zeta^2 \Big]^{1/2}}
			{ \frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta }  \left\| w \right\|_2.
	\end{align*}
\end{proposition}
	
\begin{proof}
	With the given choice of $t^*$, $\rank(\hat{M}) = \rank(M)$, conditioned on $\cE_1(\eta) \cap \cE_2(\zeta)$ due to Corollary \ref{cor:rank_data}.
	
	We write the SVD of $M$ and $Y$ as $M = U \Sigma V^T =  \sum_{j=1}^{N \wedge d} \sigma_j(M) U_j V_j^T$ and 
	$Y = \hat{U} \hat{\Sigma} \hat{V}^T = \sum_{j=1}^{N \wedge d} \sigma_j(Y) \hat{U}_j \hat{V}_j^T$. Then for any $w \in \Reals^d$ (we take the row vector 
	representation of $w$),
	\[	\varphi^{\text{hard}}_{Y; t^*} \big( w \big) =  \hat{V}_{1:r} \hat{V}_{1:r}^T w.	\]
	and moreover, if $w$ is in the row space of $M$, then $V_{1:r} V_{1:r}^T w = w$.
%	\begin{align*}
%		&\varphi^{\text{hard}}_{Y; t^*} \big( M^i \big) = \sum_{j=1}^r \cP_{\hat{V}}^j \big( M^i \big) \in span \{ \hat{V}_1^T, \ldots, \hat{V}_r^T\},	\quad\text{and}\\
%		&M^i - \varphi^{\text{hard}}_{Y; t^*} \big( M^i \big) = \sum_{j=r+1}^d \cP_{\hat{V}}^j \big( M^i \big) \in span \{ \hat{V}_1^T, \ldots, \hat{V}_r^T\}^{\perp}.
%	\end{align*}
	By Lemma \ref{lem:subsp_stable}, when conditioned on $\cE_2(\zeta)$,
	\[	
		\Big\|~ \varphi^{\text{hard}}_{Y; t^*} \big( w \big) - w \Big\|_2 
			= \Big\|~  \big( \hat{V}_{1:r} \hat{V}_{1:r}^T - V_{1:r} V_{1:r}^T \big) w \Big\|_2 
			\leq	\| \sin \Theta(V_{1:r}, \hat{V}_{1:r}) \| _2 \big\| w \big\|_2
			\leq	\frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta}  \big\| w \big\|_2.
	\]

	For soft SVT,
	\begin{align*}
		&\varphi^{\text{soft}}_{Y; t^*} \big( w \big) = \sum_{j=1}^r \frac{\sigma_j(Y) - t^*}{\sigma_j(Y)} \cP_{\hat{V}}^j \big( w \big).
	\end{align*}
	Therefore, $\varphi^{\text{soft}}_{Y; t^*} \big( w \big) - \varphi^{\text{hard}}_{Y; t^*} \big( w \big)  \in 
	span \{ \hat{V}_1^T, \ldots, \hat{V}_r^T\}$ and
	\begin{align*}
		\left\| \varphi^{\text{hard}}_{Y; t^*} \big( w \big) - \varphi^{\text{soft}}_{Y; t^*} \big( w \big) \right\|_2^2
			&= \sum_{j=1}^r  \left(\frac{ t^*}{\sigma_j(Y)}\right)^2 \cP_{\hat{V}}^j \big( w \big)^2\\
			&\leq \sum_{j=1}^r \left( \frac{ t^*  }
				{ p \sigma_r(M) - \zeta (\sqrt{N} + \sqrt{d} ) \sqrt{p} } \right)^2 	\cP_{\hat{V}}^j \big( w \big)^2	\\
			&\leq \left( \frac{ \frac{ t^*}{ (\sqrt{N} + \sqrt{d} ) \sqrt{p} } }
				{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta} \right)^2 \big\| \hat{V}_{1:r} \hat{V}_{1:r}^T w\big\|_2^2\\
			&\leq  \left( \frac{ \frac{ t^*}{ (\sqrt{N} + \sqrt{d} ) \sqrt{p} } }
				{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta} \right)^2	 \left\| w \right\|_2^2.
	\end{align*}
	We used $\hat{p} \leq (1+\eta)p$ conditioned on $\cE_1(\eta)$ and $ \big\| \hat{V}_{1:r} \hat{V}_{1:r}^T w\big\|_2 \leq\left\| w \right\|_2$.
	
	Observe that 
	\begin{align*}
		&\varphi^{\text{soft}}_{Y; t^*} \big( w \big) - w  = \varphi^{\text{soft}}_{Y; t^*} \big( w \big) - \varphi^{\text{hard}}_{Y; t^*} \big( w \big) + 
			w - \varphi^{\text{hard}}_{Y; t^*} \big( w \big)	\quad\text{and}\\
		&\left< \varphi^{\text{soft}}_{Y; t^*} \big( w \big) - \varphi^{\text{hard}}_{Y; t^*} \big( w \big)~,~ 
			w - \varphi^{\text{hard}}_{Y; t^*} \big( w \big) \right> = 0. 
	\end{align*}
	By the Pythagorean theorem yields
	\begin{align*}
		\Big\|~ \varphi^{\text{soft}}_{Y; t^*} \big( w \big) - w \Big\|_2^2 
			&= \Big\|~ \varphi^{\text{soft}}_{Y; t^*} \big( w \big) -  \varphi^{\text{hard}}_{Y; t^*} \big( w \big) \Big\|_2^2  
				+ \Big\|~ \varphi^{\text{hard}}_{Y; t^*} \big( w \big) - w \Big\|_2^2 \\
			&\leq \frac{ \Big( \frac{ t^*}{ (\sqrt{N} + \sqrt{d} ) \sqrt{p} }  \Big)^2 + \zeta^2}{ \Big(\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta \Big)^2}  \left\| w \right\|_2^2.	
	\end{align*}
\end{proof}



%%% ======================================================================
%%%	Combining the Propositions
%%% ======================================================================


\subsection{Towards Theorem \ref{thm:rowmaxnorm}: Combining Propositions \ref{prop:subG_proj} and \ref{prop:stable_subsp}}\label{sec:proof.main.1}

In this section, we put Propositions \ref{prop:subG_proj}, \ref{prop:stable_subsp} together to state and prove a result that is a step towards 
Theorem \ref{thm:rowmaxnorm}. Before stating the theorem, we define 
\begin{equation}\label{eqn:Gamma}
	\Gamma^{\text{hard}}(M; p, \zeta)	\frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta}   \qquad\text{and}\qquad
	\Gamma^{\text{soft}}(M; p, \zeta)	\frac{ \Big[  \Big( \frac{ t^*}{ (\sqrt{N} + \sqrt{d} ) \sqrt{p} }  \Big)^2 + \zeta^2 \Big]^{1/2}}
			{ \frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta }.
\end{equation}

\begin{theorem}\label{thm:main_thm}
Given $\eta, \zeta > 0$, let $t^*$ satisfy \eqref{eqn:t.star}. For every $i \in [N]$, and every $s > s^*_1(p, \eta, \zeta) $,
\begin{align*}
		&\Prob{ \left\| \frac{1}{\hat{p}}  \varphi_{Y;t^*} \big(Y^i \big) - M^i \right\|_{2} > \bigg( \Gamma(M; p, \zeta) + \frac{\eta }{1-\eta} \bigg) \big\| M^i \big\|_2 + s ~\Big|~ \cE_1(\eta) \cap \cE_2(\zeta) }\\
		&\qquad\leq \frac{1}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}} \Bigg[ 2r \exp \left( - \frac{ (1-\eta)^2 p^2~ \big\{ s^2 - s^*_1(p, \eta, \zeta)^2 \big\} }
		{4r c_1^2 c_2^2 \big( \tau + \Lambda K(p) \big)^2  } \right)+ \frac{1}{ (N \vee d )^4} \Bigg].
\end{align*}
\end{theorem}
\begin{proof}	
	By triangle inequality,
	 \begin{align*}
	 	\left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - M^i \right\|_{2}
			&\leq \left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \varphi_{Y; t^*} \big( M^i \big) \right\|_{2}
			+ \left\| \varphi_{Y; t^*} \big(M^i \big) - M^i \right\|_{2}.
	\end{align*}
	Applying the usual union bound trick, it follows that for any $s > 0$, 
	\begin{align*}
		&\Prob{ \left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - M^i \right\|_{2} > \bigg( \Gamma(M; p, \zeta) + \frac{\eta }{1-\eta} \bigg) \big\| M^i \big\|_2 + s ~\bigg|~ \cE_1(\eta) \cap \cE_2(\zeta)}\\
			&\qquad\leq \Prob{ \left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \varphi_{Y; t^*} \big( M^i \big) \right\|_{2}
				  > \frac{\eta }{1-\eta}\big\| M^i \big\|_2 + s ~\bigg| ~\cE_1(\eta) \cap \cE_2(\zeta)}\\
			&\qquad\quad	+ \Prob{  \left\| \varphi_{Y; t^*} \big(M^i \big) - M^i \right\|_{2} > \Gamma(M; p, \zeta) \big\| M^i \big\|_2 ~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}.			
	\end{align*}
	
	By Propositions \ref{prop:subG_proj},
	\begin{align*}
		&\Prob{ \left\| \frac{1}{\hat{p}} \varphi_{Y; t^*} \big( Y^i \big) - \varphi_{Y; t^*} \big( M^i \big) \right\|_{2}
				  > \frac{\eta }{1-\eta}\big\| M^i \big\|_2 + s ~\bigg| ~\cE_1(\eta) \cap \cE_2(\zeta)}\\
		&\qquad\leq \frac{1}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}} \Bigg[ 2r \exp \left( - \frac{ (1-\eta)^2 p^2~ \big\{ s^2 - s^*_1(p, \eta, \zeta)^2 \big\} }
		{4r c_1^2 c_2^2 \big( \tau + \Lambda K(p) \big)^2  } \right)+ \frac{1}{ (N \vee d )^4} \Bigg]
	\end{align*}
	for $s \geq s^*_1(p, \eta, \zeta)$. Moreover, we have
	\[ \Prob{  \left\| \varphi_{Y; t^*} \big(M^i \big) - M^i \right\|_{2} > \Gamma(M; p, \zeta) \big\| M^i \big\|_2 ~\bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)} = 0 \]
	by Proposition \ref{prop:stable_subsp}.
\end{proof}


\begin{figure}[h!]
	\centering
	\begin{tikzpicture}
		\draw[-] (-2, -1) -- (2.5, 0.6) -- (3.5, 2.6) -- (-1, 1) -- (-2, -1);	
		\draw[-] (-1.7, -0.96) -- (-2.25, -1.95) -- (4, -1.95) -- (5.25, 0.3) -- (1.7, 0.3);	%(-1, 0.3)
		\draw[dashed] (-1.7, -0.96) -- (-1, 0.3) -- (1.7, 0.3);
		
		% point M^i
		\filldraw (0.6, 0.9) circle (1pt);
		\node (Mi) at (0.9, 1.1) {$M^i$};
		% point Y^i
		\filldraw (3, 0.8) circle (1pt);
		\node (Yi) at (3.4, 1) {$\frac{1}{\hat{p}}Y^i$};
		% point projM^i
		\filldraw (0.6, -0.6) circle (1pt);
		\node (proj_Mi_hard) at (1.4, -0.3) {$\varphi_{Y; t^*}^{\text{hard}} (M^i)$};
		% point projY^i
		\filldraw (3, -0.8) circle (1pt);
		\node (proj_Yi_hard) at (3.9, -0.5) {$\frac{1}{\hat{p}}\varphi_{Y; t^*}^{\text{hard}} \big( Y^i\big)$};

		\node (Mspan) at (4.7, 2.1) {$span\{ V_1^T, \ldots, V_r^T \}$};
		\node (Yspan) at (4.2, -2.3) {$span\{ \hat{V}_1^T, \ldots, \hat{V}_r^T \}$};

		
		\draw[-stealth, line width = .5pt, dotted] (0.6, 0.9) -- (0.6, -0.6);
		\draw[-stealth, line width = .5pt, dotted] (3, 0.8) -- (3, -0.8);
		\draw[-stealth, line width = .5pt, dotted] (0.6, 0.9) -- (0, -1.1);
		\draw[-stealth, line width = .5pt, dotted] (3, 0.8) -- (2.4, -1.3);
%		\draw[dotted] (0.6, -0.6) -- (3, -0.8);
		\draw[-] (0.6, -0.4) -- (0.4, -0.55) -- (0.4, -0.75);
		
		\draw[dotted] (0.6, -0.6) -- (0, -1.1);
		% point projM^i
		\filldraw (0, -1.1) circle (1pt);
		\node (proj_Mi_soft) at (-0.2, -1.5) {$\varphi_{Y; t^*}^{\text{soft}} (M^i)$};
		% point projY^i
		\filldraw (2.4, -1.3) circle (1pt);
		\node (proj_Yi_soft) at (2.4, -1.6) {$\frac{1}{\hat{p}} \varphi_{Y; t^*}^{\text{soft}} \big(  Y^i\big)$};
		
		\draw[line width = .75 pt, dashed, red] (0.6, 0.9) -- (0.6, -0.6) -- (3, -0.8);
		\draw[line width = .75 pt, dashed, blue] (0.6, 0.9) -- (0, -1.1) -- (2.4, -1.3);
	\end{tikzpicture}
	\caption{%Diagram for the $l_2$ distance between $M^i$ and $\hat{M}^i = \frac{1}{\hat{p}}\varphi_{Y; t^*} \big( Y^i \big)$; 
	An illustration of the Proof Theorem \ref{thm:main_thm} ({\color{red} Red}: hard SVT, and {\color{blue} Blue}: soft SVT).}
	\label{fig:max_l2_row}
\end{figure}




==> contents/Appx99_premise1_subgaussian.tex <==
%%% ======================================================================
%%%	Proof of Premise 3
%%% ======================================================================

\section{Proof of Lemma \ref{lem:subG_est}}\label{sec:proof.prem.3}
\begin{proof}
	Observe that for any $u \in \bbS^{d-1}$, and any $\lambda \in \Reals$,
	\begin{align*}
		\Exp{ \exp\left\{ \lambda \left(\frac{1}{\hat{p}}Y^i - M^i \right) u\right\} ~ \bigg| ~ \cE_1(\eta) }
			&= \int_0^{\infty} \Prob{ \exp\left\{ \lambda \left(\frac{1}{\hat{p}}Y^i - M^i \right) u\right\}
				\geq s ~ \bigg| ~ \cE_1(\eta)} ds
	\end{align*}
	because $ \exp\left\{ \lambda \left(\frac{1}{\hat{p}}Y^i - M^i \right) u \right\} \geq 0$. Recall that $\Prob{E_0} \geq \Prob{E_0, E_1} 
	=  \Prob{E_0 \big| E_1} \Prob{E_1}$ for any events $E_0$ and $E_1$. When $\Prob{E_1} > 0$, this implies $ \Prob{E_0 \big| E_1} 
	\leq \frac{\Prob{E_0}}{\Prob{E_1}}$. We let $E_1 = \cE_1(\eta)$. Then it follows that
	\begin{align}
		\int_0^{\infty} \Prob{ \exp\left\{ \lambda \left(\frac{1}{\hat{p}}Y^i - M^i \right) u\right\}
				\geq s ~ \bigg| ~ \cE_1(\eta)} ds
			&\leq \frac{1}{\Prob{\cE_1(\eta)}} 
				\int_0^{\infty} \Prob{ \exp\left\{ \lambda \left(\frac{1}{\hat{p}}Y^i - M^i \right) u\right\}  \geq s} ds		\nonumber\\
			&= \frac{1}{\Prob{\cE_1(\eta)}} \Exp{ \exp\left\{ \lambda \left(\frac{1}{\hat{p}}Y^i - M^i \right) u\right\} }.	\label{eqn:B.term.1}
	\end{align}
	
	Now it suffices to find an upper bound on the expectation in \eqref{eqn:B.term.1}.
	Decompose the $i$-th row ($i \in [N]$) of the matrix of interest as
	\[	\frac{1}{ \hat{p} }Y^i - M^i = \frac{1}{\hat{p}} \left( Y^i - pM^i \right) + \frac{p - \hat{p}}{\hat{p}} M^i. 	\]
	For any $q > 1$,
	\begin{align}
		&\Exp{ \exp\left\{ \lambda \left(\frac{1}{\hat{p}}Y^i - M^i \right) u\right\} ~ \bigg| ~ \cE_1(\eta) }	\nonumber\\
		&\qquad=  \Exp{ \exp\left\{ \lambda \left( \frac{1}{\hat{p}} \left( Y^i - pM^i \right) 
				+ \frac{p - \hat{p}}{\hat{p}} M^i \right) u\right\} ~ \bigg| ~ \cE_1(\eta) }	\nonumber\\
		&\qquad\leq \frac{1}{q} \Exp{ \exp\left( \frac{q \lambda}{\hat{p}} \left( Y^i - pM^i \right) u \right) ~ \bigg| ~ \cE_1(\eta) }%\nonumber\\
				+ \frac{q-1}{q} \Exp{ \exp\left( \frac{\frac{q}{q-1} \lambda (p - \hat{p})}{\hat{p}} M^i u \right)~ \bigg| ~ \cE_1(\eta) }
					\label{eqn:sec7_term.0}.
	\end{align}
	The last line follows from Young's inequality for the product : if $a, b \geq 0$ and $q, r > 0$ with 
	$\frac{1}{q} + \frac{1}{r} = 1$, then $ab \leq \frac{a^q}{q} + \frac{b^r}{r}$ ($r = \frac{q}{q-1}$).
	
	Since $\hat{p} \geq (1 - \eta) p$ when conditioned on $\cE_1(\eta)$, we have
	\begin{align}
		\Exp{ \exp\left( \frac{q \lambda}{\hat{p}} \left( Y^i - pM^i \right) u \right) \bigg| ~\cE_1(\eta)~}
			&\leq \Exp{ \exp\left( \frac{q \lambda}{(1-\eta) p} \left( Y^i - pM^i \right) u \right) \bigg| ~\cE_1(\eta)~}	\nonumber\\
			&\leq \frac{1}{\Prob{\cE_1(\eta)}}\Exp{ \exp\left( \frac{ q \lambda}{(1-\eta)p} \left( Y^i - pM^i \right) u \right) }.	
				\label{eqn:sec7.term1}
	\end{align}
	
	By Lemma \ref{lem:subG_Y} and the equivalence between $\|\cdot\|_{\psi_2}$ and $\| \cdot \|_{\phi_2}$ 
	(see Definition \ref{defn:phi2}), we know that
	\begin{align}
		\bigg\|\frac{q}{(1-\eta)p} (Y^i - pM^i)u \bigg\|_{\phi_2}
			&\leq	\frac{q c_2}{(1-\eta)p} \sup_{u \in \bbS^{d-1}} \big\| (Y^i - pM^i)u \big\|_{\psi_2}	\nonumber\\
			&\leq \frac{q c_1 c_2}{(1-\eta)p} \left( \tau + \Lambda K(p) \right). 	\label{eqn:sec7.phi1}
	\end{align}
	
	In the same vein,
	\begin{align}
		\Exp{ \exp\left( \frac{\frac{q-1}{q} \lambda (p - \hat{p})}{\hat{p}} M^i u \right) \bigg| ~\cE_1(\eta)~}
			&\leq \Exp{ \exp\left( \frac{ (q-1) \lambda}{(1-\eta)pq} (p - \hat{p}) M^i u \right) \bigg| ~\cE_1(\eta)~}	\nonumber\\
			&\leq \frac{1}{\Prob{\cE_1(\eta)}}\Exp{ \exp\left( \frac{(q-1) \lambda}{(1-\eta)pq} (p - \hat{p}) M^i u \right) }.
				\label{eqn:sec7.term2}
	\end{align}
	We know that $(p - \hat{p})M^iu$ is a centered sub-gaussian random variable from the model assumption. Recall that 
	$\hat{p} = \frac{1}{Nd} \sum_{(i,j) \in [N] \times [d]} \Ind{E_{ij} = 1}$ is the average of $Nd$ independent sub-gaussian random variables. 
	Therefore,
	\begin{align*}
		\| \hat{p} - p \|_{\phi_2} &= \frac{1}{\sqrt{Nd}}\big\| \Ind{E_{ij} = 1} - p \big\|_{\phi_2} \\
			&\leq \frac{1}{\sqrt{Nd}} K(p).	\qquad \because \text{Theorem } \ref{thm:phi2_Bernoulli},
	\end{align*}
	This yields
	\begin{align}
		\bigg\| \frac{ (q-1)}{(1-\eta)pq} (p - \hat{p}) M^i u \bigg\|_{\phi_2}
			&\leq	 \frac{(q-1) M^i u}{(1-\eta)pq } \frac{K(p)}{\sqrt{Nd}}	\nonumber\\
			&\leq \frac{(q-1)\Lambda }{(1-\eta)pq \sqrt{N}}K(p)	\label{eqn:sec7.phi2}
	\end{align}
	because $M^i u \leq \| M^i \|_2 \leq \sqrt{d}$.

	By definition, $\Exp{ \exp(\lambda X)} \leq \exp \left( \frac{\lambda^2}{2} \| X \|_{\phi_2}^2 \right)$ for all $\lambda \in \Reals$. 
	Combining \eqref{eqn:sec7.term1}, \eqref{eqn:sec7.phi1}, \eqref{eqn:sec7.term2}, \eqref{eqn:sec7.phi2} with 
	\eqref{eqn:sec7_term.0} leads to the conclusion:
	\begin{align*}	
		&\Exp{ \exp\left( \lambda u^T \left(\frac{1}{\hat{p}}Y_i - M_i \right)\right) \bigg| ~\cE_1(\eta)~}\\
			&\qquad\leq \frac{1}{\Prob{\cE_1(\eta)}}
				\Bigg\{ \frac{1}{q} \exp\bigg( \frac{\lambda^2}{2} \frac{q^2 c_1^2 c_2^2}{(1-\eta)^2p^2} \left( \tau + \Lambda K(p) \right)^2 \bigg)
				+ \frac{q-1}{q}  \exp \bigg( \frac{\lambda^2}{2}	  \frac{(q-1)^2 }{(1-\eta)^2p^2q^2 N} \Lambda^2  K(p)^2	\bigg) \Bigg\}.	\label{eqn:subG.term.1}
%			&\qquad\leq \frac{1}{\Prob{\cE_1(\eta)}}
%				\exp\bigg( \frac{\lambda^2}{2} \frac{100 c_2^2}{81p^2} \left( c_1\tau + c_1c_2\frac{\max\{ p, 1-p \}}{\sqrt{\ln 2}} \right)^2 \bigg).
	\end{align*}
	
	We may assume $c_1 c_2 \geq 1$, $\tau \geq 0$. Optimizing over $q > 1$, we get the best upper bound 
	with $q \to 1$ (in the limit).
	\begin{align*}	
		\Exp{ \exp\left( \lambda u^T \left(\frac{1}{\hat{p}}Y^i - M^i \right)\right) \bigg| ~\cE_1(\eta)~}
			&\leq \frac{1}{\Prob{\cE_1(\eta)}}
				\exp\bigg( \frac{\lambda^2}{2} \frac{c_1^2 c_2^2}{(1-\eta)^2p^2} \left( \tau + \Lambda K(p) \right)^2 \bigg).
	\end{align*}
	This inequality holds for any choice of $u \in \bbS^{d-1}$, hence, the proof is complete.
\end{proof}

==> contents/Appx99_premise2_op_norm.tex <==
%%% ======================================================================
%%%	Proof of Premise 2
%%% ======================================================================

\section{Proof of Lemma \ref{lem:noise_singular}}\label{sec:proof_lem_spectral}

%\begin{lemma} \label{lem:noise_singular}
%Let $Z = Y - pM$. For every $t \geq 0$,
%\begin{align*}
%	\sigma_{1}(Z) &\leq \bigg\{ Np \big[ (1-p) \Lambda^2 + p \tau^2 \big] + c_1^2 \big( \tau + \Lambda K(p) \big)^2\\
%		&\qquad \times \Big[ C_3 \sqrt{N}(\sqrt{d} + t ) \vee C_3^2 (\sqrt{d} + t )^2 \Big] \bigg\}^{1/2}
%\end{align*}
%with probability at least $1 - 2 \cdot 9^{-t^2}$. Here, $C_3 = C_3(c) > 0$ is an absolute constant, which depends 
%only on another absolute constant $c$ (appearing in Bernstein's inequality; Lemma \ref{lem:Bernstein})
%\end{lemma}

\begin{proof}
Observe that $Z = Y - pM$ is an $N \times d$ matrix whose rows $Z^i$ are independent, mean zero, 
sub-gaussian random vectors in $\Reals^d$ (see Appendix \ref{sec:properties}). Specifically, we know
\[	\sup_{u \in \bbS^{d-1}} \big\| Z^i u \big\|_{\psi_2} \leq c_1 \big( \tau + \Lambda K(p) \big)	\]
for all $i \in [N]$ by Lemma \ref{lem:subG_Y}.
	
Applying Corollary \ref{cor:op_upper} yields for every $t \geq 0$,
\begin{align*}
	\sigma_{1}(Z) &\leq \bigg\{ \sigma_{1}\big( \Exp{Z^T Z} \big) + c_1^2 \big( \tau + \Lambda K(p) \big)^2
		\Big[ C_3 \sqrt{N}(\sqrt{d} + t ) \vee C_3^2 (\sqrt{d} + t )^2 \Big] \bigg\}^{1/2}
\end{align*}
with probability at least $1 - 2 \cdot 9^{-t^2}$.

By Lemma \ref{lem:cov_Y},
\begin{align*}
	 \Exp{Z^T Z}	
	 	&= p(1-p) diag\big(M^T M \big)	+ p^2 \Exp{ \big(X - M \big)^T \big(X - M \big) }.
\end{align*}
Therefore,
\begin{align*}
	\sigma_{1}\big( \Exp{Z^T Z} \big)
		&\leq p(1-p) \sigma_1 \Big( diag\big(M^T M \big)\Big)	+p^2 \sigma_1 \Big( \Exp{ \big(X - M \big)^T \big(X - M \big) } \Big)\\
		&\leq p(1-p) \max_{j \in [d]} \bigg( \sum_{i=1}^N M_{ij }^2 \bigg) 	+ p^2 \sum_{i=1}^N \sigma_1 \Big( \Exp{ \big(X^i - M^i \big)^T \big(X^i - M^i \big) } \Big)  \\
		&\leq Np \big[ (1-p) \Lambda^2 + p \| X^i \|_{\phi_2}^2 \big]. 
\end{align*}
The last inequality follows from the model assumption $|M_{ij}| \leq \Lambda$ and Lemma \ref{lem:tail_to_variance};
$\Big\| \Exp{ \big(X^i - M^i \big)^T \big(X^i - M^i \Big) } \big\|_2 \leq \| X^i \|_{\phi_2}^2$. 
%\leq \tau^2$ .
\end{proof}



%%% ======================================================================
%%%	Proof of Premise 2
%%% ======================================================================

%\subsection{Proof of Corollary \ref{cor:discrepancy_spectral}}\label{sec:proof_cor_spectral}
%First, we observe an immediate corollary of Lemma \ref{lem:noise_singular}.
%\begin{corollary}\label{cor:Z_spectral}
%	For any $p \in (0, 1]$, 
%	\begin{align*}
%		\sigma_{1}(Z) 
%			&\leq \sqrt{(1-p) \Lambda^2 + p \tau^2} \sqrt{Np}\\
%				&\qquad +c_1\sqrt{C_3 \vee C_3^2} \big( \tau + \Lambda K(p) \big) (\sqrt{N} + \sqrt{d})
%	\end{align*}
%	with probability at least $1 - 2 \cdot 9^{-N}$.
%\end{corollary}


%
%Recall the definition of $\cE_2$ from \eqref{eqn:conditioning_event.2}:
%\[	\cE_2 \triangleq \left\{ \big\| Y - pM \big\|_2 \leq C_1 \sqrt{Np} \right\}.		\]
%
%
%
%
%\begin{proof}
%	By the implication of Lemma \ref{lem:noise_singular} (see Eq. \eqref{eqn:smax_upper}) and a trivial inequality 
%	$(a + b)^{1/2} \leq \sqrt{a} + \sqrt{b}$ for $a, b > 0$, we have
%	\begin{align*}
%		\sigma_1\left( Y - pM \right)
%			&\leq 	\Big[ N \big\| \Sigma_Y (p) \big\|_2 \Big]^{1/2}			\\
%			&\quad+  c_1 \big( \tau + K(p) \big) \big( 2 C_2 Np\big)^{1/2}.	
%	\end{align*}
%	
%	First of all, we argue that $\sigma_1\big( \Sigma_Y(p) \big) = O(p)$. Recall the expression for $\Sigma_Y(p)$ 
%	in Lemma \ref{lem:cov_Y} and observe that $\big((M^1)^T M^1 \big)_{ii} = M_{1i}^2 \leq 1$ for all $i \in [d]$ 
%	by the boundedness assumption ($M^1\in [-1, 1]^d$), and $\big( \Sigma(M^1)\big)_{ii} = e_i^T \Sigma(M^1) e_i 
%	\leq \big\| \Sigma(M^1) \big\|_2 \leq \tau^2$ for all $i \in [d]$. It follows that 
%	\begin{align*}
%		&\Big\| diag\left( (M^1)^T M^1 + \Sigma(M^1) \right) \Big\|_2\\
%			&\qquad= \max_{i \in [d]} \Big( (M^1)^T M^1 + \Sigma(M^1)\Big)_{ii} \\
%			&\qquad\leq \tau^2 + 1.
%	\end{align*}
%	Therefore,
%	
%	We conclude by inserting Eq. \eqref{eqn:prem2.term.2} in Eq. \eqref{eqn:prem2.term.1} that
%	\begin{align*}
%		&\sigma_1\left( Y - pM \right)\\
%		&\qquad\leq \left\{\sqrt{ \tau^2 + 1 - p} + \sqrt{2 C_2} c_1 \big( \tau + K(p) \big) \right\} \sqrt{Np}.
%	\end{align*}
%	Since $\tau = O(1)$ and $\max\{p, 1-p\} \leq 1$, the proof becomes complete by letting $C_1 = \frac{10}{9}\left\{\sqrt{ \tau^2 + 1} 
%	+ c_1\sqrt{2 C_2} \left(  \tau + K(p) \right) \right\}$.
%\end{proof}

==> contents/Appx99_premise3_stable.tex <==
%%% ======================================================================
%%%	Proof of Premise 4
%%% ======================================================================

\section{Deferred Proofs from Section \ref{ssec:premise4}}\label{sec:proof.prem.4}

\subsection{Davis-Kahan $\sin \Theta$ Theorem}\label{sec:DK_sin_theta}

In this section, we recap perturbation bounds for singular subspaces known from literature. Specifically, we recall 
Davis-Kahan $\sin \Theta$ theorem (Wedin's modified version for singular values) \cite{davis1970rotation, 
wedin1972perturbation}, which will be used in our proofs. It would be convenient to keep in mind that $M$ is the 
parameter matrix of our interest, and $\hat{M} = \frac{1}{p}Y$ is the estimate of $M$. We can write $\hat{M} = M + Z$ 
where $Z = \frac{1}{p}Y - M$ is a perturbation.


Let $M \in \Reals^{N \times d}$ be an approximately rank-$r$ matrix with SVD $M = U \Sigma V^T$, 
where $\sigma_r(M) \gg \sigma_{r+1}(M)$. Since the leading $r$ left and right singular vectors of $M$ 
are of our interest, we decompose $M$ as follows:
\begin{equation}\label{eqn:M}
	M = 
	\begin{bmatrix} U_0 & U_{\perp} \end{bmatrix}
	\begin{bmatrix} \Sigma_1 & 0 \\ 0 & \Sigma_2 \end{bmatrix}
	\begin{bmatrix} V_0^T \\ V_{\perp}^T \end{bmatrix},
\end{equation}
where $U_0 \in \Reals^{N \times r}$, $V_0 \in \Reals^{d \times r}$, $\Sigma_1 = diag \big( \sigma_1(M), \ldots, \sigma_r(M) \big)$, 
$\Sigma_2 = diag \big( \sigma_{r + 1}(M), \ldots \big)$ and $\begin{bmatrix} U_0 & U_{\perp} \end{bmatrix} \in 
\Reals^{N \times N}$, $\begin{bmatrix} V_0 & V_{\perp}\end{bmatrix} \in \Reals^{d \times d}$ are orthogonal matrices.

Let $Z$ be a perturbation matrix and let $\hat{M} = M + Z$. We write the SVD of $\hat{M}$ in the same way:
\begin{equation}\label{eqn:Mhat}
	\hat{M} = 
	\begin{bmatrix} \hat{U}_0 & \hat{U}_{\perp} \end{bmatrix}
	\begin{bmatrix} \hat{\Sigma}_1 & 0 \\ 0 & \hat{\Sigma}_2 \end{bmatrix}
	\begin{bmatrix} \hat{V}_0^T \\ \hat{V}_{\perp}^T \end{bmatrix},
\end{equation}
where $\hat{U}_0, \hat{V}_0, \hat{\Sigma}_1, \hat{\Sigma}_2$ have the same structures as $U_0, V_0, \Sigma_1, \Sigma_2$.

Given two $d \times r$ orthogonal columns $V_0$ and $\hat{V}_0$, we measure their distance by the $\sin \Theta$ metric. 
Suppose the singular values of $V_0^T \hat{V}_0$ are $s_1 \geq s_2 \geq \ldots \geq s_r \geq 0$. Then we call 
\[	\Theta(V_0, \hat{V}_0) = diag \big( \arccos(s_1), \arccos(s_2), \ldots, \arccos(s_r)  \big)	\]
as the principal angles between $V_0$ and $\hat{V}_0$. We are particularly interested in the quantitative measure 
$\| \sin \Theta(V, \hat{V}) \| = \sin \arccos(s_r)$, which corresponds to the maximum angle between the column space 
of $V$ and the column space of $\hat{V}$. It is well known that 
\[	\| \sin \Theta(V_0, \hat{V}_0) \| = \| V_0 V_0^T - \hat{V}_0\hat{V}_0^T \|	= \| \cP_{V_0} - \cP_{\hat{V}_0} \|.	\]
Here, $\cP_{V_0} = V_0 V_0^T$ denotes the projection operator onto the column space of $V_0$ when acting by left multiplication.

\begin{theorem}[The generalized $\sin \Theta$ theorem; \cite{wedin1972perturbation}, section 3 ]\label{thm:DK_sin}
	Let $\delta = \max \{ \sigma_r - \hat{\sigma}_{r+1}, \hat{\sigma}_r - \sigma_{r+1}  \}$. If $\delta > 0$, then
	\begin{equation}
		\| \sin \Theta(U_0, \hat{U}_0) \|, \| \sin \Theta(V_0, \hat{V}_0) \| 
			\leq \frac{ \max\{ \|Z V_{\perp} \|, \| Z^T \hat{U}_{\perp} \| \} }{\delta}
	\end{equation}
	for any unitary invariant norm $\| \cdot\|$.
\end{theorem}
Note that $ \max\{ \|Z V_{\perp} \|, \| Z^T \hat{U}_{\perp} \| \} \leq \| Z \|$ for unitary invariant norms.







\subsection{Proof of Lemma \ref{lem:thresholding}}
\begin{proof}%[Proof of Lemma \ref{lem:thresholding}]
%	Let $\hat{M} = SVT\big(\frac{1}{\hat{p}}Y; t\big)$ (soft or hard) with $t = \frac{1}{2}\sqrt{\frac{N \log d }{\hat{p}}}$. 
%	Conditioned on $\cE$, $rank(\hat{M}) = r$.
%	
	First of all, we observe that the data matrix can be decomposed into the scaled parameter matrix plus 
	a perturbation:
	\[	Y = p M + \big( Y - pM \big).	\]
	When conditioned on $\cE_2(\zeta)$, 
	\[	\sigma_1 \left( Y - pM \right) \leq \zeta (\sqrt{N} + \sqrt{d}) \sqrt{p}.	\]	
	Therefore, 
	\begin{align*}
		\sigma_r(Y)	&\geq \sigma_r(pM) - \big\| Y - pM \big\|_2
				\geq p \sigma_r(M) - \zeta (\sqrt{N} + \sqrt{d}) \sqrt{p}, \qquad\text{and} \\
		\sigma_{r+1}(Y)	&\leq \sigma_{r+1}(pM) + \big\| Y - pM \big\|_2
				\leq \zeta (\sqrt{N} + \sqrt{d}) \sqrt{p}. 
	\end{align*}
\end{proof}

\subsection{Proof of Lemma \ref{lem:subsp_stable}}
\begin{proof}%[Proof of Lemma \ref{lem:subsp_stable}]
	We write the data matrix $Y$ as the sum of the signal (=the scaled parameter matrix) $pM$ and a perturbation $Z = Y - pM$:
	\[	Y = pM + (Y - pM).	\]
	As discussed in the proof of Lemma \ref{lem:thresholding}, when conditioned on $\cE_2(\zeta)$,
	$ \sigma_{r+1}(Y) \leq \zeta (\sqrt{N} + \sqrt{d}) \sqrt{p}$.
%	Observe that for any $v \in span\{ V_1, \ldots, V_r \}$, 
%	\[
%		\Big\| v - \hat{V}_{1:r} \hat{V}_{1:r}^T v  \Big\|_2
%			= \Big\| \big(V_{1:r} V_{1:r}^T - \hat{V}_{1:r} \hat{V}_{1:r}^T \big) v \Big\|_2
%			\leq \Big\| V_{1:r} V_{1:r}^T - \hat{V}_{1:r} \hat{V}_{1:r}^T \Big\|_2 \| v \|_2
%			= \| \sin \Theta(V_0, \hat{V}_0) \| _2 \|v \|_2.
%	\]
%	
	When conditioned on $\cE_2(\zeta)$, we conclude by applying Davis-Kahan sin $\theta$ theorem (Theorem \ref{thm:DK_sin}) that
	\begin{align*}
		\| \sin  \Theta(V_{1:r}, \hat{V}_{1:r}) \| _2
			\leq \frac{\big\| Y - pM \big\|_{2}}{\sigma_{r} (pM) - \sigma_{r+1} (Y) }  
			\leq \frac{\zeta(\sqrt{N} + \sqrt{d}) \sqrt{p} }{p \sigma_r(M)- \zeta(\sqrt{N} + \sqrt{d}) \sqrt{p}}
			\leq \frac{\zeta}{\frac{\sqrt{p}\sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta}.
	\end{align*}
\end{proof}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%	We do not use this subsection for now
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse{
\subsection{Perturbation bound when $rank(M) \ll N \wedge d$: Implication of Theorem \ref{thm:Cai_subspace}}

In this section, we present a simplified version of Theorem \ref{thm:Cai_subspace}, which will be used in our proofs. 
It would be convenient to keep in mind $\hat{M} = \frac{1}{p}Y$ and $\tilde{Z} = \frac{1}{p}Y - M$.

Let $M \in \Reals^{N \times d}$ be a rank-$r$ matrix with SVD $M = U \Sigma V^T$. We decompose $M$ as in 
\eqref{eqn:M}:
\begin{equation*}
	M = 
	\begin{bmatrix} U_0 & U_{\perp} \end{bmatrix}
	\begin{bmatrix} \Sigma_1 & 0 \\ 0 & \Sigma_2 \end{bmatrix}
	\begin{bmatrix} V_0^T \\ V_{\perp}^T \end{bmatrix},
\end{equation*}
where $U_0 \in \Reals^{N \times r}$, $V_0 \in \Reals^{d \times r}$, $\Sigma_1 = diag \big( \sigma_1(M), \ldots, \sigma_r(M) \big)$, 
$\Sigma_2 = diag \big( \sigma_{r + 1}(M), \ldots \big)$ and $\begin{bmatrix} U_0 & U_{\perp} \end{bmatrix} \in 
\Reals^{N \times N}$, $\begin{bmatrix} V_0 & V_{\perp}\end{bmatrix} \in \Reals^{d \times d}$ are orthogonal matrices.

Let $\tilde{Z}$ be a perturbation matrix and let $\hat{M} = M + \tilde{Z}$. We write the SVD of $\hat{M}$ in the same way:
\begin{equation*}
	\hat{M} = 
	\begin{bmatrix} \hat{U}_0 & \hat{U}_{\perp} \end{bmatrix}
	\begin{bmatrix} \hat{\Sigma}_1 & 0 \\ 0 & \hat{\Sigma}_2 \end{bmatrix}
	\begin{bmatrix} \hat{V}_0^T \\ \hat{V}_{\perp}^T \end{bmatrix},
\end{equation*}
where $\hat{U}_0, \hat{V}_0, \hat{\Sigma}_1, \hat{\Sigma}_2$ have the same structures as $U_0, V_0, \Sigma_1, \Sigma_2$.

Decompose the perturbation $\tilde{Z}$ into four blocks:
\begin{equation*}
	\tilde{Z} = \tilde{Z}_{11} + \tilde{Z}_{12} + \tilde{Z}_{21} + \tilde{Z}_{22},
\end{equation*}
where
\begin{align*}
	\tilde{Z}_{11} = \cP_{U_0} \tilde{Z} \cP_{V_0},			\qquad&	\tilde{Z}_{21} = \cP_{U_{\perp}} \tilde{Z} \cP_{V_0},\\
	\tilde{Z}_{12} = \cP_{U_0} \tilde{Z} \cP_{V_{\perp}},	\qquad&	\tilde{Z}_{22} = \cP_{U_{\perp}} \tilde{Z} \cP_{V_{\perp}}.
\end{align*}

Suppose that $r = rank(M) \ll N \wedge d$. Since $U_0^T \hat{M} V_0 = U_0^T M V_0 + U_0^T \tilde{Z} V_0 = 
\Sigma_1 + U_0^T \tilde{Z} V_0$, 
\begin{align*}
	  \sigma_r(M) - \| \tilde{Z}_{11} \| \leq \sigma_{\textrm{min}}(U_0^T \hat{M} V_0) \leq \sigma_r(M) + \| \tilde{Z}_{11} \|.
\end{align*}
Similarly, $U_{\perp}^T \hat{M} V_{\perp} = \Sigma_2 + U_{\perp}^T \tilde{Z} V_{\perp}$ and
\[	\| U_{\perp}^T \hat{M} V_{\perp} \| \leq \| \tilde{Z}_{22} \|.	\]

Therefore, simplifying the statement of Theorem \ref{thm:Cai_subspace} reduces to finding upper bounds on 
$\|\tilde{Z}_{11}\|, \|\tilde{Z}_{12}\|, \|\tilde{Z}_{21}\|, \|\tilde{Z}_{22}\|$. 

\DG{Something's wrong...?}
\begin{lemma}
	Let $Z \in \Reals^{N \times d}$ be a random matrix with independent, mean zero, sub-gaussian rows such that
	\[\| Z^i \|_{\psi_2} \leq \tau,~~\forall i \in [N].	\]
	Let $\tilde{U} \in \Reals^{N \times p_1}, \tilde{V} \in \Reals^{d \times p_2}$ have orthogonal columns. Then
	\begin{align*}
		\| \cP_{\tilde{U}} Z \cP_{\tilde{V}} \|^2	&\leq c_2 p_1 \tau^2 + t
	\end{align*}
	with probability at least $1 - 2 \exp \left\{ -c \left( \frac{t^2}{\tau^4 p_1} \wedge \frac{t}{\tau^2 } \right) \right\}$. 
\end{lemma}

\begin{proof}
	Write $\cP_{\tilde{U}} Z \cP_{\tilde{V}} = \tilde{U}\tilde{U}^T Z \tilde{V} \tilde{V}^T$. 
	First, we observe that $Z \tilde{V} \tilde{V}^T$ has independent, mean zero, sub-gaussian rows such that
	\begin{align*}
%		&\Exp{ \big( Z\tilde{V}\tilde{V}^T\big)^T  Z\tilde{V}\tilde{V}^T } \preceq {\Sigma}_{Z}	\quad\text{and}\\
		&\| (Z\tilde{V}\tilde{V}^T)^i \|_{\psi_2} \leq \tau,\quad\forall i \in [N].
	\end{align*}
%	Since $ \Exp{ \big( Z\tilde{V}\tilde{V}^T\big)^T  Z\tilde{V}\tilde{V}^T } = \tilde{V}\tilde{V}^T \Exp{Z^T Z} \tilde{V}\tilde{V}^T$ 
%	and $\Sigma_Z \succeq 0$, for any $v \in \bbS^{d-1}$, 
%	\begin{align*}
%		&v^T  \Big( \Sigma_Z - \Exp{ \big( Z\tilde{V}\tilde{V}^T\big)^T  Z\tilde{V}\tilde{V}^T } \Big) v \\
%			&\leq v^T  \Big( \tilde{V}\tilde{V}^T \Sigma_Z \tilde{V}\tilde{V}^T 
%				-  \tilde{V}\tilde{V}^T \Exp{ Z^T Z }  \tilde{V}\tilde{V}^T \Big) v \\
%			&=  \big(\tilde{V}\tilde{V}^T v \big)^T \big( \Sigma_Z - \Exp{Z^T Z} \big) \big(\tilde{V}\tilde{V}^T v \big)\\
%			&\geq 0.
%	\end{align*}
	It is obvious that 
	\[	\sup_{v \in \bbS^{d-1}} \| Z^i\tilde{V}\tilde{V}^T v \|_{\psi_2} \leq \sup_{v \in \bbS^{d-1}} \| Z^i v \|_{\psi_2} \leq \tau.	\]
	because $\| \tilde{V}\tilde{V}^T v \|_2 \leq \| v \|_2$.
		
	Next, observe that for any $v \in \bbS^{d-1}$, $Z \tilde{V}\tilde{V}^T v \in \Reals^N$ is a random vector with independent, 
	mean zero, sub-gaussian coordinates. Also, we observe that 
	\begin{align*}
		\big( \cP_{\tilde{U}}Z \cP_{\tilde{V}} v  \big)^T \cP_{\tilde{U}}Z \cP_{\tilde{V}} v 
			= v^T \tilde{V}\tilde{V}^T Z^T \tilde{U}\tilde{U}^T Z \tilde{V}\tilde{V}^T v.
	\end{align*}
	
	Now we apply Hanson-Wright inequality (Theorem \ref{thm:HW}): for every $t \geq 0$,
	\begin{align*}
		&\mathbb{P}\bigg(\Big| 
			\big( \cP_{\tilde{U}}Z \cP_{\tilde{V}} v  \big)^T \cP_{\tilde{U}}Z \cP_{\tilde{V}} v  
			- \Exp{\big( \cP_{\tilde{U}}Z \cP_{\tilde{V}} v  \big)^T \cP_{\tilde{U}}Z \cP_{\tilde{V}} v}
			 \Big| \geq t\bigg)\\
		 &\qquad=\mathbb{P}\bigg(\Big| 
			\big( v^T \tilde{V}\tilde{V}^T Z^T \tilde{U}\tilde{U}^T Z \tilde{V}\tilde{V}^T v 
			- \Exp{v^T \tilde{V}\tilde{V}^T Z^T \tilde{U}\tilde{U}^T Z \tilde{V}\tilde{V}^T v}
		 	\Big| \geq t\bigg)\\
		 &\qquad\leq 2 \exp \left\{ -c \left( \frac{t^2}{\tau^4 \| \tilde{U}\tilde{U}^T \|_F^2} \wedge \frac{t}{\tau^2 \| \tilde{U}\tilde{U}^T \|} \right) \right\}.
	\end{align*}
	Since $\tilde{U} \in \Reals^{N \times p_1}$ has orthogonal columns, $\| \tilde{U}\tilde{U}^T \|_F^2 = p_1$ and $\| \tilde{U}\tilde{U}^T \| = 1$.

	This inequality implies
	\begin{align*}
		\| \cP_{\tilde{U}} Z \cP_{\tilde{V}} \|^2 
			&= \sup_{v \in \bbS^{d-1}} \big( \cP_{\tilde{U}}Z \cP_{\tilde{V}} v  \big)^T \cP_{\tilde{U}}Z \cP_{\tilde{V}} v\\
			&\leq \sup_{v \in \bbS^{d-1}} \Exp{\big( \cP_{\tilde{U}}Z \cP_{\tilde{V}} v  \big)^T \cP_{\tilde{U}}Z \cP_{\tilde{V}} v} + t
	\end{align*}
	with probability at least $1 - 2 \exp \left\{ -c \left( \frac{t^2}{\tau^4 p_1} \wedge \frac{t}{\tau^2 } \right) \right\}$. 
	
	Lastly, it is easy to compute the expectation of a chaos.
	\begin{align*}
		\Exp{\big( \cP_{\tilde{U}}Z \cP_{\tilde{V}} v  \big)^T \cP_{\tilde{U}}Z \cP_{\tilde{V}} v}
			&=\Exp{v^T \tilde{V}\tilde{V}^T Z^T \tilde{U}\tilde{U}^T Z \tilde{V}\tilde{V}^T v}\\
			&= \sum_{i,j=1}^{N} \big(\tilde{U}\tilde{U}^T \big)_{ij} \Exp{ (Z \tilde{V}\tilde{V}^T v)_i (Z \tilde{V}\tilde{V}^T v)_j}\\
			&\leq \text{tr}\big(\tilde{U}\tilde{U}^T \big) \| \tilde{V}\tilde{V}^T (Z^i)^T Z^i \tilde{V}\tilde{V}^T \|\\
			&= p_1 \|  \|_{\phi_2}^2\\
			&\leq c_2 p_1 \tau^2.
	\end{align*}
	
	\DG{Why doesn't $p_2$ appear anywhere?}
	We choose $t = (\frac{1}{c} \vee \frac{1}{\sqrt{c}}) p_1 \tau^2 $ and conclude the proof.
\end{proof}



\DG{***TODO}

\begin{theorem}[Corollary of Theorem \ref{thm:Cai_subspace}]
	If 
	\[	\big( \sigma_r(M) - \| \tilde{Z}_{11}\| \big)^2 > \| \tilde{Z}_{22} \|^2 + \| \tilde{Z}_{12} \|^2 \wedge \| \tilde{Z}_{21} \|^2,	\]
	then
	\begin{align*}
		\| \sin \Theta(V, \hat{V}) \|
			&\leq \frac{ \sigma_{r}(M) \| \tilde{Z}_{12} \| + \| \tilde{Z}_{22} \| \| \tilde{Z}_{21} \| }
				{ \big( \sigma_r(M) - \| \tilde{Z}_{11}\| \big)^2 - \| \tilde{Z}_{22} \|^2 - \| \tilde{Z}_{12} \|^2 \wedge \| \tilde{Z}_{21} \|^2}.
	\end{align*}
\end{theorem}

}\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> contents/Appx99_proof_clustering.tex <==
%%% ======================================================================
%%%	Proof of Theorem: Separation of Pairwise Distance
%%% ======================================================================

\section{Proof of Theorem \ref{thm:main_clustering}}\label{sec:proof.main.2}
\begin{proof}
As in the proof of Theorem \ref{thm:rowmaxnorm}, let $\eta = \left( \frac{8 \ln (2N^4d^4)}{3Ndp} \right)^{\frac{1}{2}}$ and 
$\zeta = (\Lambda \vee \tau) \frac{\sqrt{N}}{\sqrt{N} + \sqrt{d}} + \frac{ c_1(\sqrt{C_3} \vee C_3) \big(\tau + \frac{\Lambda}{4} \big)}{\sqrt{p}}$.

Write the SVD of $M$ as $M = U \Sigma V^T$. 
For any pair $a, b \in [k]$, $\mu_a - \mu_b \in span\{ V_1^T, \ldots, V_r^T \}$.
By Proposition \ref{prop:stable_subsp}, when conditioned on $\cE_2(\zeta)$ for some $\zeta > 0$,
\begin{align}
	\big\| \varphi_{Y;t^*}^{\text{hard}} \big( \mu_a \big) - \varphi_{Y;t^*}^{\text{hard}} \big( \mu_b \big) \big\|_2
		&= \big\| \varphi_{Y;t^*}^{\text{hard}} \big( \mu_a - \mu_b \big) \big\|_2		\nonumber\\
		&\geq \big\| \mu_a - \mu_b \big\|_2 
			- \big\| \varphi_{Y;t^*}^{\text{hard}} \big( \mu_a - \mu_b \big) -  \big( \mu_a - \mu_b \big) \big\|_2		\nonumber\\
		&\geq 	\left( 1 - \frac{ \zeta }{\frac{\sqrt{p} \sigma_r(M)} {\sqrt{N} + \sqrt{d}} - \zeta}\right)
			\big\| \mu^a - \mu^b \big\|_2.	\label{eqn:clustering.term.1}
\end{align}

In a similar manner, when conditioned on $\cE_2(\zeta)$ for some $\zeta > 0$,
\begin{align}
	\big\| \varphi_{Y;t^*}^{\text{soft}} \big( \mu_a \big) - \varphi_{Y;t^*}^{\text{soft}} \big( \mu_b \big) \big\|_2
		&= \big\| \varphi_{Y;t^*}^{\text{soft}} \big( \mu_a - \mu_b \big) \big\|_2		\nonumber\\
		&\geq \big\| \mu_a - \mu_b \big\|_2 
			- \big\| \varphi_{Y;t^*}^{\text{soft}} \big( \mu_a - \mu_b \big) -  \big( \mu_a - \mu_b \big) \big\|_2		\nonumber\\
		&\geq  \left( 1 - 	\frac{ \Big[  \Big( \frac{ t^*}{ (\sqrt{N} + \sqrt{d} ) \sqrt{p} }  \Big)^2 + \zeta^2 \Big]^{1/2}}
			{ \frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta } \right)
			\big\| \mu^a - \mu^b \big\|_2.	\label{eqn:clustering.term.2}
\end{align}
Observe that 
\[	\left( 1 - \frac{ \zeta }{\frac{\sqrt{p} \sigma_r(M)} {\sqrt{N} + \sqrt{d}} - \zeta}\right) \geq \frac{1}{2}	\qquad\text{and}\qquad
	\left( 1 - 	\frac{ \Big[  \Big( \frac{ t^*}{ (\sqrt{N} + \sqrt{d} ) \sqrt{p} }  \Big)^2 + \zeta^2 \Big]^{1/2}}
			{ \frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta } \right) \geq \frac{1}{4}	\]
for the given choice of $p$ and $\zeta$.

Now, observe the following. For $i_1, i_2 \in [N]$ such that $\alpha(i_1) = \alpha(i_2)$, 
$M^{i_1} = M^{i_2} = \mu^{\alpha(i_1)}$ and therefore,
\begin{align}	
	&\Big\| \frac{1}{\hat{p}}\varphi_{Y;t^*} \big( Y^{i_1} \big) - \frac{1}{\hat{p}} \varphi_{Y;t^*} \big( Y^{i_2} \big) \Big\|_2	\nonumber\\
	&\qquad\leq		\Big\| \frac{1}{\hat{p}}\varphi_{Y;t^*} \big( Y^{i_1} \big) - \varphi_{Y;t^*} \big( M^{i_1} \big) \Big\|_2	
		+ \Big\| \frac{1}{\hat{p}} \varphi_{Y;t^*} \big( Y^{i_2} \big) - \varphi_{Y;t^*} \big( M^{i_2} \big) \Big\|_2
		+ \Big\| \varphi_{Y;t^*} \big( M^{i_1} \big) - \varphi_{Y;t^*} \big( M^{i_2} \big) \Big\|_2	\nonumber\\
	&\qquad\leq 2  \max_{i \in [N]} \left\| \frac{1}{\hat{p}}  \varphi_{Y;t^*} \big(Y^i \big) - M^i \right\|_{2}.			\label{eqn:intra_cluster}
\end{align}
On the other hand, for $i_1, i_2$ such that $\alpha(i_1) \neq \alpha(i_2)$, 
\begin{align}	
	&\Big\| \frac{1}{\hat{p}}\varphi_{Y;t^*} \big( Y^{i_1} \big) - \frac{1}{\hat{p}} \varphi_{Y;t^*} \big( Y^{i_2} \big) \Big\|_2	\nonumber\\
	&\qquad\geq	\Big\| \varphi_{Y;t^*} \big( M^{i_1} \big) - \varphi_{Y;t^*} \big( M^{i_2} \big) \Big\|_2
		-\Big\| \frac{1}{\hat{p}}\varphi_{Y;t^*} \big( Y^{i_1} \big) - \varphi_{Y;t^*} \big( M^{i_1} \big) \Big\|_2
		- \Big\| \frac{1}{\hat{p}} \varphi_{Y;t^*} \big( Y^{i_2} \big) - \varphi_{Y;t^*} \big( M^{i_2} \big) \Big\|_2	\nonumber\\
	&\qquad\geq	\big\| \varphi_{Y;t^*} \big( \mu_{\alpha(i_1)} \big) - \varphi_{Y;t^*} \big( \mu_{\alpha(i_2)} \big) \big\|_2	
			- 2  \max_{i \in [N]} \left\| \frac{1}{\hat{p}}  \varphi_{Y;t^*} \big(Y^i \big) - M^i \right\|_{2} .	\label{eqn:inter_cluster}
\end{align}
We want a significant gap between the upper bound in Eq. \eqref{eqn:intra_cluster} and the lower bound in Eq. \eqref{eqn:inter_cluster} 
(conditioned on $\cE_1(\eta) \cap \cE_2(\zeta)$).

By Theorem \ref{thm:rowmaxnorm}, 
\begin{align*}
	\max_{i \in [N]} \left\| \hat{M}^i - M^i \right\|_{2} 
		&\leq C' \left( \frac{\sqrt{N} + \sqrt{d}}{p \sigma_r(M)} + \sqrt{\frac{\log (Nd)}{p Nd}} \right)  \left( \max_{i' \in [N]}\big\| M^{i'} \big\|_2\right) \\
		&\qquad+ \frac{C^{''}(\tau + \Lambda K(p))}{p} 
		\left( \sqrt{r \log (Nr)} \vee \frac{ \sqrt{\tau + \Lambda K(p)}d^{\frac{3}{4}}}{\sqrt{\sigma_r(M)}}\log^{\frac{3}{2}}(N \vee d ) \right)
\end{align*}
with probability at least $1-2/(N \vee d)^3$. 

Since $\Prob{\cE_1(\eta)^c \cup \cE_2(\zeta)^c} \leq \frac{2}{N^4d^4} \leq 2/(N \vee d)^3$, it suffices to have
\begin{align*}
	\Delta
		&> 8C' \left( \frac{\sqrt{N} + \sqrt{d}}{p \sigma_r(M)} + \sqrt{\frac{\log (Nd)}{p Nd}} \right)  \left( \max_{i' \in [N]}\big\| M^{i'} \big\|_2\right) \\
		&\qquad+ \frac{8C^{''}(\tau + \Lambda K(p))}{p} 
			\left( \sqrt{r \log (Nr)} \vee \frac{ \sqrt{\tau + \Lambda K(p)}d^{\frac{3}{4}}}{\sqrt{\sigma_r(M)}}\log^{\frac{3}{2}}(N \vee d ) \right)\\
		&\geq 8 \max_{i \in [N]} \left\| \hat{M}^i - M^i \right\|_{2}
\end{align*}
for hard SVT for the distance-based clustering algorithm to succeed with probability at least $1 - 4/(N \vee d)^3$; and
\begin{align*}
	\Delta
		&> 16C' \left( \frac{\sqrt{N} + \sqrt{d}}{p \sigma_r(M)} + \sqrt{\frac{\log (Nd)}{p Nd}} \right)  \left( \max_{i' \in [N]}\big\| M^{i'} \big\|_2\right) \\
		&\qquad+ \frac{16C^{''}(\tau + \Lambda K(p))}{p} 
			\left( \sqrt{r \log (Nr)} \vee \frac{ \sqrt{\tau + \Lambda K(p)}d^{\frac{3}{4}}}{\sqrt{\sigma_r(M)}}\log^{\frac{3}{2}}(N \vee d ) \right)\\
		&\geq 16 \max_{i \in [N]} \left\| \hat{M}^i - M^i \right\|_{2}
\end{align*}
for soft SVT.

\end{proof}




==> contents/Appx99_proof_matrix.tex <==
%%% ======================================================================
%%%	Proof of Theorem: Matrix Estimation
%%% ======================================================================

\section{Proof of Theorem \ref{thm:rowmaxnorm}}\label{sec:proof_theorem.1}

\subsection{Full Version of the Main Theorem}
We state an important Corollary of Theorem \ref{thm:main_thm} here. This will help us conclude 
the proof of Theorem \ref{thm:rowmaxnorm}.  To that end, by applying a simple inequality derived 
from the law of total probability and the union bound, we achieve the following probabilistic bound 
on the max $\ell_2$ row norm of $\frac{1}{\hat{p}} SVT \big( Y; t^* \big) - M$. 

\begin{theorem}\label{thm:max_ell2}
Given any $\eta, \zeta > 0$, let $t^*$ satisfy \eqref{eqn:t.star}. For any $s > s^*_1(p, \eta, \zeta) $,
\begin{align*}
	&\Prob{ \max_{i \in [N]} \left\| \frac{1}{\hat{p}} SVT \big( Y; t^* \big)^i - M^i \right\|_{2} 
		>  \bigg( \Gamma(M; p, \zeta) + \frac{\eta }{1-\eta} \bigg) \max_{i \in [N]} \big\| M^i \big\|_2 + s }\\
		&\qquad	\leq	N\Bigg[ 2r \exp \left( - \frac{ (1-\eta)^2 p^2~ \big\{ s^2 - s^*_1(p, \eta, \zeta)^2 \big\} }
		{4r c_1^2 c_2^2 \big( \tau + \Lambda K(p) \big)^2  } \right)+ \frac{1}{ (N \vee d )^4} \Bigg]
			+ \Prob{\cE_1(\eta)^c \cup \cE_2(\zeta)^c}.
\end{align*}
\end{theorem}
\begin{proof}
	By the usual union bound argument and Theorem \ref{thm:main_thm}, for any given $\eta, \zeta > 0$,
	\begin{align*}
		&\Prob{ \max_{i \in [N]} \left\| \frac{1}{\hat{p}} SVT \big( Y; t^* \big)^i - M^i \right\|_{2} 
			>  \bigg( \Gamma(M; p, \zeta) + \frac{\eta }{1-\eta} \bigg) \max_{i \in [N]} \big\| M^i \big\|_2 + s ~ \bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}\\
		&\qquad=  \Prob{ \bigcup_{i=1}^N \left\{ \left\| \frac{1}{\hat{p}} SVT \big( Y; t^* \big)^i - M^i \right\|_{2} 
			>  \bigg( \Gamma(M; p, \zeta) + \frac{\eta }{1-\eta} \bigg) \max_{i \in [N]} \big\| M^i \big\|_2 + s \right\}~ \bigg|  ~ \cE_1(\eta) \cap \cE_2(\zeta)}\\
		&\qquad\leq \sum_{i=1}^N \Prob{ \left\| \frac{1}{\hat{p}} SVT \big( Y; t^* \big)^i - M^i \right\|_{2} 
			>  \bigg( \Gamma(M; p, \zeta) + \frac{\eta }{1-\eta} \bigg) \max_{i \in [N]} \big\| M^i \big\|_2 + s ~ \bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}\\
		&\qquad\leq \sum_{i=1}^N \Prob{ \left\| \frac{1}{\hat{p}} SVT \big( Y; t^* \big)^i - M^i \right\|_{2} 
			>  \bigg( \Gamma(M; p, \zeta) + \frac{\eta }{1-\eta} \bigg) \big\| M^i \big\|_2 + s ~ \bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}\\
		&\qquad\leq \frac{N}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}} \Bigg[ 2r \exp \left( - \frac{ (1-\eta)^2 p^2~ \big\{ s^2 - s^*_1(p, \eta, \zeta)^2 \big\} }
			{4r c_1^2 c_2^2 \big( \tau + \Lambda K(p) \big)^2  } \right)+ \frac{1}{ (N \vee d )^4} \Bigg].
	\end{align*}
	
	Recall the law of total probability. For any events $E_0, E_1$,
	\begin{align*}
		\Prob{E_0} = \Prob{E_0 | E_1}\Prob{E_1} + \Prob{E_0 | E_1^c}\Prob{E_1^c}	\leq  \Prob{E_0 | E_1}\Prob{E_1} + \Prob{E_1^c}
	\end{align*}
	because probability is always in $[0,1]$. We conclude the proof by letting 
	\begin{align*}
		E_0	&= \left\{  \max_{i \in [N]} \left\| \frac{1}{\hat{p}} SVT \big( Y; t^* \big)^i - M^i \right\|_{2} 
		>  \bigg( \Gamma(M; p, \zeta) + \frac{\eta }{1-\eta} \bigg) \max_{i \in [N]} \big\| M^i \big\|_2 + s \right\},\\
		E_1 &= \cE_1(\eta) \cap \cE_2(\zeta).
	\end{align*}
\end{proof}


\subsubsection{A Simpler Version Assuming $\sigma_r(M) \gg \frac{\sqrt{N}+\sqrt{d}}{p}$}
\begin{theorem}\label{thm:max_ell2_simple}
Given any $\eta, \zeta > 0$ \DG{upper bound on $\zeta$ -- from C.8}, let $t^*$ satisfy \eqref{eqn:t.star}. For any $s > 0 $,
\begin{align*}
	&\Prob{ \max_{i \in [N]} \left\| \frac{1}{\hat{p}} SVT \big( Y; t^* \big)^i - M^i \right\|_{2} 
		>  \bigg( \Gamma(M; p, \zeta) + \frac{\eta }{1-\eta} \bigg) \max_{i \in [N]} \big\| M^i \big\|_2 + s }\\
		&\qquad	\leq	
				4Nd
				\exp\Bigg( - \frac{(1-\eta)^2 p^2}{2 c_1^2 c_2^2 \big( \tau + \Lambda K(p) \big)^2} 
				\frac{1}{\Big(1 + \sqrt{\frac{d}{r}} \frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta} \Big)^2} 
				\frac{ s^2}{r} \Bigg)
			+ \Prob{\cE_1(\eta)^c \cup \cE_2(\zeta)^c}.
\end{align*}
\end{theorem}
\begin{proof}
	Follow the same line of arguments as in the proof of Theorem \ref{thm:max_ell2} except that we utilize 
	Proposition \ref{prop:subG_proj_simple} in place of Proposition \ref{prop:subG_proj}.
	\begin{align*}
		&\Prob{ \max_{i \in [N]} \left\| \frac{1}{\hat{p}} SVT \big( Y; t^* \big)^i - M^i \right\|_{2} 
			>  \bigg( \Gamma(M; p, \zeta) + \frac{\eta }{1-\eta} \bigg) \max_{i \in [N]} \big\| M^i \big\|_2 + s ~ \bigg| ~ \cE_1(\eta) \cap \cE_2(\zeta)}\\
		&\qquad\leq\frac{4Nd}{\Prob{\cE_1(\eta) \cap \cE_2(\zeta)}}
				\exp\Bigg( - \frac{(1-\eta)^2 p^2}{2 c_1^2 c_2^2 \big( \tau + \Lambda K(p) \big)^2} 
				\frac{1}{\Big(1 + \sqrt{\frac{d}{r}} \frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta} \Big)^2} 
				\frac{ s^2}{r} \Bigg).
	\end{align*}
	We conclude the proof by applying the union bound.
\end{proof}

We interpret Theorem \ref{thm:max_ell2_simple} in this way. For any $\eta, \zeta > 0$, 
\begin{align*}
	\max_{i \in [N]} \left\| \frac{1}{\hat{p}} SVT \big( Y; t^* \big)^i - M^i \right\|_{2} 
		&\leq  \bigg( \Gamma(M; p, \zeta) + \frac{\eta }{1-\eta} \bigg) \max_{i \in [N]} \big\| M^i \big\|_2 \\
			&\quad+ \frac{ 2\sqrt{2} c_1 c_2 \big( \tau + \Lambda K(p) \big)}{(1-\eta) p} 
				\bigg(1 + \sqrt{\frac{d}{r}} \frac{\zeta}{\frac{\sqrt{p} \sigma_r(M)}{\sqrt{N} + \sqrt{d}} - \zeta} \bigg) \sqrt{r \log(4Nd)}
\end{align*}
with probability at least $1 - \frac{1}{(4Nd)^3} - \Prob{\cE_1(\eta)^c \cup \cE_2(\zeta)^c}$.



\subsection{Complexity Analysis on $p$ and $N$}\label{sec:complexity}
First, we observe the following lower bound on $p$, which is set by our analysis.
\begin{remark}\label{rem:p_lower}		
	We need
	$$p \geq \left(\frac{ c_1\big(\sqrt{C_3} \vee C_3 \big) \big(\tau + \frac{\Lambda}{4} \big)}{\zeta - 
	(\Lambda \vee \tau) \frac{\sqrt{N}}{\sqrt{N} + \sqrt{d}}}\right)^2$$ 
	because of Lemma \ref{lem:spectral}. 
\end{remark}

Recall the definition of $\Gamma$ (see \eqref{eqn:Gamma}). We want $\Gamma = o(1)$ to obtain a vanishing max $\ell_2$ error; see Theorem \ref{thm:max_ell2}. 
An even more stringent condition, namely, $\Gamma = O\left( \frac{\Delta}{\sqrt{d \log N}} \right)$, is needed for our simple distance-based 
mixture clustering algorithm to work. 
These conditions are satisfied for hard SVT provided that $\zeta = o\left( \frac{\sqrt{p}\sigma_r(M)}{\sqrt{N} + \sqrt{d}} \right)$
and $\zeta = O\left( \frac{\Delta}{\sqrt{d \log N}} \frac{\sqrt{p}\sigma_r(M)}{\sqrt{N} + \sqrt{d}} \right)$, respectively. 

Suppose that $\sigma_r(M) \gg \sqrt{N} + \sqrt{d}$. Letting $\zeta =  \frac{\sqrt{p}\sigma_r(M)}{\sqrt{N} + \sqrt{d}}$ as per Remark \ref{rem:zeta_upper}, 
we can observe $p = \omega \left( \frac{\sqrt{N} + \sqrt{d}}{\sigma_r(M)} \right)^2$ 
%and $p = \Omega \left( \frac{\sqrt{d \log N}}{\Delta} \frac{\sqrt{N} + \sqrt{d}}{\sigma_r(M)} \right)$
is necessary. We obtain a similar result for soft SVT; when $t^* = \Theta(\zeta)$, the same requirement for $p$ holds.

Recall the definition of $s^*_1(p, \eta, \zeta)$ (see \eqref{eqn:s_star.1}). We need $s^*_1(p, \eta, \zeta) = o(\sqrt{d})$. 
That is to say, 
$\frac{1}{p} \frac{d^{3/2}}{\sigma_r(M)} \big(\log (N \vee d)\big)^3 = o(d)$, and equivalently, $\sigma_r(M) = \omega \left( \frac{\sqrt{d}}{p}  
\big(\log (N \vee d)\big)^3 \right)$. If we assume $\sigma_r(M) = \Theta \left( \sqrt{\frac{Nd}{r}} \right)$, this leads to 
$N = \omega \left( \frac{r}{p^2} \big(\log (N \vee d)\big)^6  \right)$.
If we require $s^*_1(p, \eta, \zeta) = O\big(\frac{\Delta^2}{\log N}\big)$, then $\sigma_r(M) = \Omega \left( \frac{d\sqrt{d}}{p \Delta^2} \big(\log (N \vee d)\big)^4 \right)$
is necessary; assuming $\sigma_r(M) = \Theta \left( \sqrt{\frac{Nd}{r}} \right)$ leads to 
$N = \Omega \left( \frac{d^2 r}{p^2 \Delta^4} \big(\log (N \vee d)\big)^8  \right)$. In other words, the additional requirement increases the sample complexity 
by the multiplicative factor of $\frac{d^2}{\Delta^4} (\log N)^2$.



\subsection{Proof of Theorem \ref{thm:rowmaxnorm}}
We choose the value of $\eta, \zeta > 0$ based on the observation in section \ref{sec:conditioning}. Theorem \ref{thm:rowmaxnorm} naturally follows from 
Theorem \ref{thm:max_ell2}, once the asymptotic behavior of terms are examined as per section \ref{sec:complexity}.
\begin{proof}
Choosing $\eta = \left( \frac{8 \ln (2N^4d^4)}{3Ndp} \right)^{\frac{1}{2}}$ implies $\Prob{\cE_1(\eta)^c}\leq \frac{1}{N^4d^4}$. 
Letting $\zeta = (\Lambda \vee \tau) \frac{\sqrt{N}}{\sqrt{N} + \sqrt{d}} + \frac{ c_1(\sqrt{C_3} \vee C_3) \big(\tau + \frac{\Lambda}{4} \big)}{\sqrt{p}}$,
$\Prob{\cE_2(\zeta)^c} \leq 2 \cdot 9^{-N} \leq \frac{1}{N^4d^4}$ for a sufficiently large $N$.

Theorem \ref{thm:rowmaxnorm} follows from realizing that 
\begin{enumerate}
	\item
	$\frac{\eta}{1-\eta} = O \left( \sqrt{\frac{\log(Nd)}{Ndp}} \right)$; 
	\item
	$ \Gamma(M; p, \zeta) = O\left( \frac{\zeta(\sqrt{N} + \sqrt{d})}{\sqrt{p}\sigma_r(M)}\right) 
		= O\left( \frac{\sqrt{N} + \sqrt{d}}{p\sigma_r(M)}\right)$ (see \eqref{eqn:Gamma});
	\item$ s^*_1(p, \eta, \zeta) = O\left( \frac{ (\tau + \Lambda K(p))^{\frac{3}{2}}d^{\frac{3}{4}}}{p \sqrt{\sigma_r(M)}} \log^{3/2} (N \vee d ) \right)$ 
		(see \eqref{eqn:s_star.1}); 
	\item
	$\frac{2 \sqrt{r} c_1 c_2 (\tau + \Lambda K(p))}{ (1-\eta)p} = O \left( \frac{\tau + \Lambda K(p)}{p}\sqrt{r} \right)$; and
	\item
	for $p$ in the given range, $t^*$ satisfies the assumption in Corollary \ref{cor:rank_model} with the aforementioned choice of $\zeta$, i.e., 
	$$\zeta \big( \sqrt{N} + \sqrt{d} \big) \sqrt{p}	 < t^* < 	p \sigma_r(M) - \zeta \big( \sqrt{N} + \sqrt{d} \big) \sqrt{p}.	$$ 
\end{enumerate}
\end{proof}


==> contents/AppxA_subgaussian.tex <==
%%% ======================================================================
%%%	Appendix: Sub-gaussian Random Variables
%%% ======================================================================

\subsection{Sub-gaussian Random Variable}\label{sec:subg_rv}

%%% ======================================================================
%%%	Basic Properties
%%% ======================================================================

\subsubsection{Basic Properties}\label{sec:subG_properties}
%In fact, we are interested more in the variance proxy of the $i$-th row of $Y - pM$ than its covariance structure. 
Here we recall some properties of sub-gaussian random variables.
We may assume the random variable $X$ of our interest is centered, i.e., $\Exp{X} = 0$, 
and define sub-gaussianity of the random variable utilizing the Laplace transform characterization. 
Other equivalent characterizations are also presented in Proposition \ref{prop:subG_characterization} 
(see section \ref{sec:subG_characterization}).

\begin{definition}
	A real-valued random variable $X$ with $\Exp{X} = 0$ is said to be sub-gaussian if there exists 
	$\tau_X < \infty$ such that 
	\begin{equation}\label{eqn:laplace}
		\Exp{e^{\lambda X}} \leq e^{\frac{1}{2}\lambda^2 \tau_X^2} \text{ for all }\lambda \in \Reals.
	\end{equation}
	We refer to the infimum of $\tau_X^2$ satisfying Eq. \eqref{eqn:laplace} as the variance proxy of $X$.
\end{definition}

Given two sub-gaussian random variables, the sum of them is still sub-gaussian and the variance proxy 
of the sum has an upper bound in terms of the variance proxies of the original random variables.

\begin{proposition}\label{prop:phi2_independent}
	Suppose that $X_1, X_2$ are sub-gaussian random variables with variance proxy $\tau_{X_1}^2, \tau_{X_2}^2$, 
	respectively. Then $X_1 + X_2$ is also sub-gaussian with variance proxy $\tau_{X_1 + X_2}^2 \leq 
	\big(\tau_{X_1} + \tau_{X_2} \big)^2$.
\end{proposition}
\begin{proof}
	Let $p, q >1$ satisfy $\frac{1}{p} + \frac{1}{q} = 1$. By H\"older's inequality,
	\begin{align*}
		\Exp{e^{\lambda(X_1 + X_2)}}
			&= \Big\| e^{\lambda X_1} e^{\lambda X_2} \Big\|_{L^1}\\
			&\leq \Big\| e^{\lambda X_1}\Big\|_{L^p} \Big\| e^{\lambda X_2} \Big\|_{L^q}\\
			&= \Exp{\Big( e^{\lambda X_1} \Big)^p}^{1/p} \Exp{\Big( e^{\lambda X_2} \Big)^q}^{1/q}\\
			&\leq e^{\frac{1}{2} \lambda^2 p \tau_{X_1}^2} e^{\frac{1}{2} \lambda^2 q \tau_{X_2}^2}\\
			&= e^{\frac{1}{2} \left( p \tau_{X_1}^2 + \frac{p}{p-1} \tau_{X_2}^2 \right)}.
	\end{align*}
	Minimizing the last term over $p >1$, we obtain $\Exp{e^{\lambda(X_1 + X_2)}}\leq 
	e^{\frac{1}{2}\lambda^2(\tau_{X_1} + \tau_{X_2})^2}$ with the choice of $p = p^* 
	= \frac{\tau_{X_1}+\tau_{X_2}}{\tau_{X_1}}$.
\end{proof}

We have a stronger upper bound on the variance proxy of the sum of sub-gaussian random variables when 
the two summands, $X_1$ and $X_2$, are independent.

\begin{proposition}
	Suppose that $X_1, X_2$ are independent sub-gaussian random variables with variance proxy 
	$\tau_{X_1}^2, \tau_{X_2}^2$, respectively. Then $X_1 + X_2$ is also sub-gaussian with variance proxy 
	$\tau_{X_1 + X_2}^2 \leq \tau_{X_1}^2 + \tau_{X_2}^2$.
\end{proposition}
\begin{proof}
	Due to the independence between $X_1$ and $X_2$,
	\begin{align*}
		\Exp{e^{\lambda(X_1 + X_2)}}
			= \Exp{e^{\lambda X_1}}\Exp{e^{\lambda X_2}}
			\leq e^{\frac{1}{2}\lambda^2 \big(\tau_{X_1}^2 + \tau_{X_2}^2 \big)}.
	\end{align*}
\end{proof}


%%% ======================================================================
%%%	Characterization
%%% ======================================================================

\subsubsection{Equivalent Characterizations of Sub-gaussian Random Variables}\label{sec:subG_characterization}
There are various ways to characterize a sub-gaussian random variable. 
\begin{proposition}[Proposition 2.5.2 in \cite{vershynin2018high}]\label{prop:subG_characterization}
	Let $X$ be a random variable. Then the following properties are equivalent. Moreover, the parameters $K_i > 0$ 
	appearing in each of the properties differ from each other by at most an absolute constant factor; there exists an 
	absolute constant $C$ such that property $i$ with parameter $K_i$ implies property $j$ with parameter $K_j \leq C K_i$ 
	for any two properties $i, j \in \{1, 2, 3, 4, 5\}$.
	\begin{enumerate}
		\item
		The tails of $X$ satisfy
		\[	\Prob{|X| \geq t} \leq 2 \exp \left( - \frac{t^2}{K_1^2} \right), \qquad\forall t\geq0.	\]
		\item
		The moments of $X$ satisfy
		\[	\|X\|_{L^p} = \Big( \Exp{\big|X\big|^p} \Big)^{1/p} \leq K_2 \sqrt{p}, \qquad\forall p\geq1.	\]
		\item
		The MGF of $X^2$ satisfies
		\[	\Exp{\exp(\lambda^2 X^2)} \leq \exp(K_3^2 \lambda^2),	\quad\forall \lambda\text{ s.t. }|\lambda| \leq \frac{1}{K_3}.	\]
		\item
		The MGF of $X^2$ is bounded at some point, namely
		\[	\Exp{\exp\left( \frac{X^2}{K_4^2} \right)} \leq 2.	\]
		
	\end{enumerate}
	Moreover, if $\Exp{X} = 0$, then properties 1-4 are also equivalent to the following one.
	\begin{enumerate}
		\item[(5)]
		The MGF of $X$ satisfies
		\[	\Exp{\exp(\lambda X)} \leq \exp(K_5^2 \lambda^2),	\qquad\forall \lambda \in \Reals.	\]
	\end{enumerate}
\end{proposition}

The equivalence between (2) and (5) in Proposition \ref{prop:subG_characterization} suggests that the covariance 
(=the second central moment) of a sub-gaussian random vector is bounded. The next lemma certifies this with a 
tight constant.

%\begin{remark}\label{rem:subG_subE}
%In a similar manner, one can define sub-exponential random variables. The sub-exponential norm of $X$, denoted $\| X \|_{\psi_1}$, 
%is defined as
%\[	\| X \|_{\psi_1} \triangleq \inf \left\{ t > 0: \bbE \exp \left(\frac{|X|}{t} \leq 2 \right) \right\}.	\]
%
%It is known that a random variable is sub-gaussian if and only if $X^2$ is sub-exponential. Moreover, 
%\[	\| X^2 \|_{\psi_1} = \| X \|_{\psi_2}^2.	\]
%
%For more details, see \cite[Definition 2.7.5, Lemma 2.7.6]{vershynin2018high}, for example.
%\end{remark}


\begin{lemma}\label{lem:tail_to_variance}
Suppose that $X$ is a sub-gaussian random vector with $\| X \|_{\phi_2} = \tau$. Then 
\[	\Big\| ~\Exp{ (X - \Exp{X}) (X - \Exp{X})^T} \Big\|_2 \leq \tau^2.	\]
\end{lemma}

\begin{proof}
Choose a vector $u \in \bbS^{d-1}$ and define a function 
\[	f_u(\lambda) = \exp\bigg( \frac{\lambda^2 \tau^2}{2}\bigg) - \Exp{ \exp \big( \lambda u^T (X - \Exp{X}) \big)}.	\] 
It is easy to see $f_u(0) = \exp(0) - \exp(0) = 0$.

We consider the first and the second derivatives of $f_u(\lambda)$ evaluated at $\lambda = 0$. 
Recall the following property of the moment generating function (MGF) that for any positive integer $k$,
\begin{align*}
	\frac{d^k}{d\lambda^k} \Exp{\exp \big( \lambda u^T (X - \Exp{X}) \big)}\Big|_{\lambda = 0}
		&= \Exp{ \big( u^T (X - \Exp{X}) \big)^k }.
\end{align*}

Therefore, we can observe
\begin{align*}
	\frac{d}{d \lambda} f_u (\lambda) \Big|_{\lambda = 0}
		&= \lambda \tau^2 \exp\bigg( \frac{\lambda^2 \tau^2}{2}\bigg) \bigg|_{\lambda = 0} - \Exp{u^T(X - \Exp{X})}\\
		&= 0
\end{align*}
and
\begin{align*}
	\frac{d^2}{d \lambda^2} f_u (\lambda) \Big|_{\lambda = 0}
		&= \big(\tau^2 + \lambda^2 \tau^4 \big) \exp\bigg( \frac{\lambda^2 \tau^2}{2}\bigg) \bigg|_{\lambda = 0}
			- \Exp{u^T(X - \Exp{X})( X - \Exp{X})^T u }.
\end{align*}

Since we assumed $\| X \|_{\phi_2} = \tau$, 
\[	\Exp{ \exp \big( \lambda u^T (X - \Exp{X}) \big)} \leq \exp\bigg( \frac{\lambda^2 \tau^2}{2}\bigg),	\quad\forall \lambda \in \Reals	\] 
by definition of $\| \cdot \|_{\phi_2}$, and hence, $f_u(\lambda) \geq 0$ for all $\lambda \in \Reals$. 
We have seen $f_u(0) = 0, \frac{d}{d\lambda}f_u(0) = 0$. If $\frac{d^2}{d \lambda^2} f_u (\lambda) \Big|_{\lambda = 0} < 0$, 
there exists $\lambda_*$ in the neighborhood of $0$ such that $f_u(\lambda_*) < 0$. This is a contradiction. 

Therefore, $\frac{d^2}{d \lambda^2} f_u (\lambda) \Big|_{\lambda = 0} \geq 0$ and
\[	 \Exp{u^T(X - \Exp{X})(X - \Exp{X})^T u} \leq \tau^2.	\]
The proof is complete as the upper bound holds for all $u \in \bbS^{d-1}$.
\end{proof}






==> contents/AppxB_aux_lemmas.tex <==
%%% ======================================================================
%%%	Appendix: Spectral Norm of Random Matrices with Independent Rows
%%% ======================================================================

\subsection{Spectral Norm of a Random Matrix with Independent Rows}
A concentration inequality (Lemma \ref{lem:corr_op}) essential in the proof of Lemma \ref{lem:noise_singular} 
is presented. This is a classic result in high-dimensional statistics and random matrix theory, and we follow 
Vershynin's version; see Theorem 5.39 and Remark 5.40 in \cite{vershynin2010introduction}.

\subsubsection{Concentration of Spectral Norm}
\begin{lemma}\label{lem:corr_op}
	Let $A$ be an $N \times d$ matrix whose rows $A_i$ are independent, mean zero, sub-gaussian 
	random vectors in $\Reals^d$. Then for every $t \geq 0$,
	\begin{align*}
		&\left\| \frac{1}{N} A^T A - \Sigma ~\right\|_{2} \leq K^2 \max\{ \delta, \delta^2 \} 
			\qquad\text{where}\quad \delta = c_3\left(\sqrt{\frac{d}{N}}+ \frac{t}{\sqrt{N}}\right)	
	\end{align*}
	with probability at least $1 - 2 \cdot 9^{-t^2}$. Here, $K = \max_i \| A^i \|_{\psi_2}$, $\Sigma = \frac{1}{N} 
	\Exp{ A^T A}$, and $c_3 = c_3(c_0) > 0$ is an absolute constant\footnote{$c_0$ is another absolute 
	constant that is from Lemma \ref{lem:Bernstein}}.
\end{lemma}

This lemma directly implies an upper bound on $\sigma_1(A)$.
\begin{corollary}\label{cor:op_upper}
Let $A$ be an $N \times d$ matrix whose rows $A_i$ are independent, mean zero, sub-gaussian 
random vectors in $\Reals^d$. Then for every $t \geq 0$,
\begin{align*}
	\sigma_{1}(A) %&= \sigma_{1}(A^T A)^{1/2}\\
	&\leq \bigg\{ N\sigma_{1}(\Sigma) + K^2  \Big[ c_3 \sqrt{N}(\sqrt{d} + t ) \vee c_3^2 (\sqrt{d} + t )^2 \Big] \bigg\}^{1/2}
\end{align*}
with probability at least $1 - 2 \cdot 9^{-t^2}$.
\end{corollary}

%By a trivial inequality 
%	$(a + b)^{1/2} \leq \sqrt{a} + \sqrt{b}$ for $a, b > 0$, we have
%	\begin{align*}
%		\sigma_1\left( Y - pM \right)
%			&\leq 	\Big[ N \big\| \Sigma_Y (p) \big\|_2 \Big]^{1/2}			\\
%			&\quad+  c_1 \big( \tau + K(p) \big) \big( 2 C_2 Np\big)^{1/2}.	
%	\end{align*}
%	
%



\subsubsection{Technical Tools for the Proof of Lemma \ref{lem:corr_op}}
We need the following auxiliary lemmas to prove Lemma \ref{lem:corr_op}. These results, including the proof 
of Lemma \ref{lem:corr_op} can be found in standard textbooks on high-dimensional probability and statistics; 
see \cite{vershynin2018high} for example.

\paragraph{Sub-exponential Random Variables}
\begin{definition}
	The sub-exponential norm of a random variable $X$, denoted $\|X\|_{\psi_1}$ is defined as
	\[	\|X\|_{\psi_1} \triangleq \inf \left\{ t > 0: \Exp{ \exp \left(\frac{|X|}{t} \right)} \leq 2 \right\}.	\]
	$X$ is called a sub-exponential random variable if $\|X\|_{\psi_1} < \infty$.
\end{definition}

\begin{lemma}\label{lem:subE_subG}
	A random variable $X$ is sub-gaussian if and only if $X^2$ is sub-exponential. In addition,
	\[	\| X^2 \|_{\psi_1} = \| X \|_{\psi_2}^2.	\]
\end{lemma}

\begin{lemma}[centering]\label{lem:centering}
	If $X$ is a sub-gaussian random variable, then so is $X - \bbE X$. Moreover, there exists an absolute constant $C$ such that
	\begin{align*}
		\| X - \bbE X \|_{\psi_2} &\leq C \| X \|_{\psi_2}.
	\end{align*}
	
	Similarly, if $X$ is a sub-exponential random variable, 
	so is $X - \bbE X$. 
	\begin{align*}
		\| X - \bbE X \|_{\psi_1} &\leq C \| X \|_{\psi_1}.
	\end{align*}
\end{lemma}

\begin{lemma}[Bernstein's inequality]\label{lem:Bernstein}
	Let $X_1, \ldots, X_N$ be independent, mean zero, sub-exponential random variables. Then, for every $t \geq 0$, we have
	\begin{align*}
		\Prob{\left| \sum_{i=1}^N X_i \right| \geq t}
			&\leq	2 \exp \left[ - c_0 \min \left( \frac{t^2}{\sum_{i=1}^N \| X_i \|_{\psi_1}^2}, \frac{t}{\max_i \| X_i \|_{\psi_1}} \right) \right],
	\end{align*}
	where $c_0>0$ is an absolute constant.
\end{lemma}

\paragraph{The $\eps$-net Argument}
Let $\cN(K, \eps)$ denote the covering number of $K$--the 
smallest possible cardinality of an $\eps$-net--and $\cP(K, \eps)$ denote the packing number of $K$--the largest possible cardinality of 
an $\eps$-separated subset of a given set $K$.
\begin{lemma}\label{lem:aux1}
	Let $K$ be a subset of $\Reals^d$ and $\eps > 0$. Then
	\[	\frac{vol(K)}{vol(\eps B_2^d)} \leq \cN(K, \eps) \leq \cP(K, \eps) 
			\leq \frac{vol(K + \frac{\eps}{2}B_2^d)}{vol(\frac{\eps}{2} B_2^d)}.	\]
\end{lemma}
\begin{corollary}\label{cor:aux1}
	The covering number of the unit Euclidean ball $B_2^d$ satisfy the following bounds for any $\eps > 0$:
	\[	\left(\frac{1}{\eps}\right)^d \leq \cN(B_2^d, \eps) \leq \left(\frac{2}{\eps} + 1\right)^d. 	\]
	The same upper bound is true for $\bbS^{d-1}$.
\end{corollary}
\begin{lemma}\label{lem:aux2}
	Let $A$ be an $N \times d$ matrix and $\eps \in [0, 1)$. Then for any $\eps$-net $\cN$ of the sphere $\bbS^{d-1}$, 
	we have
	\[	\sup_{x \in \cN} \| Ax \|_2 \leq \| A \|_2 \leq \frac{1}{1 - \eps} \sup_{x \in \cN} \| Ax \|_2.	\]
\end{lemma}

\subsubsection{Proof of Lemma \ref{lem:corr_op}}
\begin{proof}%[Proof of ]
	We can find a $\frac{1}{4}$-net $\cN$ of the unit sphere $\bbS^{d-1}$ with cardinality $|\cN| \leq 9^d$ due to Corollary \ref{cor:aux1}. 
	Then it follows that
	\begin{align*}
		\left\| \frac{1}{N}A^T A - \Sigma~ \right\| 
			&\leq 2 \max_{x \in \cN} \left| x^T \left( \frac{1}{N}A^T A - \Sigma \right) x \right|\\
			&= 2 \max_{x \in \cN}  \left| \frac{1}{N} \|A x \|_2^2 - x^T \Sigma x \right|.
	\end{align*}
	It suffices to show the following inequality holds with the required probability:
	\[	\max_{x \in \cN}  \left| \frac{1}{N} \|A x \|_2^2 - x^T \Sigma x \right| 
			\leq \frac{\eps}{2} \quad\text{where}\quad \eps := K^2 \max\{ \delta, \delta^2\}.	\]
	
	For any fixed $x \in \bbS^{d-1}$, we can write $\|Ax\|_2^2$ as a sum of independent random variables:
	$ \|Ax\|_2^2 = \sum_{i=1}^N \big( A^i x \big)^2$,
	where $A^i$ denotes the $i$-th row of $A$. $A^i$'s are independent and $\| A^i x \|_{\psi_2} \leq K$ 
	by assumption. 
	
	The squared random variable $(A^i x )^2 = x^T A_i A_i^T x$ is sub-exponential (Lemma \ref{lem:subE_subG}) 
	and so is the centered version (Lemma \ref{lem:centering}). That is to say, $x^T A_i A_i^T x - x^T \Exp{A_i A_i^T } x$ 
	are independent, mean zero, and sub-exponential random variables with
	\[	\Big\|~ x^T A_i A_i^T x - x^T \Exp{A_i A_i^T } x ~ \Big\|_{\psi_1} \leq C K_i^2.	\]
	
	Recall that $ \Sigma = \frac{1}{N}\sum_{i=1}^N \Exp{ (A^i)^T A^i}$. Applying Bernstein's inequality (Lemma \ref{lem:Bernstein}), 
	we obtain
	\begin{align*}
		\Prob{\left| \frac{1}{N} \| Ax \|_2^2 - x^T \Sigma x \right| \geq \frac{\eps}{2}}
			&	= \Prob{\left| \frac{1}{N} \sum_{i=1}^N \left( x^T A_i A_i^T x - x^T \Exp{A_i A_i^T} x \right) \right| \geq \frac{\eps}{2}}\\
			&	\leq 2 \exp \left[ -c_0 N \min \left\{ \frac{N\eps^2}{\sum_i K_i^4}, \frac{\eps}{\max_i K_i^2} \right\} \right]\\
			&	\leq 2 \exp \left[ -c_0 N \min \left\{ \frac{\eps^2}{K^4}, \frac{\eps}{K^2} \right\} \right]\\
			&	=	2 \exp \left[ - c_0 \delta^2 N \right]		\qquad \because \frac{\eps}{K^2} = \max \{ \delta, \delta^2 \}\\
			&	\leq	2 \exp \left[ -c_0 c_3^2( d + t^2 ) \right].
	\end{align*}
	The last inequality follows from the definition of $\delta$ and the inequality $(a+b)^2 \geq a^2 + b^2$ for $a, b \geq 0$.
	
	Lastly, applying the union bound over all choices of $x \in \cN$, we obtain
	\begin{align*}
		\Prob{ \max_{x \in \cN} \left| \frac{1}{N} \| Ax \|_2^2 - x^T \Sigma x \right| \geq \frac{\eps}{2}}
			&	\leq |\cN| \cdot 2 \exp \left[ -c_0 c_3^2( d + t^2 ) \right]\\
			&	\leq 2 \exp\left[ \big(2\ln 3 -c_0 c_3^2\big) d \right] \exp \left[  - c_0 c_3^2 t^2 \right]\\
			&	\leq 2 \cdot 9^{- t^2 }
	\end{align*}
	if we choose $c_3$ sufficiently large, e.g., $c_3 \geq \sqrt{\frac{2 \ln 3}{c_0}}$, where $c_0>0$ is an absolute 
	constant (cf. Lemma \ref{lem:Bernstein}).
\end{proof}
	
%\subsection{Hanson-Wright Inequality}
%\begin{theorem}\label{thm:HW}
%	Let $X = (X_1, \ldots, X_n) \in \Reals^n$ be a random vector with independent, mean zero, sub-gaussian coordinates. 
%	Let $A$ be an $n \times n$ matrix. Then, for every $t \geq 0$, we have
%	\begin{align*}	
%		\Prob{\big| X^T A X - \Exp{X^T A X} \big| \geq t}
%			&	\leq 2 \exp \left[ - c\left( \frac{t^2}{K^4 \| A \|_F^2} \wedge \frac{t}{K^2 \|A \|} \right) \right],	
%	\end{align*}
%	where $K = \max_{i \in [n]} \| X_i \|_{\psi_2}$.
%\end{theorem}



==> contents/AppxC_davis_kahan.tex <==

\subsection{Subspace Stability and Davis-Kahan Sin $\Theta$ Theorem}\label{sec:DK_sin_theta}
In this section, we recap perturbation bounds for singular subspaces known from literature. Specifically, we recall 
Davis-Kahan $\sin \Theta$ theorem (Wedin's modified version for singular values) \cite{davis1970rotation, 
wedin1972perturbation}, which will be used in our proofs. It would be convenient to keep in mind that $M$ is the 
parameter matrix of our interest, and $\hat{M} = \frac{1}{p}Y$ is the estimate of $M$. We can write $\hat{M} = M + Z$ 
where $Z = \frac{1}{p}Y - M$ is a perturbation.


Let $M \in \Reals^{N \times d}$ be an approximately rank-$r$ matrix with SVD $M = U \Sigma V^T$, 
where $\sigma_r(M) \gg \sigma_{r+1}(M)$. Since the leading $r$ left and right singular vectors of $M$ 
are of our interest, we decompose $M$ as follows:
\begin{equation}\label{eqn:M}
	M = 
	\begin{bmatrix} U_0 & U_{\perp} \end{bmatrix}
	\begin{bmatrix} \Sigma_1 & 0 \\ 0 & \Sigma_2 \end{bmatrix}
	\begin{bmatrix} V_0^T \\ V_{\perp}^T \end{bmatrix},
\end{equation}
where $U_0 \in \Reals^{N \times r}$, $V_0 \in \Reals^{d \times r}$, $\Sigma_1 = diag \big( \sigma_1(M), \ldots, \sigma_r(M) \big)$, 
$\Sigma_2 = diag \big( \sigma_{r + 1}(M), \ldots \big)$ and $\begin{bmatrix} U_0 & U_{\perp} \end{bmatrix} \in 
\Reals^{N \times N}$, $\begin{bmatrix} V_0 & V_{\perp}\end{bmatrix} \in \Reals^{d \times d}$ are orthogonal matrices.

Let $Z$ be a perturbation matrix and let $\hat{M} = M + Z$. We write the SVD of $\hat{M}$ in the same way:
\begin{equation}\label{eqn:Mhat}
	\hat{M} = 
	\begin{bmatrix} \hat{U}_0 & \hat{U}_{\perp} \end{bmatrix}
	\begin{bmatrix} \hat{\Sigma}_1 & 0 \\ 0 & \hat{\Sigma}_2 \end{bmatrix}
	\begin{bmatrix} \hat{V}_0^T \\ \hat{V}_{\perp}^T \end{bmatrix},
\end{equation}
where $\hat{U}_0, \hat{V}_0, \hat{\Sigma}_1, \hat{\Sigma}_2$ have the same structures as $U_0, V_0, \Sigma_1, \Sigma_2$.

Given two $d \times r$ orthogonal columns $V_0$ and $\hat{V}_0$, we measure their distance by the $\sin \Theta$ metric. 
Suppose the singular values of $V_0^T \hat{V}_0$ are $s_1 \geq s_2 \geq \ldots \geq s_r \geq 0$. Then we call 
\[	\Theta(V_0, \hat{V}_0) = diag \big( \arccos(s_1), \arccos(s_2), \ldots, \arccos(s_r)  \big)	\]
as the principal angles between $V_0$ and $\hat{V}_0$. We are particularly interested in the quantitative measure 
$\| \sin \Theta(V, \hat{V}) \| = \sin \arccos(s_r)$, which corresponds to the maximum angle between the column space 
of $V$ and the column space of $\hat{V}$. It is well known that 
\[	\| \sin \Theta(V_0, \hat{V}_0) \| = \| V_0 V_0^T - \hat{V}_0\hat{V}_0^T \|	= \| \cP_{V_0} - \cP_{\hat{V}_0} \|.	\]
Here, $\cP_{V_0} = V_0 V_0^T$ denotes the projection operator onto the column space of $V_0$ when acting by left multiplication.

\begin{theorem}[The generalized $\sin \Theta$ theorem; \cite{wedin1972perturbation}, section 3 ]\label{thm:DK_sin}
	Let $\delta = \max \{ \sigma_r - \hat{\sigma}_{r+1}, \hat{\sigma}_r - \sigma_{r+1}  \}$. If $\delta > 0$, then
	\begin{equation}
		\| \sin \Theta(U_0, \hat{U}_0) \|, \| \sin \Theta(V_0, \hat{V}_0) \| 
			\leq \frac{ \max\{ \|Z V_{\perp} \|, \| Z^T \hat{U}_{\perp} \| \} }{\delta}
	\end{equation}
	for any unitary invariant norm $\| \cdot\|$.
\end{theorem}
Note that $ \max\{ \|Z V_{\perp} \|, \| Z^T \hat{U}_{\perp} \| \} \leq \| Z \|$ for unitary invariant norms.








==> contents/AppxC_subspace.tex <==
%%% ======================================================================
%%%	Appendix: Subspace Stability
%%% ======================================================================

\section{Stability of Subspace under Perturbation}
In this section, we recap perturbation bounds for singular subspaces known from literature \cite{cai2018rate}. 
\cite{davis1970rotation, wedin1972perturbation}
Let $M \in \Reals^{N \times d}$ be an approximately rank-$r$ matrix with SVD $M = U \Sigma V^T$, 
where $\sigma_r(M) \gg \sigma_{r+1}(M)$. Since the leading $r$ left and right singular vectors of $M$ 
are of our interest, we decompose $M$ as follows:
\begin{equation}\label{eqn:M}
	M = 
	\begin{bmatrix} U_0 & U_{\perp} \end{bmatrix}
	\begin{bmatrix} \Sigma_1 & 0 \\ 0 & \Sigma_2 \end{bmatrix}
	\begin{bmatrix} V_0^T \\ V_{\perp}^T \end{bmatrix},
\end{equation}
where $U_0 \in \Reals^{N \times r}$, $V_0 \in \Reals^{d \times r}$, $\Sigma_1 = diag \big( \sigma_1(M), \ldots, \sigma_r(M) \big)$, 
$\Sigma_2 = diag \big( \sigma_{r + 1}(M), \ldots \big)$ and $\begin{bmatrix} U_0 & U_{\perp} \end{bmatrix} \in 
\Reals^{N \times N}$, $\begin{bmatrix} V_0 & V_{\perp}\end{bmatrix} \in \Reals^{d \times d}$ are orthogonal matrices.

Let $Z$ be a perturbation matrix and let $\hat{M} = M + Z$. We write the SVD of $\hat{M}$ in the same way:
\begin{equation}\label{eqn:Mhat}
	\hat{M} = 
	\begin{bmatrix} \hat{U}_0 & \hat{U}_{\perp} \end{bmatrix}
	\begin{bmatrix} \hat{\Sigma}_1 & 0 \\ 0 & \hat{\Sigma}_2 \end{bmatrix}
	\begin{bmatrix} \hat{V}_0^T \\ \hat{V}_{\perp}^T \end{bmatrix},
\end{equation}
where $\hat{U}_0, \hat{V}_0, \hat{\Sigma}_1, \hat{\Sigma}_2$ have the same structures as $U_0, V_0, \Sigma_1, \Sigma_2$.

Given two $d \times r$ orthogonal columns $V_0$ and $\hat{V}_0$, we measure their distance by the $\sin \Theta$ metric. 
Suppose the singular values of $V_0^T \hat{V}_0$ are $s_1 \geq s_2 \geq \ldots \geq s_r \geq 0$. Then we call 
\[	\Theta(V_0, \hat{V}_0) = diag \big( \arccos(s_1), \arccos(s_2), \ldots, \arccos(s_r)  \big)	\]
as the principal angles between $V_0$ and $\hat{V}_0$. We are particularly interested in the quantitative measure 
$\| \sin \Theta(V, \hat{V}) \| = \sin \arccos(s_r)$, which corresponds to the maximum angle between the column space 
of $V$ and the column space of $\hat{V}$. It is well known that 
\[	\| \sin \Theta(V_0, \hat{V}_0) \| = \| V_0 V_0^T - \hat{V}_0\hat{V}_0^T \|	= \| \cP_{V_0} - \cP_{\hat{V}_0} \|.	\]
Here, $\cP_{V_0} = V_0 V_0^T$ denotes the projection operator onto the column space of $V_0$ when acting by left multiplication.

Decompose the perturbation $Z$ into four blocks:
\begin{equation}\label{eqn:Z}
	Z = Z_{11} + Z_{12} + Z_{21} + Z_{22},
\end{equation}
where
\begin{align*}
	Z_{11} = \cP_{U_0} Z \cP_{V_0},			\qquad&	Z_{21} = \cP_{U_{\perp}} Z \cP_{V_0},\\
	Z_{12} = \cP_{U_0} Z \cP_{V_{\perp}},	\qquad&	Z_{22} = \cP_{U_{\perp}} Z \cP_{V_{\perp}}.
\end{align*}

\begin{theorem}[\cite{cai2018rate}, Theorem 1]\label{thm:Cai_subspace}
	Let $M, \hat{M}$ and $Z$ be given as \eqref{eqn:M},\eqref{eqn:Mhat},\eqref{eqn:Z}. 
	If 
	\[	\sigma_{\textrm{min}}(U_0^T \hat{M} V_0)^2 > \| U_{\perp}^T \hat{M} V_{\perp} \|^2 + \| Z_{12} \|^2 \wedge \| Z_{21} \|^2,	\]
	then
	\begin{align*}
		&\| \sin \Theta(V_0, \hat{V}_0) \|\\
			&\quad\leq \frac{ \sigma_{\textrm{min}}(U_0^T \hat{M} V_0) \| Z_{12} \| + \| U_{\perp}^T \hat{M} V_{\perp} \| \| Z_{21} \| }
				{ \sigma_{\textrm{min}}(U_0^T \hat{M} V_0)^2 - \| U_{\perp}^T \hat{M} V_{\perp} \|^2 - \| Z_{12} \|^2 \wedge \| Z_{21} \|^2} ,
	\end{align*}
	and
	\begin{align*}
		&\| \sin \Theta(U_0, \hat{U}_0) \|\\
			&\quad\leq \frac{ \sigma_{\textrm{min}}(U_0^T \hat{M} V_0) \| Z_{21} \| + \| U_{\perp}^T \hat{M} V_{\perp} \| \| Z_{12} \| }
				{ \sigma_{\textrm{min}}(U_0^T \hat{M} V_0)^2 - \| U_{\perp}^T \hat{M} V_{\perp} \|^2 - \| Z_{12} \|^2 \wedge \| Z_{21} \|^2} .
	\end{align*}
\end{theorem}



==> contents/figure1.tex <==
\begin{figure*}[t!]
\centering
	\begin{subfigure}{0.1\linewidth}
		\centering
		\hfill
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		True labels
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		Unlabelled data
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		Estimated labels
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		Pairwise distances
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		After SVT
	\end{subfigure}
	%
	\\
	%
	\begin{subfigure}{0.1\linewidth}
		\centering
		Success\\
		($\sigma=0.3$)
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma03_expnum50_p10_principal_2d_true.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma03_expnum50_p10_principal_2d.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma03_expnum50_p10_principal_2d_estimated.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma03_expnum50_p10_hist_orig.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma03_expnum50_p10_hist_svd.png}
	\end{subfigure}
	%
	\\
	%
	\begin{subfigure}{0.1\linewidth}
		\centering
		Partial success\\
		($\sigma=0.5$)
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma05_expnum50_p10_principal_2d_true.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma05_expnum50_p10_principal_2d.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma05_expnum50_p10_principal_2d_estimated.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma05_expnum50_p10_hist_orig.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma05_expnum50_p10_hist_svd.png}
	\end{subfigure}
	%
	\\
	%
	\begin{subfigure}{0.1\linewidth}
		\centering
		Failure\\
		($\sigma=1.0$)
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma10_expnum50_p10_principal_2d_true.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma10_expnum50_p10_principal_2d.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma10_expnum50_p10_principal_2d_estimated.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma10_expnum50_p10_hist_orig.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.17\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/exp1_works/figure_synthetic_d30_k100_sigma10_expnum50_p10_hist_svd.png}
	\end{subfigure}
	\caption{Illustration of how Algorithm \ref{alg:main_algorithm} works for Gaussian noise model at three noise levels: $\sigma \in \{ 0.3, 0.5, 1.0 \}$. }
%		From left to right, each column displays (a) ranking profiles with true label in top-2 principal components; (b) ranking profiles with the labels 
%		deleted; (c) ranking profiles with the labels reconstructed by the algorithm; (d) histogram of pairwise distance; and (e) histogram of pairwise 
%		distance after singular value thresholding.}
	\label{fig:algorithm_works}
\end{figure*}
